AdaCap: Adaptive Capacity control for Feed-Forward Neural Networks

The capacity of a ML model refers to the range of functions this model can approximate. It impacts both the complexity of the patterns a model can learn but also memorization, the ability of a model to fit arbitrary labels. We propose Adaptive Capacity (AdaCap), a training scheme for Feed-Forward Neural Networks (FFNN). AdaCap optimizes the capacity of FFNN so it can capture the high-level abstract representations underlying the problem at hand without memorizing the training dataset. AdaCap is the combination of two novel ingredients, the Muddling labels for Regularization (MLR) loss and the Tikhonov operator training scheme. The MLR loss leverages randomly generated labels to quantify the propensity of a model to memorize. We prove that the MLR loss is an accurate in-sample estimator for out-of-sample generalization performance and that it can be used to perform Hyper-Parameter Optimization provided a Signal-to-Noise Ratio condition is met. The Tikhonov operator training scheme modulates the capacity of a FFNN in an adaptive, differentiable and data-dependent manner. We assess the effectiveness of AdaCap in a setting where DNN are typically prone to memorization, small tabular datasets, and benchmark its performance against popular machine learning methods.

==> Old/Old_main/Karim_attempt_section_MLR_loss.tex <==
An over-parameterized model trained on $\mathcal{D}_{train}$ can generalize
\sout{outperform the intercept model on the test set $\mathcal{D}_{test}$} even though it perfectly memorized the training set. This means that this trained model was able to learn generalizing patterns between features and targets. This phenomenon, known as benign overfitting, was highlighted for Deep Neural Network (\DNN) for instance in \cite{zhang2016understanding,arpit2017closer} where it was argued that gradient descent schemes used to train over-parametrized deep learning models perform some form of implicit regularization. However, this does not necessarily mean that the trained model contains only generalizing patterns.It is more likely that it contains both some generalizing patterns but also some spurious patterns that correspond only to memorisation of the training set. These spurious patterns may degrade the model performance on the test set. Based on this observation, we asked ourselves the following question:

{\it Is it possible to discriminate generalizing patterns from spurious ones during training and thus retain only the generalizing patterns?}

If we can design such a method, then it may be possible to train over-parametrized models more efficiently even with a limited number of observations.

In order to understand the benign overfitting phenomenon for \sgd-trained \DNN{},  \cite{zhang2016understanding,arpit2017closer} empirically compared the learning dynamics of \sgd-trained over-parametrized \DNN{} on the original data versus randomized data (e.g. partially corrupted labels, random labels, shuffling or random generation of features). They highlighted that these models tend to learn meaningful patterns first before eventually memorizing the whole train set. In addition, \cite{arpit2017closer} found that "explicit regularization
can substantially limit the speed of memorization of noise data without significantly impacting learning on real data." 

Note that \cite{zhang2016understanding,arpit2017closer} only used randomised data as an investigation tool. In our paper, we want to exploit randomised data further to train a \DNN{} model with improve generalization performance. 


Our first idea was to train two \DNN{} with identical architecture in parallel, one on the true data and the other on randomized labels. Comparing their train loss provides a metric to quantify the memorization occurring in the model. Minimizing this metric during training should remove the negative impact of memorization on the generalization performance of the \DNN{} trained on the true data. \textcolor{red}{This idea did not lead to anything good}.

Second we tried to solve the following bi-level optimization problem on the train set. For a \DNN{} model with weights $\theta$ and loss $L$, solve
\begin{align}
    &\widehat{\theta} = \mathrm{argmin}_{\theta} L\left(\bY,f_{\theta}(\bx)\right)\\
    &\hspace{1cm}\text{subject to}\quad \theta \in \mathrm{argmin}_{\theta} \sum_{t=1}^{T}|L\left(\bY_{\texttt{perm}_t},\bY_{intercept}\right) -  L\left(\bY_{\texttt{perm}_t},f_{\theta}(\bx)\right)|.\notag
\end{align}





 After further investigation, we built the \MLR{} loss that leverages randomized labels and allows to train only one \DNN{}-model with improved 


As it turned out, we built a metric that allows us to train only one 







% \paragraph{Initial idea.} An over-parameterized \FFNN{} trained on $\mathcal{D}_{train}$ can outperform the intercept model on the test set $\mathcal{D}_{test}$ if it is able to learn generalizable patterns between features and targets. However, since an over-parameterized \FFNN{} is also able to memorize the training set, it will try to minimize the loss on the training set using both memorization and generalization, which can lead to overfitting.

% Indeed, in over-parametrized models, there are a lot of possible directions to explore to reduce training error {\color{red}via Gradient Descent (GD), known to be a greedy procedure.} GD selects the direction of steepest descent. The gradient direction corresponding to the quadratic loss contains both meaningful patterns and memorization. {\color{red}How to disentangle the directions  containing only memorization from the one containing meaningful patterns ?}


% An over-parameterized \FFNN{} trained on $\mathcal{D}_{train}$ can outperform the intercept memorized the training set.

% Over-parametrized neural nets trained on the train set $\mathcal{D}_{train}$ can outperform the intercept model on the test set $\mathcal{D}_{test}$ even though they perfectly reproduce the training set. This means that this trained neural nets are able to learn generalizable patterns between features and targets. This phenomenon is known as bening overfitting and was observed in several situations \cite{?}. 
 



==> Old/Old_main/brouillon_intro.tex <==





DNN trained by conventional methods with small datasets commonly shows worse performance than traditional machine learning methods

%Another important aspect of many tabular data learning tasks is the small number of training samples.




data regime.




the proposed DNN approaches do not consistently outperform the state-of-the-art shallow models by a notable margin.



The main goal of this paper to present a new DL architecture that adresses this point.


%a large number of Kaggle ML competitions with tabular data are still won by the shallow GBDT methods (Harasymiv, 2015).





However, there is no clear DNN still underperforms classical machine methods (RF, Gradient Boosting Trees (GBTs) on many tabular dataset learning tasks \cite{}. 


However there is no dominant DNN architecture to tackle tabular dataset learning tasks



still underperforms classical machine methods (RF, Gradient Boosting Trees (GBTs) on many tabular dataset learning tasks \cite{}. 



However, to the best of our knowledge, there is no yet a state-of-the-art DNN architecture for tabular data.


have not yet proposed efficient architectures to tackle tabular data. 


Learning tasks on tabular data did not benefit yet from the full power



However DNN still underperforms Gradient Boosting Trees (GBTs) on many tabular dataset learning tasks \cite{}. 






While the superiority of deep architectures in these domains is undoubtful, machine learning for tabular data still did not fully benefit from the DNN power.   Namely,  the state-of-the-art perfor-mance in problems with tabular heterogeneous data is often achieved by ”shallow” models, such as gradient boosted decision trees (GBDT) (Friedman, 2001; Chen & Guestrin, 2016; Ke et al., 2017;Prokhorenkova et al., 2018). While the importance of deep learning on tabular data is recognized by the ML community,  and many works address this problem (Zhou & Feng, 2017; Yang et al.,2018; Miller et al., 2017; Lay et al., 2018; Feng et al., 2018; Ke et al., 2018), the proposed DNN approaches do not consistently outperform the state-of-the-art shallow models by a notable margin. In particular, to the best of our knowledge, there is still no universal DNN approach that was shown to systematically outperform the leading GBDT packages (e.g., XGBoost (Chen & Guestrin, 2016)).As additional evidence, a large number of Kaggle ML competitions with tabular data are still wonby the shallow GBDT methods (Harasymiv, 2015).  Overall, at the moment, there is no dominant deep learning solution for tabular data problems, and we aim to reduce this gap by our paper.





%Deep learning works remarkably well, and has helped dra-matically  improve  the  state-of-the-art  in  areas  ranging from  speech  recognition,  translation  and  visual  object recognition  to  drug  discovery,  genomics  and  automatic game playing (1]  Y. LeCun, Y. Bengio, and G. Hinton, Nature521, 436(2015).[2]  Y. Bengio, Foundations and trendsR©in Machine Learn-ing2, 1 (2009).)

DNN are typically overparametrized but paradoxically achieve low generalization error ([3]) for reasons that have yet to be fully understood. Nevertheless, it is widely accepted that DNN can achieve excellent generalization performance when lots of data is available. Learning DNN parameters requires to run a large number of iterations that can result in overfitting and poor generalization performance for small data sets.


https://arxiv.org/pdf/1706.08947.pdf



This issue is especially predominant for ...

In several fields of sciences, collecting data is costly \cite{}, there


However for relatively small data, DNN trained by conventional methods underperform traditional ensemble methods (Random forest, GBT). 


data augmentation, drop-out, 

Our method requires only a small number of iterations to train several networks with small variance and reasonable generalization. Next we combine these networks to obtain the final prediction with reduced variance and improved generalization.


%https://arxiv.org/pdf/1706.08947.pdf
%
%Learning with deep neural networks has enjoyed huge empirical success in recent years across a wide variety of tasks. Despite being a complex, non-convex optimization problem, simple methods such as stochastic gradient descent (SGD) are able to recover good solutions that minimize the training error.More surprisingly, the networks learned this way exhibit good generalization behavior, even whenthe number of parameters is significantly larger than the amount of training data
%%
%%B. Neyshabur, R. Tomioka, and N. Srebro.  In search of the real inductive bias:  On the role of implicit regularization in deep learning.Proceeding of the International Conference onLearning Representations workshop track, 2015
%%C. Zhang, S. Bengio, M. Hardt, B. Recht, and O. Vinyals. Understanding deep learning requiresrethinking generalization. InInternational Conference on Learning Representations, 2017.



can learn several nets in a few iterations and combines them to obtain the final prediction



%£This difficulty stems 

%Learning DNN parameters requires to run a large number of iterations that can result in overfitting for small data sets.




from the low availability of data,









Neural networks are the basic building blocks of Deep learning models. However, Deep neural networks have millions of parameters to learn and this means we need a lot of iterations before we find the optimum values. If we have small data, running a large number of iteration can result in overfitting. Large dataset helps us avoid overfitting and generalizes better as it captures the inherent data distribution more effectively.





DNN trained on 

Large neural nets trained on relatively small datasets can overfit the training data.

If we have small data, running a large number of iteration can result in overfitting. Large dataset helps us avoid overfitting and generalizes better as it captures the inherent data distribution more effectively
However, DNN trained by conventional methods with small datasets commonly shows worse performance than traditional machine learning methods, e.g. shallow neural network and support vector machine. This inherent limitation prevented the wide adoption of DNN in material study because collecting and assembling big dataset in material science is a challenge.



Modern neural networks (NNs) have way more parameters than training data points, which allow them to achieve near-zero training error while simultaneously — for some reason yet to be understood — have low generalization error ([3])


%Neural networks are the basic building blocks of Deep learning models. However, Deep neural networks have millions of parameters to learn and this means we need a lot of iterations before we find the optimum values. 

DNN are popular for their ability to generalize and handle massive dataset.
It is widely accepted that Deep learning exhibits excellent generalization performance when lots of data is available.  
DNN have to learn millions of parameters, often more than the number of training points which allow them to achieve near-zero training error while simultaneously — for some reason yet to be understood — have low generalization error .




It is widely accepted that Deep learning requires lot of data to achieve excellent generalization performance. 


Large neural nets trained on relatively small datasets can overfit the training data.
If we have small data, running a large number of iteration can result in overfitting. Large dataset helps us avoid overfitting and generalizes better as it captures the inherent data distribution more effectively
However, DNN trained by conventional methods with small datasets commonly shows worse performance than traditional machine learning methods, e.g. shallow neural network and support vector machine. This inherent limitation prevented the wide adoption of DNN in material study because collecting and assembling big dataset in material science is a challenge.


https://arxiv.org/pdf/1412.6614.pdf


\paragraph{Justification pourquoi s'interesser aux petit jeux de données}

In several fields of sciences, large data sets are unavailable as collecting and assembling lots of data is too expensive \cite{}. 





Thus we only have access t  Therefore are not available \cite{}. 

\paragraph{Ce qui est fait en pratique pour SmallD : Methodes ensembliste RF...}


\paragraph{smallData deep}

With limited training data, however, many of these complicated relationships will be the result of sampling noise, so they will exist in the training set but not in real test data even if it is drawn from the same distribution. This leads to overfitting and many methods have been developed for reducing it. These include stopping the training as soon as performance on a validation set starts to get worse, introducing weight penalties of various kinds such as L1 and L2 regularization and soft weight sharing (Nowlan and Hinton, 1992)

Drop out (n>500); data augmentation; transfert; early stopping; regularization: pen l1,L2

Modern Neural Networks Generalize on Small Data Sets

Drop out does not work for extremely small data sets ($n\leq 500$) \cite{}. 

\paragraph{Ce qui est fait en Deep pour les SmallD : Visio et image}

Transfer learning (TL) is a cornerstone of computer vision. It consists in transfering knowledge from an ImageNet pre-trained CNN to another task on a smaller data set. TL can lead to significant generalization improvement \cite{Razavian2014,}. But it may sometimes result in worse performances for data sets with large domain mismatch \cite{pulkit2014,?,?,[4]}. 




\paragraph{Ce qui est fait en deep pour smallD tabulaire :rien pas grand chose}

Modern Neural Networks Generalize on Small Data Sets classif.

Net-DNF: Effective Deep Modeling of Tabular Data




\paragraph{nombre de neurone}

Increasing the number of hidden units, thereby increasing the number of parameters, can lead to a decrease in generalization error even when the training error does not decrease [19]. We would expect to see the complexity measure decrease as we increase the number of hidden units.

[19] B. Neyshabur, R. Tomioka, and N. Srebro. In search of the real inductive bias: On the role of implicit regularization in deep learning. Proceeding of the International Conference on Learning Representations workshop track, 2015.


- DNN popular for their ability to generalize and handle massive dataset.

- Incredible success of deep neural networks (DNN) in a large number of machine learning tasks: computer vision [1], natural language processing, speech recognition [2], reinforcement learning (Goodfellow et al., 2016). 

- DNN still underperforms Gradient Boosting Trees (GBTs) on many tabular-dataset learning tasks. 




References:

[1] Alex Krizhevsky, Ilya Sutskever, and Geoffrey E Hinton. ImageNet Classification with Deep Convolu- tional Neural Networks.  

[2] Chung-Cheng Chiu, Tara N Sainath, Yonghui Wu, Rohit Prabhavalkar, Patrick Nguyen, Zhifeng Chen, Anjuli Kannan, Ron J Weiss, Kanishka Rao, Ekaterina Gonina, Navdeep Jaitly, Bo Li, Jan Chorowski, and Michiel Bacchiani Google. State-Of-The-Art Speech Recognition with Sequence-To-Sequence Models.  

[3] Chiyuan Zhang, Samy Bengio, Moritz Hardt, Benjamin Recht, and Oriol Vinyals. Understanding deep learning requires rethinking generalization. arXiv preprint arXiv:1611.03530, 2016.

[4] H.-C.  Shin,  H.  R.  Roth,  M.  Gao,  L.  Lu,  Z.  Xu,  I.  Nogues,  J.  Yao,D. Mollura, and R. M. Summers, “Deep convolutional neural networksfor  computer-aided  detection:  Cnn  architectures,  dataset  characteristicsand transfer learning,”IEEE transactions on medical imaging, vol. 35,no. 5, pp. 1285–1298, 2016.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{brouillon}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage



# Towards Understanding the Role of Over-Parametrization in Generalization of Neural Networks (2018)


As part of our investigation we will establish that large neural networks with tens of thousands of parameters are capable of achieving superior test accuracy on data sets with only hundreds of observations. This is surprising, as it is commonly thought that deep neural networks require largedata sets to train properly [19,7].  We believe that this gap in knowledge has led to the commonmisbelief that unregularized, deep neural networks will necessarily overfit the types of data consideredby small-data professions.  In fact, we establish that with minimal tuning, deep neural networksare able to achieve performance on par with a random forest classifier, which is considered to havestate-of-the-art performance on data sets from the UCI Repository

[7] Noah Golowich, Alexander Rakhlin, and Ohad Shamir. Size-independent sample complexity of neural networks.arXiv preprint arXiv:1712.06541, 2017

19]Behnam Neyshabur, Ruslan Salakhutdinov, and Nathan Srebro. Path-SGD: Path-normalized optimization in deepneural networks. InAdvances in Neural Information Processsing Systems (NIPS), 2015



The mechanism by which a random forest is able to generalize well on small data sets is straightfor-ward: a random forest is an ensemble of low-bias, decorrelated trees. Randomization combined withaveraging reduces the ensemble’s variance, smoothing out the predictions from fully grown trees. Itis clear that a neural network should excel at bias reduction, but the way in which it achieves variance reduction is much more mysterious. The same paradox has been examined at length in the literature on AdaBoost, and in particular, it has been conjectured that the later stages of AdaBoost serve as abaggingphase which reduces variance [4, 5, 6, 23]


# cholet 

You’ll  sometimes  hear  that  deep  learning  only  works  when  lots  of  data  is  available.



# Neural Network Modeling for Small Datasets

Bartlett (1998) showingthat the generalization performance of an MLP depends moreon theL1norm‖c‖1of the weights between the hidden layerand the output layer rather than on the total number of weights.




# Learnability, stability and uniform convergence. Journal of Machine Learning Research, 11:2635–2670, October 2010.





# Harnessing the Power of Infinitely Wide Deep Nets on Small-dataTasks
https://arxiv.org/pdf/1910.01663.pdf

We recall that recently Olson et al. (2018) showed that multilayer neural networks can be reasonably effective on small datasets,specifically on a UCI testbed of tasks with as few as dozens of training examples. Of course, this requiredsome hyperparameter tuning, although they noted that such tuning is also needed for the champion method,Random Forests (RF), which multilayer neural networks could not beat


Can NTK’s do better? Below wewill see that in the setup of Olson et al. (2018), NTK predictors indeed outperforms corresponding finite deepnetworks, and also slightly beats the earlier gold standard, RandomForests. This suggests NTK predictorsshould belong in any list of off-the-shelf machine learning methods.














# DeepLabCut: markerless pose estimation of user-defined body parts with deep learning
Nature Neuroscience volume 21, pages1281–1289(2018)

Quantifying behavior is crucial for many applications in neuroscience. Videography provides easy methods for the observation and recording of animal behavior in diverse settings, yet extracting particular aspects of a behavior for further analysis can be highly time consuming. In motor control studies, humans or other animals are often marked with reflective markers to assist with computer-based tracking, but markers are intrusive, and the number and location of the markers must be determined a priori. Here we present an efficient method for markerless pose estimation based on transfer learning with deep neural networks that achieves excellent results with minimal training data. We demonstrate the versatility of this framework by tracking various body parts in multiple species across a broad collection of behaviors. Remarkably, even when only a small number of frames are labeled (~200), the algorithm achieves excellent tracking performance on test frames that is comparable to human accuracy.


#Spectrally-normalized margin bounds for neural networks
Peter L. Bartlett∗Dylan J. Foster†Matus Telgarsky
https://arxiv.org/pdf/1706.08498.pdf

Neural networks owe their astonishing success not only to their ability to fit any data set: they also generalize well, meaning they provide a close fit on unseen data. A classical statistical adage is that models capable of fitting too much will generalize poorly; what’s going on here?

any analysis based solely on the number of possible labellings on a finite training set — as is thecase with VC dimension — is doomed: if the function class can fit all possible labels (as is the case withneural networks in standard configurations (Zhang et al., 2017)), then this analysis can not distinguish it from the collection of all possible functions!




# champs d'application petit dataset

https://www.ncbi.nlm.nih.gov/pmc/articles/PMC4454870/
(environnement)


Electronic health records:
- AlvinRajkomar,EyalOren,KaiChen,AndrewMDai,NissanHajaj,MichaelaHardt,PeterJLiu,Xiaob- ing Liu, Jake Marcus, Mimi Sun, Patrik Sundberg, Hector Yee, Kun Zhang, Yi Zhang, Gerardo Flores, Gavin E Duggan, Jamie Irvine, Quoc Le, Kurt Litsch, Alexander Mossin, Justin Tansuwan, De Wang, James Wexler, Jimbo Wilson, Dana Ludwig, Samuel L Volchenboum, Katherine Chou, Michael Pearson, Srinivasan Madabushi, Nigam H Shah, Atul J Butte, Michael D Howell, Claire Cui, Greg S Corrado, and Jeffrey Dean. Scalable and accurate deep learning with electronic health records. npj Digital Medicine, 1, 2018.

- Riccardo Miotto,LiLi,BrianAKidd,andJoelTDudley.DeepPatient:AnUnsupervisedRepresentation to Predict the Future of Patients from the Electronic Health Records. Nature Publishing Group, 2016. 



# NEURAL OBLIVIOUS DECISION ENSEMBLES FOR DEEP LEARNING ON TABULAR DATA
1909.06312.pdf

In an important case of heterogenous tabular data, the advantage of DNNs over shallow counterparts remains questionable. In particular, there is no sufficient evidence that deep learning machinery allows constructing methods that outperform gradient boosting decision trees (GBDT), which are of- ten the top choice for tabular problems. 

While the superiority of deep architectures in these domains is undoubtful, machine learning for tabular data still did not fully benefit from the DNN power. Namely, the state-of-the-art perfor- mance in problems with tabular heterogeneous data is often achieved by ”shallow” models, such as gradient boosted decision trees (GBDT) (Friedman, 2001; Chen & Guestrin, 2016; Ke et al., 2017; Prokhorenkova et al., 2018). While the importance of deep learning on tabular data is recognized by the ML community, and many works address this problem (Zhou & Feng, 2017; Yang et al., 2018; Miller et al., 2017; Lay et al., 2018; Feng et al., 2018; Ke et al., 2018), the proposed DNN approaches do not consistently outperform the state-of-the-art shallow models by a notable margin. In particular, to the best of our knowledge, there is still no universal DNN approach that was shown to systematically outperform the leading GBDT packages (e.g., XGBoost (Chen & Guestrin, 2016)). As additional evidence, a large number of Kaggle ML competitions with tabular data are still won by the shallow GBDT methods (Harasymiv, 2015). Overall, at the moment, there is no dominant deep learning solution for tabular data problems, and we aim to reduce this gap by our paper.

Specific DNN for tabular data. While a number of prior works propose architectures designed for tabular data (Ke et al., 2018; Shavitt & Segal, 2018), they mostly do not compare with the properly tuned GBDT implementations, which are the most appropriate baselines. The recent preprint (Ke et al., 2018) reports the marginal improvement over GBDT with default parameters, but in our experiments, the baseline performance is much higher. To the best of our knowledge, our approach is the first to consistently outperform the tuned GBDTs over a large number of datasets.













# Using deep neural network with small dataset to predict material defects.
Materials & Design, Volume 162, 15 January 2019, Pages 300-310

Large neural nets trained on relatively small datasets can overfit the training data.


However, DNN trained by conventional methods with small datasets commonly shows worse performance than traditional machine learning methods, e.g. shallow neural network and support vector machine. This inherent limitation prevented the wide adoption of DNN in material study because collecting and assembling big dataset in material science is a challenge.

It is found that a pre-trained and fine-tuned DNN shows better generalization performance over shallow neural network, support vector machine, and DNN trained by conventional methods. The trained DNN transforms scattered experimental data points into a map of high accuracy in high-dimensional chemistry and processing parameters space. Though DNN with big datasets is the optimal solution, DNN with small datasets and pre-training can be a reasonable choice when big datasets are unavailable in material study.




# Self-Normalizing Neural Networks
Klambauer et al. 1706.02515


success stories of Deep Learning with standard feed-forward neural networks (FNNs) are rare. FNNs that perform well are typically shallow and, therefore cannot exploit many levels of abstract representations.

We compared SNNs on (a) 121 tasks from the UCI machine learning repository, on (b) drug discovery benchmarks, and on (c) astronomy tasks with standard FNNs, and other machine learning methods such as random forests and support vector machines. 

 For FNNs we considered (i) ReLU networks without normalization, (ii) batch normalization, (iii) layer normalization, (iv) weight normalization, (v) highway networks, and (vi) residual networks. SNNs significantly outperformed all competing FNN methods at 121 UCI tasks, outperformed all competing methods at the Tox21 dataset, and set a new record at an astronomy data set. The winning SNN architectures are often very deep. Implementations are available at: github.com/bioinf-jku/SNNs.
 
 However, looking at Kaggle challenges that are not related to vision or sequential tasks, gradient boosting, random forests, or support vector machines (SVMs) are winning most of the competitions. Deep Learning is notably absent, and for the few cases where FNNs won, they are shallow. For example, the HIGGS challenge, the Merck Molecular Activity challenge, and the Tox21 Data challenge were all won by FNNs with at most four hidden layers. Surprisingly, it is hard to find success stories with FNNs that have many hidden layers, though they would allow for different levels of abstract representations of the input [3].


To robustly train very deep CNNs, batch normalization evolved into a standard to normalize neuron activations to zero mean and unit variance [20]. Layer normalization [2] also ensures zero mean and unit variance, while weight normalization [32] ensures zero mean and unit variance if in the previous layer the activations have zero mean and unit variance. However, training with normalization techniques is perturbed by stochastic gradient descent (SGD), stochastic regularization (like dropout), and the estimation of the normalization parameters.


In contrast, FNNs trained with normalization techniques suffer from these perturbations and have high variance in the training error (see Figure 1). This high variance hinders learning and slows it down. Furthermore, strong regularization, such as dropout, is not possible as it would further increase the variance which in turn would lead to divergence of the learning process. We believe that this sensitivity to perturbations is the reason that FNNs are less successful than RNNs and CNNs.







# Regularization Learning Networks: Deep Learning for Tabular Datasets
Shavitt et Segal Neurips 2018

Despite their impressive performance, Deep Neural Networks (DNNs) typically underperform Gradient Boosting Trees (GBTs) on many tabular-dataset learning tasks. 

Here, we introduce Regularization Learning Networks (RLNs), which overcome this challenge by introducing an efficient hyperparameter tuning scheme which minimizes a new Counterfactual Loss. 

Our results show that RLNs significantly improve DNNs on tabular datasets, and achieve comparable results to GBTs, with the best performance achieved with an ensemble that combines GBTs and RLNs.





# dropout


 Nitish Srivastava,  Hinton  [21]  [23]  proposed  the  method  of  Dropout  to prevent  over-fitting,  effectively  reducing  the parameters of the full connection layer, and solve the problem of insufficient samples.
 
 

Large neural nets trained on relatively small datasets can overfit the training data.

This has the effect of the model learning the statistical noise in the training data, which results in poor performance when the model is evaluated on new data, e.g. a test dataset. Generalization error increases due to overfitting.

One approach to reduce overfitting is to fit all possible different neural networks on the same dataset and to average the predictions from each model. This is not feasible in practice, and can be approximated using a small collection of different models, called an ensemble.



# Small dataset in deep


Neural networks are the basic building blocks of Deep learning models. However, Deep neural networks have millions of parameters to learn and this means we need a lot of iterations before we find the optimum values. If we have small data, running a large number of iteration can result in overfitting. Large dataset helps us avoid overfitting and generalizes better as it captures the inherent data distribution more effectively.

Here are a few important factors which influence the network optimization process:

  1.  Optimization Algorithm: Gradient descent is the most popular optimization algorithm used for neural networks. The algorithm performance directly depends on the size of the training data. We may try updating the weights with a smaller training set(stochastic gradient descent being the extreme case when we do updates with single data point) which makes the training process fast however the updates have larger fluctuation. Training with the whole dataset makes training computationally expensive and slow. Adam, RMSprop, Adagrad, Stochastic Gradient descent are a few variations of gradient descent which optimizes the gradient update process and improves model performance

2 Loss function: Loss function also plays a crucial role in the optimization process and carefully selected loss function can help in improving the training process. Hinge loss is one such example which makes training with small dataset possible.

3.Parameter initialization: The initial state of the parameters greatly influences the optimization process. Poorly chosen initialization values can result in issues of divergence and getting stuck at saddle points or local minimum. Also, this increases the requirement of the training data for the training process.


4. Data size: Data size is a very crucial part of training neural networks. Larger datasets can help us better learn model parameters and improve the optimization process and imparts generalization.



1. Transfer learning:

Transfer learning refers to the approach of using the learning from one task on to another task without the requirement of learning from scratch. It directly addresses the smart parameter initialization point for training neural networks. This technique has been widely used in computer vision tasks and has been instrumental in the wide application of deep learning in the industry.



==> Old/Old_main/exclus_10_21.tex <==
% We will make two important distinctions with our previous example. There is not a close form expression of a neural network given a set of hyper-parameters, we will use gradient descent to learn the weights. Previously, we did not use MLR to explore the entire space of weights for linear models. We restricted ourselves to weights which were solutions of the minimization of the \TempHP-penalized loss on the train set. Here, we want to explore freely the high-dimensional space of neuron weights in every possible directions. 

%  If we try to minimize the loss on the train set, the gradient direction is a mixture of both meaningful patterns and memorization, just as with our previous example. Disentangling the part of the improvement on the train loss which corresponds to generalization from the part corresponding to memorization is not obvious in general. Therefore, at each step of gradient descent, instead of trying to artificially skew the gradient in directions which memorize less, we want the update the weights such that at the next step of gradient descent, the direction of the gradient towards the steepest reduction of the train loss will naturally increase generalization much more than memorization in proportion. We do not want to reduce memorization, we want to reduce the capacity of the network to memorize.
 
 
%  set  afe toward a state where the next gradient towards the steepest reduction of the loss on the train set  towards 
 
%  Prophilactic approach
 
 
%  Conversely, since we want to identify the direction of steepest descent towards generalization, we need to disentangle from the gradient direction towards the steepest reduction of the loss on the train set the direction which increase the capacity of the neural network to memorize the train set. We do not want to prevent memorization during learning, 



% Our goal at each step of the gradient descent is to find the direction of steepest descent towards generalization.

% There is not a close form expression of a neural network given a set of hyper-parameters,we will use gradient descent to learn the weights. Our goal at each step of the gradient descent is to find the direction of steepest descent towards generalization. If we try to minimize the loss on the train set, the gradient direction contains both meaningful patterns and memorization, just as with our previous example. If we use MLR to tune 


% GD is a greedy procedure which selects the direction of steepest descent. When used to minimize the train loss, the gradient direction contains both meaningful patterns and memorization, just as with our previous example. We do not want to use MLR to optimize the amount of weight decay during training to skew the updates while aiming to minimize the train loss. Our goal is to disentangle the part of the improvement on the train loss which corresponds to generalization from the part corresponding to memorization to get the direction which actually  update the weights (W,L) of the NN at each step of gradient descent in the direction which increases \TempGen the most.

%  GD is a greedy procedure which selects the direction of steepest descent. Here, at each gradient update,  The gradient direction corresponding to the loss contains both meaningful patterns and memorization. Disentangling the part of the improvement on the train loss which corresponds to generalization from the part corresponding to memorization is not obvious in general. 

% Again, departing from other methods, our goal here is not to skew the weight updates towards direction which lead to increased generalization, at each step using L2 regularization 

% Therefore, extending our ridge example to neural network does not mean using the MLR criterion to pick the amount of L2 weight decay

% The equivalent of Ridge penalization for neural networks is L2 penalization/weight decay applied during training. However the goal we set ourselves is to learn the weights of the neural network by directly optimizing generalization, not just skew the gradient updates in a direction which generalizes more through explicit regularization. More precisely, when we try to 


% \subsection{Plan}
% % Objectif en Deep Learning: 

% % Idee MLR: quantifier la memorisation d'un modele et la minimiser pendant l'entrainement

% \paragraph{Context/Constat (Problématique).}

% Probleme du deep: training = memorisation +generalization entangled. How to favoriser generalization a la memomrisation durant le training.


% %\paragraph{Constat (Problématique).}
% ///
% /// On introduit les deux concepts et  //

% //La mémorisation on en veut pas parce que ça abime la robustesse mais aussi ça que ça abime la généralisation en prenant sa place.// 


% Problématique tel que nous on la formule: Donc c'est un bon objectif de minimiser la mémorisation durant l'entraînement (Chaque iteration doit etre la plus utile/efficace possible "Make it count"). //////UNderstainf deep learning requires rethinking////

% Jusqu'à présent, on peut pas acceder cette quantité durant l'entrainement. Les gens ont proposé/utilisé des proxy (eg.tel la variance du modèle), ils sont imparfait car quand on les minimise certe on réduit la mémorisation mais on atteint pas son minimum. 
% Fin Constat (Problématique)
% ///

% \paragraph{Notre Objectif.}

% MLR objectif d'améliorer le tradeoff entre memorization et généralization.

% Fondement de MLR: Et pour se faire notre parti pris/principe fondamentale: c'est de quantifier la memorisation en utilisant le train set, pour la minimiser durant l'apprentissage.\\

% ///
% \paragraph{Presentation du principe/methode MLR.}\\
% \subsection{Démonstration}

% f, w, Loss, (jeu train, jeu test)

% Entrainé un modèle 
% what = argmin w de L(w, train)
% G = L(what, test)
% M = L(what, test) - L(what, train)

% Régularisé pour une autre loss $L$,
% L(omega)(w, train)

% %bilevel optim ci-dessous
% what(omega) = argmin \{L(omega)(w, train)\}
% omegahat = argmin (omega) \{ L(what(omega), test)\}

% MLR Critère: 
% omegaMLR = argmin (omega) \{ L(omega)(w, train)- L(omega)(w, permut train)\}
 
%  MLR loss: on sépare w = (w1, w2) (rq: w1 les poids des couche cachée, w2 les poids de la couche de sortie)
%  w2hat(omega) = argmin w2 \{L(omega)(w1, w2, train)\}
 
 
%  w2hat est une fct de w1, omega et train: (la forme close du ridge)
%  w2hat(omega, w1, train) 
 
%  MLR: (w1MLR, omegaMLR) = argmin (w1, omega) L(w1,  w2hat(omega, w1, train), train) - L(w1,  w2hat(omega, w1, permut train) , permut train)
%  Donc on optimise les poids à l'intérieur, pas l'hyper paramètre omega: C'est pas du biniveau on optimise w1 en même temps que omega. pas l'un dans l'autre.
 
%  Etape suivante : 
%  MLR: (w1MLR, omegaMLR) = argmin (w1, omega) L(w1,  w2hat(omega, w1, train), train) + |1 - L(w1,  w2hat(omega, w1, permut train) , permut train)|
 
% Rq : La loss de  w2hat(omega) n'est pas celle de w1, omega, obvious pour la classif, Lomega c'est le risque empirique pour les coefs du ridge, L c'est la cross entropie.
 
 
%  Qui est w1, qui est w2:
%  Quelle est la forme de w, définisse WB, f(w)
 
%  Our approach is to separate the weights of the architecture in two sets, one being dedicated to fit the permuted labels, the other being dedicated to prevent them from doing so. Precisely, the weights of the output layer are tasked with fitting the target given the output of the last hidden layer as well as possible. The weights on the hidden layer are tasked with producing an activation which makes that task as easy as possible with true labels, and as hard as possible with permuted labels.
 
%  Maintenant
 
%  Qui est L(omega)(w1,w2, train) pour identifier  w2hat(omega, w1, train): L(omega) c'est le risque quadratique de l'estimateur ridge, donc w2hat(omega, w1, train) admet une forme close.
%   To avoid solving a bi-level optimization, we leverage the fact that the inner part of our nested optimization process admits a closed-form solution. This closed-form is directly the solution of the following optimization problem: fit the target (true or permuted) given the activation of the last hidden layer. Since it is differentiable, the loss can be back-propagated through the closed-form to the weights of the hidden layers. And since it is a linear function of the target being fitted, it can efficiently be computed for both true and permuted targets.

% De plus pourquoi la pénalisation et l'introduction de omega? Pour well defined le tradeoff
% Depending on the activation values, the width of the last hidden layer, and the size of the batch, if we use the closed-form of the OLS, we could get into situations where it is either too easy or too hard to fit the targets, (for both true and permuted labels), which would lead to gradient vanishing. To ensure the trade-off between these two goals (fitting true labels, not fitting permuted labels) is correctly set, we use instead the ridge closed-form. That way, through the ridge regularization parameter  we can control how difficult it is to fit targets.




%  Dithering.
% Dithering can be used to regularize. Increasing the magnitude of the dithering increases regularization up to a point. However, If the noise level of the dithering goes above a certain threshold howether, it will skew the gradient in a random direction so much at each step that instability will prevent convergence all together.

% To avoid this drawback, we want to enforce gradient vanishing with respect to the random noise added to the target. To do so, our solution is to use the residuals of a standard gaussian white noise fitted using the aforementioned close-form. Indeed, if we fit random noise using a linear closed-form, the resulting residuals correspond to random variations that cannot be minimized through that closed-form. As such, even if the residuals have a strong impact on the loss, they will have a low impact on the gradient of that loss, meaning we can increase the magnitude of that random noise without skewing the gradient as much as we would with regular gaussian white noise. This is how we came up with the structured dithering ingredient.



 
% % Le résultat du papier théorique |omegahat - omegaMLR | petit descend vite, 

% % In over-parametrized models, there are a lot of possible directions to explore to reduce training error via Gradient Descent. GD is a greedy procedure which selects the direction of steepest descent. The gradient direction corresponding to the quadratic loss contains both meaningful patterns and memorization. Disentangling the part of the improvement on the train loss which corresponds to generalization from the part corresponding to memorization is not obvious in general.

% % The tradeoff between generalization and memorization is trivial when learning on randomly permuted labels (like in Zhou et al). Any improvement by gradient iteration corresponds exclusively to memorization. 

% % Perf Intercept (train) - Perf modèle (train) = M + G
% % Dans le cas label permuté, G = 0 donc M/(M+G) = 1

% % Another quantifiable edge case, saturating the regularization parameter of the Ridge intercept. When lambda = +inf, Perf Intercept (train) - Perf modèle (train) = 0. This is true with origin and permuted labels. However, for other values of lambda Perf Intercept (train) - Perf modèle (train) and Perf Intercept (Permuted train) - Perf modèle (Permuted train) are not necessarily equal. Our first big assumption is the following: maximizing that difference leads to maximizing G. Theoretical justification of this claim is far from trivial and beyond the scope of this paper, and available in another paper called. The theoretical backing of this claim.

% % On a donc un premier cas, le modèle Ridge ou on peut quantifier la mémorisation comme une fonction du train et de paramètres du modèle. , pour un modèle spécifique (le Ridge). 


% \paragraph{MLR method applied to Neural Networks.}
% Dans le cas précédent, MLR n'est pas utilisé pour choisir la meilleure combinaison de poids parmi tous les modèles linéaires possibles, c'est un critère pour choisir le meilleur proxy parmi toutes les fonctions de pertes à minimiser parmi celles du ridge. Il s'agit en fait d'un pb d'optimisation bi-niveau dont le niveau intérieur dispose d'une forme explicite et dérivable.

% - On reprend l'expression mais en l'écrivant avec le weight decay du Ridge. 
% - On retombe dans une selection d'HP et pas du tout dans notre objectif initiale, directement optimiser le gradient selon le tradeoff generalization/mémorisation. 

% - On veut pas optimiser la diff entre les deux, on veut optimiser la capacité à optimiser la diff. 
% (solution naturelle qui marche pas Yann Lecun)

% - Découpage bi level 

% Dans le cadre du Ridge, la forme close supprime la distinction entre proxy et 

% On veut pas améliorer le trade-off Mem Gen on veut choisir un point ou le tradeoff est encore plus favorable 

% On veut optimiser la capacité à mémoriser: MLR(théta+1) - MLR(Théta)

% A norme de gradient constante, on veut que l'amélioration de la loss quand on fait une update avec les vrai label soit le plus grand possible comparé au gain avec des labels permutés. 

% L'idée Yann lecun c'est d'exprimer les gains en fct des gradients, d'exprimer les gradients en fct des poids et d'optimiser 

% Forward Backward = d(Forward)(omega1, omega2)  = oméga'
% Bilevel = d F(omega+omega')  = omega''
% d F(omega+d(Forward)(omega))

% d ((F(x1 + d(F(x_1,x_2)/d(x1)), x2)) - F(x1 x2) ) / d(x2)


% d'un update pour la loss pas permuté soit le plus grand possible comparé au gain dans le cas permuté.




% L'analogie naturelle entre le lambda du ridge et un réseau de neurone, c'est le coefficient de weight decay.
% Chaque coefficient de weight decay est associée à une fonction de perte pénalisée, et minimiser cette fonction est un proxy pour optimiser la généralisation. Utiliser MLR pour choisir le meilleur HP, c'est choisir le meilleur proxy. Comme dit précédemment, ce n'est pas notre objectif. On ne veut pas choisir parmi des modèles appris sur différentes loss. 

% Notre but est qu'a chaque etape de l'entrainement d'un modele, on maximise le ratio generalization/memorisation.

% on veut choisir pour un modèle la meilleure update pour améliorer l'objectif.


% On veut un chemin d'entrainement where a chaque iteration, il est plus facile de generaliser que de memoriser.


% Pour le ridge on dispose d'une expression explicite et dérivable en fonction de lambda de l'optimum pour le train et pour le train permuté. Ce qui permet d'optimiser directement la différence en fct de lambda. 



% Pour les réseaux de neurones ce n'est pas le cas. Une première approche naive ce serait de faire une grille sur les paramètres de régularisation, de faire un apprentissage complet des poids selon les deux objectifs et de choisir les HP qui maximisent la différence. 

% Ce n'est pas du tout notre objectif. On se ramènerai alors à un critère (type AIC BIC), 


% Le travail de ce papier maintenant c'est de leverage ce résultat pour des modèles plus complexes et plus puissants, Neural networks. 

% La comparaison entre gradient quand on améliore sur donnée permutée et gradient sur donnée

% Le travail de ce papier maintenant c'est de leverage ce résultat pour des modèles plus complexes et plus puissants, Neural networks. 

% La première difficulté, c'est que l'on ne dispose pas d'une expression directe des poids d'un réseau en fonction de l'objectif et des hyper-paramètres. 

% Dans ces cas là, , où le gradient est de grande dimension. Il ne suffit plus alors de choisir le sens mais aussi la direction à chaque étape qui va améliorer le trade off. 

% La première solution ce serait de constuire deux réseau avec deux sets de poids, et d'optimiser conjointement à chaque étape les paramètres de régularisation. On a alors deux quantités


% Perte quadratic (OLS), probleme gradient vanishing

% Pour le ridge, on dispose d'une forme close (no bilevel optimization). Ainsi le modèle ne dépend que d'un seul paramètre, lambda, tous les autres poids du modèle étant conditionnés. Pour un réseau de neurone, le gradient est multi-dimensionnel, 


% O
% Naivement, on voudrait apprendre en // deux réseaux et 

% Pour un réseau de neurone overparametré de paramètres oméga, la capacité à surapprendre m^me sur des donnés permutés (toujours le résultat de Zhou et al) implique que
% Perf Intercept (train) - Perf modèle (train)(Omega) = Perf Intercept (Permut train) - Perf modèle (permut train)(Omega prime) = 1. 

% Donc apprendre deux 

% Réseau 












% In the linear regression model, \cite{BKK-reg} proved that the permutation correction to the train loss allows to build a new estimator of the true generalization error. In other word, the permutation correction corresponds to the memorization part of the train objective and substracting it from the train loss leaves us only with the generalization part.


% Comment on fait la quantification de la memorisation. 



% In the seminal article (Understanding...) le juge de paix pour montrer la memorisation, c'est de regarder la perf de train dans des cas sans lien entre y et X. Nous reprenons à notre compte le postulat: tout apprentissage sur le train est du à la memorisation quand on utilise permute les labels. Ca permet d'avoir une baseline pour discriminer entre généralisation et mem: dans le cas permuté, on a nécessairement 100 pourcent de mémorisation. C'est quantifiable.





% In over-parametrized models, there are a lot of possible directions to explore to reduce training error via Gradient Descent. GD is a greedy procedure which selects the direction of steepest descent. The gradient direction corresponding to the quadratic loss contains both meaningful patterns and memorization.
% In one case, this tradeoff is trivially quantified: when learning on randomly permuted labels (like in Zhou et al). the direction of the gradient corresponds exclusively to improvement by memorization, 



% By default, it is not clear which part of the improvement on train loss is generalization and which part is memorization.


% % We can start by a simple case where quantifying memorisation is trivial. When learning on randomly permuted labels (like in Zhou et al) the direction of the gradient corresponds exclusively to improvement by memorization. generalization on train loss is due to generalization. 


% When training on permuted targets (that means there is nothing to learn beyond the expectation of ), an over-parameterized neural network is able to outperform the intercept model in terms of train loss, but only by memorizing the train set. The gradient direction corresponding to the quadratic loss contains only memorization.





% Premier Morceau:
% In over-parametrized models, there are a lot of possible directions to explore to reduce training error via Gradient Descent. GD is a greedy procedure which selects the direction of steepest descent. The gradient direction corresponding to the quadratic loss contains both meaningful patterns and memorization.\\

% When training on permuted targets (that means there is nothing to learn beyond the expectation of ), an over-parameterized neural network is able to outperform the intercept model in terms of train loss, but only by memorizing the train set. The gradient direction corresponding to the quadratic loss contains only memorization.

% MAL CONSTRUIT: Based on those observations, our goal when we replace the quadratic loss by the MLR loss is to maximize the proportion of meaningful patterns of the steepest direction of descent at each GD step during training. At each gradient step, we want to minimize the ability of the neural network to use memorization to improve the train loss, while preserving its ability to do so through generalization.

% Directions of gradient descent on permuted targets increase the ability of the NN to overfit permuted labels. By correcting the gradient for those memorization directions we also reduce the ability of NN to overfit true labels. This does not reduce the ability of the NN to increase generalization when fitting true labels.





% Second Morceau
% Now our motivation is to use the Ridge closed-form to perform this gradient correction: Minimizing the ability of the NN to increase memorization (i.e. fitting permuted labels) is a bi-level optimization problem, with two antagonistic goals. We want to address it in a tractable, efficient and differentiable manner. See the following reference for a natural approach to this bi-level optimization problem which sadly did not work in our case: Drucker et Le Cun. Improving generalization performance using double back propagation. IEEE transactions on Neural Networks (1992).

% So we had to look for an alternative approach to solve this problem.

% Our approach is to separate the weights of the architecture in two sets, one being dedicated to fit the permuted labels, the other being dedicated to prevent them from doing so. Precisely, the weights of the output layer are tasked with fitting the target given the output of the last hidden layer as well as possible. The weights on the hidden layer are tasked with producing an activation which makes that task as easy as possible with true labels, and as hard as possible with permuted labels.


% Second leap of faith (mostly because it would be far too long and tedious to explain why, for specific technical reasons,all the approaches which feel more natural we could find, either : -are very inefficient, -perform poorly, -or do not work at all.): To avoid solving a bi-level optimization, we leverage the fact that the inner part of our nested optimization process admits a closed-form solution. This closed-form is directly the solution of the following optimization problem: fit the target (true or permuted) given the activation of the last hidden layer. Since it is differentiable, the loss can be back-propagated through the closed-form to the weights of the hidden layers. And since it is a linear function of the target being fitted, it can efficiently be computed for both true and permuted targets.

% Depending on the activation values, the width of the last hidden layer, and the size of the batch, if we use the closed-form of the OLS, we could get into situations where it is either too easy or too hard to fit the targets, (for both true and permuted labels), which would lead to gradient vanishing. To ensure the trade-off between these two goals (fitting true labels, not fitting permuted labels) is correctly set, we use instead the ridge closed-form. That way, through the ridge regularization parameter  we can control how difficult it is to fit targets.

% \\
% ///
% Conséquence mode de fonctionnement, impact sur le deep
 
%  ////
 

% /// On introduit les deux concepts et on dit que l'un c'est bien et pourquoi et l'autre c'est mal et pourquoi. On dit que ya un tradeoff entre les deux, et que les différents algos sont à des endroits différents du tradeoff. Zhou UNderstainf deep learning requires rethinking // 

% Définisse bien les deux concepts. Tous les algos généralise pas autant et mémorise pas autant et certains font bien les deux ensemble et d'autres moins bien. Quand choisi un méthode et ces hyperparamètres onse pose à un 



% explicite minimise directement la quantité et pas une autre qui aurait pour conséquence. 
% (minimise la mémorisation implicitement variance poids => memorisation) régularization explicite (memorization implicite ex ils quantifie la variance selon la norme des poids, proxy) et celle implicite (on quantifie pas la capacité à memoriser, on apprend d'une façon qui mémorisera en conséquence).


% argmin Memorisation 

% Argmin Var(Norm Beta) parce que Mem est une fonction positive et croissante de Var

% Mem(X1,X2,X3) 
% Var(X1,X2)

% Chercher des quantités qui varient 


% méthode de quantification discuter ce que ça change par rapport (cross validation des HP de régularization 


% On minisiser la mem. On y a pas accès, on propose des proxy où quand on les minimise on réduit la memorisation sans forcément la minimiser. 





% implicte c'est pas d'argmin. juste une conséquence.



% Objectif : MLR objectif d'améliorer le tradeoff entre memorization et généralization


% Dans le constat on a fait intervenir dans la  définition mathématique del la quantité "memorization" à la fois le train et le test. 

% Le fondement de notre méthode c'est de proposer une quantification qui soit uniquement exprimer à l'aide du train. Et donc pénalisable durant l'apprentissage. 

% Fondemennt : Notre fondement c'est de quantifier en utilisant le train uniquement le train la mémorization pour pouvoir la pénalizer pendant l'apprentissage.





% Pouvoir augmenter les perfs sur le test tout en réduisant la variance sur le train qui suit pas.



% \subsection{Motivation for our method}

% Based on those observations, our goal when we replace the quadratic loss by the MLR loss is to maximize the proportion of meaningful patterns of the steepest direction of descent at each GD step during training. At each gradient step, we want to minimize the ability of the neural network to use memorization to improve the train loss, while preserving its ability to do so through generalization.


% Definir dans le contexte memorization notre vision du truc steepest descent


% \subsection{Démonstration}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Rebuttal Old}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The rebuttal will be uploaded by tomorrow with completed values in Table 2.

% "Using Ridge closed-form on the last hidden layer of the FFNN already gives some significant improvement of the generalization performance (See the ablation study in Table 4). Sorry, my question here was on providing "motivation or intuition", beyond saying "much stronger regularisation than adding standard L2 weight regularisation to the loss". While I feel that your approach is certainly interesting, I do not feel that you provide enough evidence to support why MLR is a good idea."\\

% We have preliminary theoretical results which prove that a MLR neural network with 0 hidden layers ()(i.e. Ridge model with only parameter  being fitted through gradient descent on the MLR loss) admits better generalization performance than a Ridge model with  being fitted through gradient descent on the quadratic loss. The reason is that the MLR loss is a much better proxy for the true generalization error than the quadratic loss. We are currently studying the extension of these theoretical results to shallow neural networks (). These results will be part of another future paper covering the theoretical aspects of MLR. Afterwards, we will attempt to tackle deep networks (), which is a much more challenging case. But all of this is beyond the scope and the time frame of this paper.

% In the meantime, here is some more insight about how we currently understand the mechanisms behind MLR:

% When training on regular targets, an over-parameterized neural network can outperform the intercept model in terms of test loss by learning generalizable relations between observations and targets. However, since it is also able to memorize the training set, it will try to minimize the loss on the training set using both memorization and generalization.
% In over-parametrized models, there are a lot of possible directions to explore to reduce training error via Gradient Descent. GD is a greedy procedure which selects the direction of steepest descent. The gradient direction corresponding to the quadratic loss contains both meaningful patterns and memorization.
% When training on permuted targets (that means there is nothing to learn beyond the expectation of ), an over-parameterized neural network is able to outperform the intercept model in terms of train loss, but only by memorizing the train set. The gradient direction corresponding to the quadratic loss contains only memorization.


% Based on those observations, our goal when we replace the quadratic loss by the MLR loss is to maximize the proportion of meaningful patterns of the steepest direction of descent at each GD step during training. At each gradient step, we want to minimize the ability of the neural network to use memorization to improve the train loss, while preserving its ability to do so through generalization.

% The leap of faith in our method (until theoretical results are made available...):

% Directions of gradient descent on permuted targets increase the ability of the NN to overfit permuted labels. By correcting the gradient for those memorization directions we also reduce the ability of NN to overfit true labels. This does not reduce the ability of the NN to increase generalization when fitting true labels.

% Now our motivation is to use the Ridge closed-form to perform this gradient correction: Minimizing the ability of the NN to increase memorization (i.e. fitting permuted labels) is a bi-level optimization problem, with two antagonistic goals. We want to address it in a tractable, efficient and differentiable manner. See the following reference for a natural approach to this bi-level optimization problem which sadly did not work in our case: Drucker et Le Cun. Improving generalization performance using double back propagation. IEEE transactions on Neural Networks (1992).

% So we had to look for an alternative approach to solve this problem.

% Our approach is to separate the weights of the architecture in two sets, one being dedicated to fit the permuted labels, the other being dedicated to prevent them from doing so. Precisely, the weights of the output layer are tasked with fitting the target given the output of the last hidden layer as well as possible. The weights on the hidden layer are tasked with producing an activation which makes that task as easy as possible with true labels, and as hard as possible with permuted labels.

% Second leap of faith (mostly because it would be far too long and tedious to explain why, for specific technical reasons,all the approaches which feel more natural we could find, either : -are very inefficient, -perform poorly, -or do not work at all.): To avoid solving a bi-level optimization, we leverage the fact that the inner part of our nested optimization process admits a closed-form solution. This closed-form is directly the solution of the following optimization problem: fit the target (true or permuted) given the activation of the last hidden layer. Since it is differentiable, the loss can be back-propagated through the closed-form to the weights of the hidden layers. And since it is a linear function of the target being fitted, it can efficiently be computed for both true and permuted targets.

% Depending on the activation values, the width of the last hidden layer, and the size of the batch, if we use the closed-form of the OLS, we could get into situations where it is either too easy or too hard to fit the targets, (for both true and permuted labels), which would lead to gradient vanishing. To ensure the trade-off between these two goals (fitting true labels, not fitting permuted labels) is correctly set, we use instead the ridge closed-form. That way, through the ridge regularization parameter  we can control how difficult it is to fit targets.

% This closed-form can also be used to improve dithering:

% Dithering can be used to regularize. Increasing the magnitude of the dithering increases regularization up to a point. However, If the noise level of the dithering goes above a certain threshold howether, it will skew the gradient in a random direction so much at each step that instability will prevent convergence all together.

% To avoid this drawback, we want to enforce gradient vanishing with respect to the random noise added to the target. To do so, our solution is to use the residuals of a standard gaussian white noise fitted using the aforementioned close-form. Indeed, if we fit random noise using a linear closed-form, the resulting residuals correspond to random variations that cannot be minimized through that closed-form. As such, even if the residuals have a strong impact on the loss, they will have a low impact on the gradient of that loss, meaning we can increase the magnitude of that random noise without skewing the gradient as much as we would with regular gaussian white noise. This is how we came up with the structured dithering ingredient.

%Our method outperforms the gold standard in terms of Friedman rank for regression and classification whatever the number of samples, of features, the type of features or the domain of the datasets.. 

%Our method proved more reliable than usual methods (Ensemble, \SVM, Boosting, Linear Regression, $etc.$ ) including the gold standards \RF{} and \GBDT{}, on our aggregated benchmark (UCI+ Kaggle).
% \textcolor{red}{It consistently ranked in the top \textcolor{red}{3 or 5} on all datasets in terms of $\Rdeux${} for regression or Accuracy and \AUC{} for binary classification,} whatever the number of samples, of features, the type of features or the domain of the datasets. 

%For $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. Moreover, this value is not too large as it preserves GPU parallelization. Consequently, $T=16$ has little to no impact on the runtime of our method. 

%We propose several models based on \FFNN{} trained with the \MLR{} loss:\\

Appendix for more details.
%We added $Value$ datasets by repeating the same process on Kaggle\cite{} using the tags with "task": "regression" and "format" : ".csv",".xls". \textcolor{red}{We repeated the same process for classification \sout{and ended up with $Value$ datasets well suited for tabular classification.}}
%See Table \ref{} in the Appendix for the list of violated rules for each available dataset. \textcolor{red}{In summary, we have ? regression datasets and ? classification datasets.}
%\textcolor{red}{B: Mauvais argument, il y a déjà des gens qui sont passés derrière et qui ont corrigés le bench. Plutôt dire que pour des raisons de temps de calcul, on a préféré faire moins de jeux de données, mais remanier en plus propre et surtout avec 10 découpages train test par expérience.}
%Although \cite{Delgado14a} already built a benchmark based on the UCI repository, their methodology presents some flaws \cite{Wainberg2016}. 
%Hence, we went back to the exhaustive list of $Value$ available datasets tagged as regression in the UCI repository and curated it through  .
%Hence, we started anew and curated the UCI repository through a set of rules detailed in the appendix ($e.g.$ discard empty or \textbf{duplicate} datasets, times series, missing target, non $i.i.d.$ samples, text format, $etc$.). After an exhaustive screening of the $Value$ available datasets tagged as regression, we were left with $Value$ datasets. We added $Value$ datasets by repeating the same process on Kaggle\cite{} using the tags with "task": "regression" and "format" : ".csv",".xls". \textcolor{red}{We repeated the same process for classification \sout{and ended up with $Value$ datasets well suited for tabular classification.}}
%See Table \ref{} in the Appendix for the list of violated rules for each available dataset. \textcolor{red}{In summary, we have ? regression datasets and ? classification datasets.}
%Contrarily to classification, there are not that many publicly available well-known datasets which are actually well suited for a tabular regression benchmark. 

%\textcolor{red}{We use a 80/20 ratio for each of the 10 $train$/$test$ splits of the dataset,} with a different seed and no stratification scheme. 
%We repeated $10$ times a $80:20$ train/test split of the data with a different seed and no stratification scheme. 

%\texttt{Fast.ai} \cite{Howard2020}, \Catboost{} \cite{Prokhorenkova2018}, \XGBoost{} \cite{guestrin2016} and \lightgbm{} \cite{Ke2017}. 
%For all our proposed \MLR-architectures, we run its standard equivalent in \DL{} (denoted as \RNN2 for \MLRb{} as an example). 
%In the rest of the paper, we only display the main classes of methods: \MLR{}, \GBDT{} (\XGB, \XGBoost, \Catboost, \lightgbm), \RF{} (\RF{} and \XRF), \SVM{}, \RNN{} (\texttt{Fast.ai} and \MLP), \MARS{}, \GLM{} (Generalized Linear Models: LSE, Elastic Net, Ridge, LASSO, Logistic regression), \TREE{} (CART, XCART) and the \Baseline{} (intercept for regression and class probabilities for classification).
%The exhaustive list of methods and results is provided in the supplementary material.
%each architecture we tested for MLR, we also ran a standard NN with the same architecture and parameters.

% \begin{table}[!hp]
% \caption{Ablation Study in Regression. %\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.}
% }
% \label{tab:ablation}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|}
% \hline
% Step  &  Mean $\Rdeux$  & Bagging $\Rdeux$ \\
% \hline
% \hline
% \FFNN   & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% \hline
% + Ridge  & $ 0.32  \pm  0.17 $ & $ 0.39  \pm  0.12 $ \\
% \hline
% + Ridge + Struct. Dithering   & $ 0.32  \pm  0.16 $ & $ 0.40  \pm  0.11 $ \\
% \hline
% + Ridge + Permut.  & $ 0.36  \pm  0.11 $ & $ 0.43  \pm  0.07 $ \\
% \hline
% \MLR{}  & $ 0.37  \pm  0.10 $ & $ 0.43  \pm  0.07 $ \\
% \hline
% \end{tabular}
% \end{table}

%\textcolor{red}{$\ast$}
%\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.

% NN2  & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% RidgeNN2  & $ 0.321  \pm  0.081 $ & $ 0.394  \pm  0.052 $ \\
% RidgeSpectral2  & $ 0.323  \pm  0.075 $ & $ 0.400  \pm  0.048 $ \\
% RidgePermut2  & $ 0.364  \pm  0.050 $ & $ 0.432  \pm  0.035 $ \\
% RidgePermutSpectral2  & $ 0.371  \pm  0.024 $ & $ 0.433  \pm  0.000 $ \\


% The following is a summary of our findings, we refer the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance.
% %See the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance. 
% The generic values ($\tilde{\sigma} = 0.03$ and $T=16$) for the \dither{} and the number of permutations hyperparameters yield consistently good results overall. The \dither{} parameter admits an optimal value (see Figure ? in the Appendix) which seems to correspond to the standard deviation of the target noise. As soon as $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. In addition, when $T=16$, GPU parallelization is still preserved.
% %For $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. Moreover, this value is not too large as it preserves GPU parallelization. Consequently, $T=16$ has little to no impact on the runtime of our method. 
% Recall that the Ridge parameter $\bla$ is trained alongside the weights of the \FFNN{} architecture and the initial value $\bla_{init}$ is fixed by the heuristic choice (\ref{lambdainiti}). Our investigations (see Figure \ref{?}) reveals that this choice is close to the optimal oracle choice on the test set. We can also see that the runtime overhead cost of replacing a matrix multiplication with a matrix inversion depends only linearly on the width $J$ and the batch size $\bs$, which are fixed in our method.

% We perform 10 repetitions of our ablation study on 3 datasets which are representative of all the 

% The improvement of each ingredient of the \MLR{} method is statistically significant 

%the 3 components of \MLR{} are Ridge regularization, structure dithering and random permutations.
%Ridge regularization is the essential component of the method as both structured dithering and random permutations are follow-up steps which require the last layer to be a close form. rely on the Ridge close-form. 
% Recall that Ridge regularization is the essential component of the method as it provides a closed form representation of the last hidden layer on which we can conveniently apply the follow-up treatments: structured dithering and/or random permutations. 

%Permutations and structured dithering nous fait battre l'etat de l'art.

 %Note also that bagging cannot help it overcome its overwhelming flaws. 
%Applying Ridge on the last hidden layer allows the \FFNN{} to learn but its generalization performance is still far behind the gold standard \RF. 



%the \MLR{} method attains a significantly higher $R^2$-score.  better higher performance


%Clearly, using permutations improves the performance much further than Structured Dithering, however, they are both useful. Without bagging, a single \NN{} can reach or even outperform the gold-standard methods on most datasets (see the following section for details). Furthermore, the improvement yielded by using bagging($0.062$ is still of the same magnitude as the one when we started ($0.073$). 
%This means these two ingredients are not just simple variance reduction techniques but actually generate more sophisticated models.

%This means these two ingredients are not simply improving the robustness of the model or reduce its variance, but contribute to learning more complex yet generalizable patterns even with such a large network, over so few samples. 




%Interestingly, the impact of the other hyperparameters in our method is sometimes strikingly different from what is usually observed in the general deep learning framework. With our method, using wider architecture and bigger batch size is always better. See Figures \ref{} and \ref{}. 



% \begin{table}[!hp]
% \caption{\textbf{Performances of the $10$ best methods} for the regression task on our benchmark. \Pa, \Pb, \Pc: the number of datasets a model achieves 90\%, 95\%, 98\% or more of the maximum test $\Rdeux$-score respectively, divided by the total number of datasets. \PMA: average percentage of the maximum test $\Rdeux$-score.}
% \label{tab:perfR2_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean $\Rdeux$-score          & \Pa              & \Pb              & \PMA                          \\ \hline
% \hline
% \hline
% \BMLR{}  & $\bm{3.50 \pm 2.38}$ & \textbf{$0.67 \pm 0.25$} & \textbf{$0.89 \pm 0.32$} & \textbf{$0.72 \pm 0.46$} & \textbf{$0.92 \pm 0.17 $}\\
% \BMLRb{}  & $ 3.94 \pm 2.84$ & $0.67 \pm 0.26$ & $0.83 \pm 0.38$ & $0.61 \pm 0.50$ & $0.88 \pm 0.28 $\\
% \BMLRa{}  & $ 5.50 \pm 4.51$ & $0.66 \pm 0.24$ & $0.83 \pm 0.38$ & $0.67 \pm 0.49$ & $0.92 \pm 0.13 $\\
% \MLRc  & $ 7.33 \pm 3.80$ & $0.65 \pm 0.27$ & $0.67 \pm 0.49$ & $0.44 \pm 0.51$ & $0.83 \pm 0.37 $\\
% \MLRb  & $ 7.94 \pm 3.83$ & $0.65 \pm 0.26$ & $0.72 \pm 0.46$ & $0.44 \pm 0.51$ & $0.86 \pm 0.26 $\\
% \MLRa   & $ 9.06 \pm 4.49$ & $0.64 \pm 0.25$ & $0.78 \pm 0.43$ & $0.44 \pm 0.51$ & $0.81 \pm 0.47 $\\
% \hline
% \RF   & $ 7.11 \pm 6.57$ & $0.64 \pm 0.28$ & $0.67 \pm 0.49$ & $0.50 \pm 0.51$ & $0.68 \pm 1.01 $\\
% \XRF  & $ 7.56 \pm 5.82$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.50 \pm 0.51$ & $0.68 \pm 0.93 $\\
% \hline
% \XGB  & $ 7.22 \pm 6.68$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.67 \pm 0.49$ & $0.76 \pm 0.59 $\\
% \hline
% \RNN2  & $ 11.72 \pm 5.29$ & $0.60 \pm 0.32$ & $0.56 \pm 0.51$ & $0.39 \pm 0.50$ & $0.62 \pm 0.91 $\\
% \hline
% \end{tabular}
% }
% %\label{tab:stat_test}
% \end{table}


% For binary classification task with the usual accuracy score, \MLR{} is a close second behind \GBDT{} both in terms of Accuracy and AUC scores. 
% %better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% %Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

%better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
%Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% \textbf{The \MLR{} method clearly outperforms all the compared methods in the regression task.} \BMLR{} with a \Pb{} of $0.72$ on the whole benchmark and Friedman Rank of $3.5$ is far above \RF{}, with a \Pb{} of $0.5$ and Friedman Rank $7.111$ in Table \ref{tab:perfR2_rank}. 
% As revealed by its \PMA{} statistics at $0.92$%in Table \ref{tab:perfR2_rank})
% , \BMLR{} is far ahead of the other methods. 
% %Thus it actually almost never "loses" to the best method by a lot. 
% This means that \BMLR{} produces reliable results at a rate that is even above methods like \RF{} which are often deemed the safest pick. The same conclusion is also valid for \BMLRa{} and \BMLRb{}.
% Standard NN (\texttt{NN2}) with equivalent architecture and MSE loss perform poorly with a Friedman rank of $11.722$.





% For binary classification task with the usual accuracy score, \XRF{} is better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% of the is similar  standard deviation of the Friedman rank of the \MLR{} performances are equivalent for the mean \AUC{}, the Friedman Rank (\FR) and the \PMA. 


% Regarding the accuracy, although \XRF{} is better in terms of mean accuracy, \Pb{}, \Pc{}, the \MLR{} performance is better than \XRF{} in terms of Friedman Rank ($4.0$ for \MLR{}, $4.31$ for \XRF), and worst for the other metrics.


% AUC: the \MLR{} method produces better discriminating models. Interesting in unbalanced settings.








% Pas utile vu qu'il y a le Friedman Rank: \textcolor{red}{\textbf{Another important take-away fact is that \MLR{} ranks in the top three on $18$ out of the $21$ datasets, on top of being the best in average.}}


% As we observe in Tables \ref{tab:perfR2_rank} and \ref{tab:ACCperf}, the depth $L$ in the \MLRL{} method seems to be the only data-dependent hyperparameter. However a simple aggregation of \NN{} of different depths performs as well as %is able to reliably mimic the best performance of 
% the \NN{} with the most adequate depth for the dataset at hand. 



%Indeed with a Friedman rank of $\textcolor{purple}{Value}$ on the benchmark, \BMLR{} outperforms all \MLRL{} architectures with a Friedman rank of $\textcolor{purple}{Value}$ at best.

%\medskip


% \subsection{Computing time/scalability??????}
% \textcolor{red}{Computing time raisonable???????}

% \textcolor{red}{scalability huge datasets ???????}

% c'est pas le but du papier vu qu'on se concentre sur les petits datasets mais \MLR{} se calcule aussi sur les gros datasets. Cependant le standard NN 


%(learning rate schedulers, optimizers, weight decay, batch-normalization, drop-out, residual layers and leaky activations. 
%All the popular \DL{} schemes can also be leveraged including learning rate schedulers, optimizers, weight decay, batch-normalization, drop-out, residual layers and leaky activations. 


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%%% END INSTRUCTIONS %%%




% \begin{table}[H]
% \caption{\textbf{Performances of the $10$ best methods} for the classification task with the accuracy score.}
% \label{tab:ACCperf}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean \Acc          & \Pb              & \Pc              & \PMA                          \\ \hline
% \hline
% \BMLR{}  & $ \bm{4.00 \pm 3.03}$ & 0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.62 \pm 0.51$ & $0.98 \pm 0.02 $\\
% \BMLRb{}  & $ 4.23 \pm 2.98$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \BMLRa{}  & $ 5.08 \pm 4.70$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \MLRc  & $ 10.00 \pm 4.93$ & $0.86 \pm 0.11$ & $0.69 \pm 0.48$ & $0.54 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \MLRb  & $ 8.23 \pm 4.25$ & $0.86 \pm 0.11$ & $0.77 \pm 0.44$ & $0.62 \pm 0.51$ & $0.97 \pm 0.04 $\\
% \MLRa  & $ 10.23 \pm 3.52$ & $0.86 \pm 0.10$ & $0.77 \pm 0.44$ & $0.46 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \hline
% \RF  & $ 4.23 \pm 4.32$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.77 \pm 0.44$ & $0.98 \pm 0.03 $\\
% \XRF  & $ 4.31 \pm 4.09$ & $0.88 \pm 0.10$ & $1.00 \pm 0.00$ & $0.85 \pm 0.38$ & $0.99 \pm 0.02 $\\
% Bagging  & $ 8.54 \pm 4.24$ & $0.87 \pm 0.10$ & $0.77 \pm 0.44$ & $0.46 \pm 0.52$ & $0.97 \pm 0.02 $\\
% \hline
% \XGB  & $ 4.69 \pm 4.29$ & $0.87 \pm 0.09$ & $0.92 \pm 0.28$ & $0.77 \pm 0.44$ & $0.98 \pm 0.03 $\\
% \hline
% \end{tabular}
% }
% %\label{tab:stat_test}
% \end{table}

% \begin{table}[H]
% \caption{\textbf{Performances of the $10$ best methods} for the classification task with \AUC{} score.}
% \label{tab:AUCperf}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean \AUC          & \Pb              & \Pc              & \PMA                          \\ \hline
%  \hline
% \BMLR{}  & $ \bm{3.46 \pm 2.63}$ & $0.92 \pm 0.09$ & $0.92 \pm 0.28$ & $0.77 \pm 0.44$ & $0.99 \pm 0.02 $\\
% \BMLRb{}  & $ 3.85 \pm 2.85$ & $0.92 \pm 0.09$ & $0.92 \pm 0.28$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \BMLRa{}  & $ 4.08 \pm 3.01$ & $0.92 \pm 0.08$ & $0.92 \pm 0.28$ & $0.92 \pm 0.28$ & $0.99 \pm 0.02 $\\
% \MLRa  & $ 9.31 \pm 2.59$ & $0.90 \pm 0.09$ & $0.85 \pm 0.38$ & $0.46 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \hline
% \RF  & $ 3.46 \pm 3.48$ & $0.92 \pm 0.09$ & $0.85 \pm 0.38$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \XRF  & $ 5.62 \pm 5.42$ & $0.91 \pm 0.09$ & $0.85 \pm 0.38$ & $0.62 \pm 0.51$ & $0.98 \pm 0.02 $\\

% \hline
% \XGB  & $ 6.15 \pm 4.81$ & $0.91 \pm 0.09$ & $0.92 \pm 0.28$ & $0.54 \pm 0.52$ & $0.98 \pm 0.03 $\\
% \hline
% \MLP  & $ 6.38 \pm 4.11$ & $0.91 \pm 0.08$ & $0.92 \pm 0.28$ & $0.62 \pm 0.51$ & $0.98 \pm 0.02 $\\
% \hline
% Enet  & $ 7.69 \pm 4.17$ & $0.90 \pm 0.09$ & $0.62 \pm 0.51$ & $0.46 \pm 0.52$ & $0.97 \pm 0.03 $\\
% Ridge  & $ 7.46 \pm 4.48$ & $0.90 \pm 0.08$ & $0.69 \pm 0.48$ & $0.54 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \hline
% \end{tabular}
% }
% %\label{tab:stat_test}
% \end{table}


% \begin{table}[!hp]
% \caption{\textbf{Performances of the $10$ best methods} for the classification task with \AUC{} score.}
% % \label{tab:classif}
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean \Acc          & \Pb              & \Pc              & \PMA                          \\ \hline
% \hline
% \BMLR{}  & $ 4.00 \pm 3.03$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.62 \pm 0.51$ & $0.98 \pm 0.02 $\\
% \BMLRb{}  & $ 4.23 \pm 2.98$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \BMLRa{}  & $ 5.08 \pm 4.70$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \MLRc  & $ 10.00 \pm 4.93$ & $0.86 \pm 0.11$ & $0.69 \pm 0.48$ & $0.54 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \MLRb  & $ 8.23 \pm 4.25$ & $0.86 \pm 0.11$ & $0.77 \pm 0.44$ & $0.62 \pm 0.51$ & $0.97 \pm 0.04 $\\
% \MLRa  & $ 10.23 \pm 3.52$ & $0.86 \pm 0.10$ & $0.77 \pm 0.44$ & $0.46 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \hline
% \RF  & $ 4.23 \pm 4.32$ & $0.88 \pm 0.10$ & $0.92 \pm 0.28$ & $0.77 \pm 0.44$ & $0.98 \pm 0.03 $\\
% \XRF  & $ 4.31 \pm 4.09$ & $0.88 \pm 0.10$ & $1.00 \pm 0.00$ & $0.85 \pm 0.38$ & $0.99 \pm 0.02 $\\
% Bagging  & $ 8.54 \pm 4.24$ & $0.87 \pm 0.10$ & $0.77 \pm 0.44$ & $0.46 \pm 0.52$ & $0.97 \pm 0.02 $\\
% \hline
% \XGB  & $ 4.69 \pm 4.29$ & $0.87 \pm 0.09$ & $0.92 \pm 0.28$ & $0.77 \pm 0.44$ & $0.98 \pm 0.03 $\\
% \hline
% \end{tabular}
% %\label{tab:stat_test}
% \end{table}


% \begin{table}[!hp]
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean \AUC          & \Pb              & \Pc              & \PMA                          \\ \hline
%  \hline
% \BMLR{}  & $ 3.46 \pm 2.63$ & $0.92 \pm 0.09$ & $0.92 \pm 0.28$ & $0.77 \pm 0.44$ & $0.99 \pm 0.02 $\\
% \BMLRb{}  & $ 3.85 \pm 2.85$ & $0.92 \pm 0.09$ & $0.92 \pm 0.28$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \BMLRa{}  & $ 4.08 \pm 3.01$ & $0.92 \pm 0.08$ & $0.92 \pm 0.28$ & $0.92 \pm 0.28$ & $0.99 \pm 0.02 $\\
% \MLRa  & $ 9.31 \pm 2.59$ & $0.90 \pm 0.09$ & $0.85 \pm 0.38$ & $0.46 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \hline
% \RF  & $ 3.46 \pm 3.48$ & $0.92 \pm 0.09$ & $0.85 \pm 0.38$ & $0.69 \pm 0.48$ & $0.98 \pm 0.02 $\\
% \XRF  & $ 5.62 \pm 5.42$ & $0.91 \pm 0.09$ & $0.85 \pm 0.38$ & $0.62 \pm 0.51$ & $0.98 \pm 0.02 $\\

% \hline
% \XGB  & $ 6.15 \pm 4.81$ & $0.91 \pm 0.09$ & $0.92 \pm 0.28$ & $0.54 \pm 0.52$ & $0.98 \pm 0.03 $\\
% \hline
% MLP  & $ 6.38 \pm 4.11$ & $0.91 \pm 0.08$ & $0.92 \pm 0.28$ & $0.62 \pm 0.51$ & $0.98 \pm 0.02 $\\
% \hline
% Enet  & $ 7.69 \pm 4.17$ & $0.90 \pm 0.09$ & $0.62 \pm 0.51$ & $0.46 \pm 0.52$ & $0.97 \pm 0.03 $\\
% Ridge  & $ 7.46 \pm 4.48$ & $0.90 \pm 0.08$ & $0.69 \pm 0.48$ & $0.54 \pm 0.52$ & $0.97 \pm 0.03 $\\
% \hline

% \end{tabular}
% %\label{tab:stat_test}
% \end{table}



% \begin{table}[!hp]
% \caption{Classification Benchmark.}
% \label{tab:classif}
% \begin{tabular}{|l||c|c||c|c||c|c||c|c||c|c||}
%   \hline
% & \multicolumn{2}{|c||}{\FR}& \multicolumn{2}{|c||}{Mean}& \multicolumn{2}{|c||}{\Pb} & \multicolumn{2}{|c||}{\Pc} &\multicolumn{2}{|c||}{\PMA}   \\
%     \cline{2-11} 
%  Method   & \AUC&\Acc& \AUC&\Acc &\AUC&\Acc&\AUC&\Acc&\AUC&\Acc\\
% \hline
% \BMLR{} & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \BMLRb  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \BMLRa  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% % &\Bag  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \MLRc  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \MLRb  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \MLRa  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \hline
% \RF & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \Bag  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \XRF & 1 & 2& 3 & 4 &5&6 &7&8&9&10\\
% \hline
% \XGB  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
%  \hline
% \end{tabular}
% \end{table}
% \begin{table}[!hp]
% \caption{Classification Benchmark \AUC.}
% \label{Classification AUC}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|c|c|c|}

% Method  & \FR  & Average \AUC & \Pb & \Pc & $\PMA \\
% \hline \hline
% \BMLR{}  &  3.462 & 0.919 & 0.923 & 0.769 & 0.987 \\
% \hline
% \BMLRa  &  4.077 & 0.919 & 0.923 & 0.923 & 0.987 \\
% \hline
% \RF  &  3.462 & 0.917 & 0.846 & 0.692 & 0.984 \\
% \hline
% \BMLRb  &  3.846 & 0.915 & 0.923 & 0.692 & 0.983 \\
% \hline
% \MLP  &  6.385 & 0.913 & 0.923 & 0.615 & 0.981 \\
% \hline
% \XRF  &  5.615 & 0.913 & 0.846 & 0.615 & 0.980 \\
% \hline
% \XGB  &  6.154 & 0.908 & 0.923 & 0.538 & 0.976 \\
% \hline
% \Enet  &  7.692 & 0.902 & 0.615 & 0.462 & 0.968 \\
% \hline
% Ridge  &  7.462 & 0.902 & 0.692 & 0.538 & 0.969 \\
% \hline
% \MLRa  &  9.308 & 0.899 & 0.846 & 0.462 & 0.966 \\
% \hline
% \end{tabular}
% \end{table}


% \begin{table}[!hp]
% \caption{Classification Benchmark Accuracy.}
% \label{Classification ACC}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|c|c|c|}
% \hline
% Method  & \FR  & Average \Accuracy          & \Pb & \Pc & $\PMA \\
% \hline
% \XRF  &  4.308 & 0.883 & 1.000 & 0.846 & 0.988 \\
% \hline
% \RF  &  4.231 & 0.879 & 0.923 & 0.769 & 0.983 \\
% \hline
% \BMLR{}  &  4.000 & 0.879 & 0.923 & 0.615 & 0.984 \\
% \hline
% \BMLRa  &  4.231 & 0.877 & 0.923 & 0.692 & 0.982 \\
% \hline
% \BMLRa  &  5.077 & 0.877 & 0.923 & 0.692 & 0.982 \\
% \hline
% \XGB  &  4.692 & 0.875 & 0.923 & 0.769 & 0.980 \\
% \hline
% \Bag  &  8.538 & 0.867 & 0.769 & 0.462 & 0.970 \\
% \hline
% \MLRc  &  10.000 & 0.864 & 0.692 & 0.538 & 0.967 \\
% \hline
% \MLRa  &  10.231 & 0.863 & 0.769 & 0.462 & 0.966 \\
% \hline
% \MLRb  &  8.231 & 0.863 & 0.769 & 0.615 & 0.965 \\
% \hline
% \end{tabular}
% \end{table}

%\begin{tabular}{|c||c|c|c||c|c|c||c|c|c||}
%   \hline
%Method & \multicolumn{3}{|c||}{\FR} & %\multicolumn{3}{|c||}{Average}& \multicolumn{3}{|c||}{\Pa}\\
%    \cline{2-4} 
 %   \cline{5-7} 
 %    \cline{8-10} 
%    & Reg &\Acc& \AUC& Reg &\Acc& \AUC& Reg &\Acc& \AUC\\
 %  \hline
%\XRF & 1 & 2& 3 &4&5&6&7&8&9\\
%\RF & 1 & 2& 3 &4&5&6&7&8&9\\
 %\hline
%\end{tabular}
% \begin{table*}[!hp]
% \footnotesize
%  	\centering
%   \resizebox{\columnwidth}{!}{%
% 	\renewcommand{\arraystretch}{0.5}
%  \begin{tabular}{|c|c|c |c|c|c |c|c|c|}
%  \hline
%  Name & $L$ & $lr$ & $maxiter$ & \fixB & $J$ & $\bs$ & $T$ & $\sigma$   \\ \hline   
%  $\MLR{}-1 $& $1$ & $10^{-2}$ & $50$ & $5'$ & $4096 = 2^{12}$ & $min(n, 4096)$ & $16$ & $0.03$ \\
%  $\MLR{}-2 $& $2$ & $10^{-3}$ & $100$ & id. & id. & id. & id. & id.\\
%  $\MLR{}-3 $& $3$ & $10^{-3}$ & $200$ & id. & id. & id. & id. & id.\\
%  $\MLR{}-4 $& $4$ & $10^{-4}$ & $400$ & id. & id. & id. & id. & id.\\
%  \hline
%  \end{tabular}
% 	}
%  	\caption{
% Selected and benchmarked architectures. \label{tab:architectures1}
%  }
%  \end{table*}


% \begin{table*}[!hp]
% \footnotesize
%  	\centering
%   % \resizebox{\columnwidth}{!}{%
% %	\renewcommand{\arraystretch}{0.5}
%  \begin{tabular}{|c||c|c |c|c|c |c|c|c|}
%  \hline
% Architecture & $L$ & $\lr$ & $\max_{iter}$ & \fixB & $J$ & $\bs$ & $T$ & $\sigma$   \\ \hline   
%  $\MLR{}-1 $& $1$ & $10^{-2}$ & $50$ & $5'$ & $2^{12}$ & $min(n, J)$ & $16$ & $0.03$ \\
%  $\MLR{}-2 $& $2$ & $10^{-3}$ & $100$ & $id.$ & $id.$ & $id.$& $id.$ & $id.$\\
%  $\MLR{}-3 $& $3$ & $10^{-3}$ & $200$ &  $id.$ & $id.$ & $id.$& $id.$ & $id.$\\
%  $\MLR{}-4 $& $4$ & $10^{-4}$ & $400$ &  $id.$ & $id.$ & $id.$& $id.$ & $id.$\\
%  \hline
%  \end{tabular}
% %	}
%  	\caption{
% Selected and benchmarked architectures. \label{tab:architectures1}
%  }
%  \end{table*}



% \begin{table}[!hp]
% \caption{Ablation studies on our benchmark.}
% \label{tab:ablation1}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Classifier        & Friedman Rank  & Average Accuracy             & \Pa              & \Pb              & $\pm$A                          \\ \hline
% NN    & ? & \textbf{81.95\%$$\pm$$14.10\%} & \textbf{88.89\%} & \textbf{72.22\%} & \textbf{95.72\% $$\pm$$5.17\%} \\ \hline
% NN+Ridge      & ?          & 80.88\%$$\pm$$14.96\%          & 81.11\%          & 65.56\%          & 94.34\% $$\pm$$7.22\%          \\ \hline
% NN+Ridge + MLR     & ?          & 81.02\%$$\pm$$14.47\%          & 85.56\%          & 60.00\%          & 94.55\% $$\pm$$5.89\%          \\ \hline
% NN+Ridge + MLR + Rotation   & ?          & 81.03\% $$\pm$$ 15.09\%        & 85.56\%          & \textbf{72.22\%} & 94.56\% $$\pm$$8.22\%          \\ \hline
% NN+Ridge + MLR + Rotation + Bagging   & ?          & 81.03\% $$\pm$$ 15.09\%        & 85.56\%          & \textbf{72.22\%} & 94.56\% $$\pm$$8.22\%          \\ \hline
% \end{tabular}
% 	}
% \end{table}
%\newpage
% \begin{table}[!hp]
% \caption{Ablation study on our benchmark.}
% \label{tab:ablation2}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% %		\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Classifier        & Friedman Rank  & Average Accuracy             & \Pa              & \Pb              & $\pm$A                          \\ \hline
% NN    & ? & \textbf{\%$$\pm$$ \%} & \textbf{88.89\%} & \textbf{72.22\%} & \textbf{95.72\% $$\pm$$5.17\%} \\ \hline
% Bagging NN     & ?          & 80.88\%$$\pm$$14.96\%          & 81.11\%          & 65.56\%          & 94.34\% $$\pm$$7.22\%          \\ \hline
% \NN     & ?          & 81.02\%$$\pm$$14.47\%          & 85.56\%          & 60.00\%          & 94.55\% $$\pm$$5.89\%          \\ \hline
% Bagging \NN             & ?          & 81.56\% $$\pm$$13.90\%         & 85.56\%          & 67.78\%          & 95.25\% $$\pm$$5.30\%          \\ \hline
% \end{tabular}
% }
% \end{table}


% \textcolor{red}{Il faut faire la Table \ref{tab:perf_rank} pour les performances avec MLR:}
% \begin{table}[!hp]
% \caption{Comparisons of 21 methods on the UCI datasets. \Pa/\Pb: the number of datasets a model achieves 90\%/95\% or more of the maximum test $\Rdeux$-score, divided by the total number of datasets. PMA: average percentage of the maximum test $\Rdeux$-score.}
% \label{tab:perf_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% %		\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Method        & Friedman Rank  & Average Accuracy          & \Pa              & \Pb              & PMA                          \\ \hline
% Bagging MLR               & \textbf{?} & \textbf{81.95\%$$\pm$$14.10\%} & \textbf{88.89\%} & \textbf{72.22\%} & \textbf{95.72\% $$\pm$$5.17\%} \\ \hline
% NN (Xavier init)      & ?          & 80.88\%$$\pm$$14.96\%          & 81.11\%          & 65.56\%          & 94.34\% $$\pm$$7.22\%          \\ \hline
% RF                & ?          & ?\% $$\pm$$13.90\%         & 85.56\%          & 67.78\%          & 95.25\% $$\pm$$5.30\%          \\ \hline
% linear SVM   & ?          & ?\% $$\pm$$ 15.09\%        & 85.56\%          & \textbf{72.22\%} & ?\% $$\pm$$8.22\%          \\ \hline
% \XGB & ?         & 78.21\% $$\pm$$ 20.30\%        & 80.00\%          & 62.22\%          & ?\% $$\pm$$18.05\%         \\ \hline
% MARS & ?         & 78.21\% $$\pm$$ 20.30\%        & 80.00\%          & 62.22\%          & ?\% $$\pm$$18.05\%         \\ \hline
% \end{tabular}	
% }
% %\label{tab:stat_test}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Results.}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\textcolor{red}{BENJAMIN : VOUS FAITES PAS LES MODIFS SUR LES TABLEAUX A LA MAIN, ON EN DISCUTE ET JE LE FAIS AUTOMATIQUEMENT AVEC MON CODE POUR QU'ON PERDES PAS DE TEMPS!}
% \begin{table}[!hp]
% \caption{Regression Benchmark.}
% \label{Regression}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|c|c|c|}
% \hline
% Method  &  $\Rdeux$& \Rank & \Pa & \Pb & $\pm$A \\
% \hline
% \BMLR{}  &  0.672 & 4.939 & 0.800 & 0.628 & 0.919 \\
% \hline
% \BMLRb  &  0.666 & 4.539 & 0.772 & 0.617 & 0.900 \\
% \hline
% \BMLRa  &  0.658 & 6.783 & 0.783 & 0.556 & 0.903 \\
% \hline
% \MLRb  &  0.651 & 7.989 & 0.694 & 0.506 & 0.889 \\
% \hline
% \MLRc  &  0.648 & 7.756 & 0.656 & 0.506 & 0.910 \\
% \hline
% \MLRa  &  0.641 & 9.139 & 0.706 & 0.428 & 0.790 \\
% \hline
% \RF  &  0.640 & 7.761 & 0.644 & 0.489 & 0.706 \\
% \hline
% \XGB  &  0.634 & 7.383 & 0.739 & 0.522 & 0.628 \\
% \hline
% \XRF  &  0.632 & 8.328 & 0.678 & 0.506 & 0.602 \\
% \hline
% \RNN~2  &  0.597 & 10.339 & 0.567 & 0.400 & 0.706 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[!hp]
% \caption{Classification Benchmark \AUC.}
% \label{Classification AUC}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|c|c|c|}

% Method  & \FR  & Average \AUC & \Pb & \Pc & $\pm$A \\
% \hline \hline
% \BMLR{}  &  3.462 & 0.919 & 0.923 & 0.769 & 0.987 \\
% \hline
% \BMLRa  &  4.077 & 0.919 & 0.923 & 0.923 & 0.987 \\
% \hline
% \RF  &  3.462 & 0.917 & 0.846 & 0.692 & 0.984 \\
% \hline
% \BMLRb  &  3.846 & 0.915 & 0.923 & 0.692 & 0.983 \\
% \hline
% \MLP  &  6.385 & 0.913 & 0.923 & 0.615 & 0.981 \\
% \hline
% \XRF  &  5.615 & 0.913 & 0.846 & 0.615 & 0.980 \\
% \hline
% \XGB  &  6.154 & 0.908 & 0.923 & 0.538 & 0.976 \\
% \hline
% \Enet  &  7.692 & 0.902 & 0.615 & 0.462 & 0.968 \\
% \hline
% Ridge  &  7.462 & 0.902 & 0.692 & 0.538 & 0.969 \\
% \hline
% \MLRa  &  9.308 & 0.899 & 0.846 & 0.462 & 0.966 \\
% \hline
% \end{tabular}
% \end{table}


% \begin{table}[!hp]
% \caption{Classification Benchmark Accuracy.}
% \label{Classification ACC}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|c|c|c|}
% \hline
% Method  & \FR  & Average \Accuracy          & \Pb & \Pc & $\pm$A \\
% \hline
% \XRF  &  4.308 & 0.883 & 1.000 & 0.846 & 0.988 \\
% \hline
% \RF  &  4.231 & 0.879 & 0.923 & 0.769 & 0.983 \\
% \hline
% \BMLR{}  &  4.000 & 0.879 & 0.923 & 0.615 & 0.984 \\
% \hline
% \BMLRa  &  4.231 & 0.877 & 0.923 & 0.692 & 0.982 \\
% \hline
% \BMLRa  &  5.077 & 0.877 & 0.923 & 0.692 & 0.982 \\
% \hline
% \XGB  &  4.692 & 0.875 & 0.923 & 0.769 & 0.980 \\
% \hline
% \Bag  &  8.538 & 0.867 & 0.769 & 0.462 & 0.970 \\
% \hline
% \MLRc  &  10.000 & 0.864 & 0.692 & 0.538 & 0.967 \\
% \hline
% \MLRa  &  10.231 & 0.863 & 0.769 & 0.462 & 0.966 \\
% \hline
% \MLRb  &  8.231 & 0.863 & 0.769 & 0.615 & 0.965 \\
% \hline
% \end{tabular}
% \end{table}

%\begin{tabular}{|c||c|c|c||c|c|c||c|c|c||}
%   \hline
%Method & \multicolumn{3}{|c||}{\FR} & %\multicolumn{3}{|c||}{Average}& \multicolumn{3}{|c||}{\Pa}\\
%    \cline{2-4} 
 %   \cline{5-7} 
 %    \cline{8-10} 
%    & Reg &\Acc& \AUC& Reg &\Acc& \AUC& Reg &\Acc& \AUC\\
 %  \hline
%\XRF & 1 & 2& 3 &4&5&6&7&8&9\\
%\RF & 1 & 2& 3 &4&5&6&7&8&9\\
 %\hline
%\end{tabular}




% \begin{table}[!hp]
% \caption{Classification Benchmark.}
% \label{tab:classif}
% \begin{tabular}{|l|l||c|c||c|c||c|c||c|c||c|c||}
%   \hline
% && \multicolumn{2}{|c||}{\FR}& \multicolumn{2}{|c||}{Average}& \multicolumn{2}{|c||}{\Pb} & \multicolumn{2}{|c||}{\Pc} &\multicolumn{2}{|c||}{$\pm$A}   \\
%     \cline{3-12} 
% Class&  Method   & \AUC&\Acc& \AUC&\Acc &\AUC&\Acc&\AUC&\Acc&\AUC&\Acc\\
% \hline
% \MLR&\BMLR{} & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\BMLRa  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\BMLRa  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\Bag  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\MLRc  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\MLRa  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\MLRb  &  1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% \hline
% \RF& \RF & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
% &\XRF & 1 & 2& 3 & 4 &5&6 &7&8&9&10\\
% \hline
% \GBDT&\XGB  & 1 & 2& 3 & 4  &5&6&7&8&9&10  \\
%  \hline
% \end{tabular}
% \end{table}

% We ran the ablation study
% Table \ref{tab:ablation1} summarizes the impact of each key ingredient on the generalization performance of our method. The main contributor is the \MLR{} loss in replacement of the standard $\MSE$ with an improvement of $\%$. Ridge and bagging also contributed more marginally with about $\%$ improvement each. Aggregating standard \RNN{} is not able to beat a single \NN{} (see Table \ref{tab:ablation2}). This further reinforces the \MLR{} loss as the key ingredient in our method. 
% %This further reinforces that the \MLR{} loss is the key ingredient in our method. 
% Moreover the addition of bagging on top of the \MLR{} loss does improve our performance further. 




% \begin{table}[!hp]
% \caption{Ablation studies on our benchmark.}
% \label{tab:ablation1}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Method        & Friedman Rank  & Average Accuracy             & \Pa              & \Pb              & $\pm$A                          \\ \hline \hline
% NN    & ? & \textbf{81.95\%$$\pm$$14.10\%} & \textbf{88.89\%} & \textbf{72.22\%} & \textbf{95.72\% $$\pm$$5.17\%} \\ \hline
% NN+Bagging    & ? & \textbf{81.95\%$$\pm$$14.10\%} & \textbf{88.89\%} & \textbf{72.22\%} & \textbf{95.72\% $$\pm$$5.17\%} \\ \hline \hline
% NN+Ridge      & ?          & 80.88\%$$\pm$$14.96\%          & 81.11\%          & 65.56\%          & 94.34\% $$\pm$$7.22\%          \\ \hline
% NN+Ridge + MLR Loss    & ?          & 81.02\%$$\pm$$14.47\%          & 85.56\%          & 60.00\%          & 94.55\% $$\pm$$5.89\%          \\ \hline
% \MLR-NN: NN+Ridge + MLR Loss + Rotation   & ?          & 81.03\% $$\pm$$ 15.09\%        & 85.56\%          & \textbf{72.22\%} & 94.56\% $$\pm$$8.22\%          \\ \hline
% Bagging \MLR-NN  & ?          & 81.03\% $$\pm$$ 15.09\%        & 85.56\%          & \textbf{72.22\%} & 94.56\% $$\pm$$8.22\%          \\ \hline
% \end{tabular}
% 	}
% \end{table}



% \begin{table}[!hp]
% \caption{Performances of ??? methods for the regression task \textcolor{red}{on the UCI database.  on the UCI datasets????}. \Pa/\Pb: the number of datasets a model achieves 90\%/95\% or more of the maximum test $\Rdeux$-score, divided by the total number of datasets. $\pm$A: average percentage of the maximum test $\Rdeux$-score.}
% \label{tab:perfR2_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% %		\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Method        & Friedman Rank  & Average $\Rdeux$-score          & \Pa              & \Pb              & $\pm$A                          \\ \hline
% \hline
% ensemble  &  3.500 & 0.672 & 0.889 & 0.722 & 0.918 \\
% \hline
% \BMLRb{}// MLR2bagging  &  3.944 & 0.666 & 0.833 & 0.611 & 0.880 \\
% \hline
% \BMLRa{}// MLR1bagging  &  5.500 & 0.658 & 0.833 & 0.667 & 0.916 \\
% \hline
% MLR2  &  7.944 & 0.651 & 0.722 & 0.444 & 0.863 \\
% \hline
% MLR3  &  7.333 & 0.648 & 0.667 & 0.444 & 0.830 \\
% \hline
% MLR1  &  9.056 & 0.641 & 0.778 & 0.444 & 0.809 \\
% \hline
% \RF   &  7.111 & 0.640 & 0.667 & 0.500 & 0.677 \\
% \hline
% \XGB  &  7.222 & 0.634 & 0.722 & 0.667 & 0.756 \\
% \hline
% \XRF  &  7.556 & 0.632 & 0.722 & 0.500 & 0.677 \\
% \hline
% \texttt{NN2} &  11.722 & 0.597 & 0.556 & 0.389 & 0.616 \\
% \hline
% \end{tabular}	
% }
% %\label{tab:stat_test}
% \end{table}





% \subsection{Overall Performance comparisons.}

%\paragraph{R2 Score.}



% \begin{table}[!hp]
% \caption{\textcolor{red}{rajouter la colonne class aussi.} Performances of ??? methods for the regression task \textcolor{red}{on the UCI database.  on the UCI datasets????}. \Pa/\Pb: the number of datasets a model achieves 90\%/95\% or more of the maximum test $\Rdeux$-score, divided by the total number of datasets. $\pm$A: average percentage of the maximum test $\Rdeux$-score.}
% \label{tab:perfR2_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% %		\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Method        & Friedman Rank  & Average $\Rdeux$-score          & \Pa              & \Pb              & $\pm$A                          \\ \hline
% \hline
% \BMLR{}  &  3.500 & 0.672 & 0.889 & 0.722 & 0.918 \\
% \hline
% \BMLRb{}  &  3.944 & 0.666 & 0.833 & 0.611 & 0.880 \\
% \hline
% \BMLRa{}  &  5.500 & 0.658 & 0.833 & 0.667 & 0.916 \\
% \hline
% \MLRb  &  7.944 & 0.651 & 0.722 & 0.444 & 0.863 \\
% \hline
% \MLRc  &  7.333 & 0.648 & 0.667 & 0.444 & 0.830 \\
% \hline
% \MLRa  &  9.056 & 0.641 & 0.778 & 0.444 & 0.809 \\
% \hline
% \RF   &  7.111 & 0.640 & 0.667 & 0.500 & 0.677 \\
% \hline
% \XGB  &  7.222 & 0.634 & 0.722 & 0.667 & 0.756 \\
% \hline
% \XRF  &  7.556 & 0.632 & 0.722 & 0.500 & 0.677 \\
% \hline
% \texttt{NN2} &  11.722 & 0.597 & 0.556 & 0.389 & 0.616 \\
% \hline
% \end{tabular}	
% }
% %\label{tab:stat_test}
% \end{table}





% \begin{table}[!hp]
% \caption{\textcolor{red}{rajouter la colonne class aussi.} Performances of ??? methods for the regression task \textcolor{red}{on the UCI database.  on the UCI datasets????}. \Pa/\Pb: the number of datasets a model achieves 90\%/95\% or more of the maximum test $\Rdeux$-score, divided by the total number of datasets. \PMA: average percentage of the maximum test $\Rdeux$-score.}
% \label{tab:perfR2_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{%
% %		\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Class& Method        & Friedman Rank  & Mean $\Rdeux$-score          & \Pa              & \Pb              & \PMA                          \\ \hline
% \hline
% \MLR&\BMLR{}  &  3.500 & 0.672 & 0.889 & 0.722 & 0.918 \\
% &\BMLRb{}  &  3.944 & 0.666 & 0.833 & 0.611 & 0.880 \\
% &\BMLRa{}  &  5.500 & 0.658 & 0.833 & 0.667 & 0.916 \\
% &\MLRc  &  7.333 & 0.648 & 0.667 & 0.444 & 0.830 \\
% &\MLRb  &  7.944 & 0.651 & 0.722 & 0.444 & 0.863 \\
% % \MLRc  &  7.333 & 0.648 & 0.667 & 0.444 & 0.830 \\
% % \hline
% &\MLRa  &  9.056 & 0.641 & 0.778 & 0.444 & 0.809 \\
% \hline
% \texttt{Ens.}&\RF   &  7.111 & 0.640 & 0.667 & 0.500 & 0.677 \\
% &\XGB  &  7.222 & 0.634 & 0.722 & 0.667 & 0.756 \\
% &\XRF  &  7.556 & 0.632 & 0.722 & 0.500 & 0.677 \\
% \hline
% &\XGB  &  7.222 & 0.634 & 0.722 & 0.667 & 0.756 \\
% \hline
% \DL&\RNN2 &  11.722 & 0.597 & 0.556 & 0.389 & 0.616 \\
% \hline
% \end{tabular}	
% }
% %\label{tab:stat_test}
% \end{table}


% \begin{table}[!hp]
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean $\Rdeux$-score          & \Pa              & \Pb              & \PMA                          \\ \hline
% \hline
% \hline
% \BMLR{}  & $ 3.50 \pm 2.38$ & $0.67 \pm 0.25$ & $0.89 \pm 0.32$ & $0.72 \pm 0.46$ & $0.92 \pm 0.17 $\\
% \BMLRb{}  & $ 3.94 \pm 2.84$ & $0.67 \pm 0.26$ & $0.83 \pm 0.38$ & $0.61 \pm 0.50$ & $0.88 \pm 0.28 $\\
% \BMLRa{}  & $ 5.50 \pm 4.51$ & $0.66 \pm 0.24$ & $0.83 \pm 0.38$ & $0.67 \pm 0.49$ & $0.92 \pm 0.13 $\\
% \MLRc  & $ 7.33 \pm 3.80$ & $0.65 \pm 0.27$ & $0.67 \pm 0.49$ & $0.44 \pm 0.51$ & $0.83 \pm 0.37 $\\
% \MLRb  & $ 7.94 \pm 3.83$ & $0.65 \pm 0.26$ & $0.72 \pm 0.46$ & $0.44 \pm 0.51$ & $0.86 \pm 0.26 $\\
% \MLRa   & $ 9.06 \pm 4.49$ & $0.64 \pm 0.25$ & $0.78 \pm 0.43$ & $0.44 \pm 0.51$ & $0.81 \pm 0.47 $\\
% \hline
% \RF   & $ 7.11 \pm 6.57$ & $0.64 \pm 0.28$ & $0.67 \pm 0.49$ & $0.50 \pm 0.51$ & $0.68 \pm 1.01 $\\
% \XRF  & $ 7.56 \pm 5.82$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.50 \pm 0.51$ & $0.68 \pm 0.93 $\\
% \hline
% \XGB  & $ 7.22 \pm 6.68$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.67 \pm 0.49$ & $0.76 \pm 0.59 $\\
% \hline
% \RNN2  & $ 11.72 \pm 5.29$ & $0.60 \pm 0.32$ & $0.56 \pm 0.51$ & $0.39 \pm 0.50$ & $0.62 \pm 0.91 $\\
% \hline
% \end{tabular}
% %\label{tab:stat_test}
% \end{table}

==> Old/Old_main/old_results_section.tex <==
% \section{Experiments}\label{sec:exp}


% Our goal is this section is to tabulate the performance of \trainmet{} against a large set of available methods including the standard \DNN{} implementations on benchmark datasets


% Our goal is this section is to tabulate the performance of \trainmet{} compared to a he standard \DNN{}

% Our goal in this section is to tabulate the performance of
% PFL and its variants against the state-of-art algorithms on
% benchmark datasets. We sample device data to synthesize
% various degrees of statistical data heterogeneity and task
% diversity among devices. We then report performance and
% tabulate our results against several metrics including oracle
% performance (centralized data), average customization performance, best and worst device customization. For each of
% these, we report the number of model transmissions required
% by PFL to achieve target accuracy of the competito



% Finding:

% Voir : % http://proceedings.mlr.press/v139/acar21a/acar21a.pdf
% - à feature équivalente, si on change la target on a le classement qui change, l traitement des features fait pas tout
% - trainmet est parfois meilleur\\
% - trainmet est le plus utile pour aller chercher les derniers points de généralisation sur des jeux de donnée midsize\\
% - Catboost reste l'algo qui marche le mieux le plus souvent\\
% - Plein de méthodes différentes sont parfois les meilleurs il faut continuer à tester plein de méthodes sur les benchmarks\\
% - En faisant du métalearning on peut dépasser la meilleure méthode avec d'autre, donc la meilleure méthode suffit pas\\
% - En faisant du bagging on peut améliorer significativement ça peut être bcp plus efficace et bcp moins cher \\
% - La gestion des features catégorielles est pas le seul axe d'amélioration, sur des jeux de données sans feature cat il y a encore bcp de chose à dire/à faire.\\
% - C'est important de regarder les tailles de données, ça suffit pas de regarder juste la classification. \\
% - shrinkage peut déjà améliorer beaucoup, ensuite MLR est une upgrade\\
% - La seed influence surtout le train valid cut pour l'early stopping, pas le choix des permuts\\
% - trainmet marche mieux avec des réseaux larges\\
% - trainmet marche mieux avec des batch larges\\
% - sur les petits modèles trainmet est bcp plus long que la méthode classique, sur les gros modèle c'est pas le cas\\
% - trainmet se combine très bien avec resblock, très mal avec dropout et batchnorm\\
% - trainmet requires earlystopping\\
% - trainmet loss match beaucoup plus la perf de généralization que la loss normale (et on devrait s'y attendre!)\\
% - trainmet loss est beaucoup plus stable que standard loss, beaucoup/pas d'estimation \\

% - trainmet est-il plus fiable que regularnet? plus souvent dans le top? Moins de fois très mauvais?\\
% - trainmet est-il parfois vraiment bien meilleur que les autres? \\
% - Il faut pas mettre de coefficient devant les termes de MLR ça marche moins bien.\\
% - trainmet marche bien aussi avec des convnets, la plus value est très importante sur un trainset plus petit\\
% - Les tabular dataset c'est encore un champ très ouvert, on peut pas pour l'instant choisir une solution unique ou même restreindre à quelques candidats.\\
% - Commentaire sur l'impact de la profondeur sur trainmet\\
% - Commentaire sur la taille des données qui cela favorise\\
% - beaucoup de dataset + beaucoup de seed + beaucoup de méthodes = coûte cher et compliqué, tâche trop générale, il faudrait peut être restreindre ou segmenter le problème pour pouvoir mieux progresser.\\
% - Les méthodes les plus réputées le sont quand même pour de bonnes raisons, 

% - Pour le même dataset, selon la taille du train size le classement des méthodes peut changer du tout au tout, besoin de tester plusieurs trainsize pour comprendre\\
% -Il y a pas vraiment un trade off temps performance, les temps de calcul varient énormément entre méthodes, et entre implémentations\\
% - c'est quoi les méthodes qui sont jamais les meilleurs, c'est lesquels qu'on peut commencer à exclure, qui sont toujours moins bonne qu'une autre?\\
% - les métriques utilisées impactes beaucoup les résultats du benchmark, R2 vs RMSE\\
% - Le nombre de seed est important pour le découpage train test, d'une seed à l'autre les résultats peuvent bcp changer.\\
% - C'est important d'avoir une diversité de dataset et méthodes









% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{The goal of this benchmark.}

% Phrase objectif de l'etude.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{\trainmet{} Methods.}
% We evaluate \trainmet{} variants, namely,...\\
% We compare our methods to



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Compared models.}

% See Appendix \ref{} for the exhaustive list of compared methods and details about their implementations.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Datasets.}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Performance metrics.}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Results.}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Considered models.}
% \textcolor{red}{A REPRENDRE et METTRE DANS LA PARTIE SUIVANTE.}
% % \sout{We propose several models with varying depth based on \FFNN{} trained with the \MLR{} loss. We also create ensemble models combining architectures of different depth.
% % %We propose several models based on \FFNN{} trained with the \MLR{} loss:\\
% % Our models are:\\
% % $\bullet$  \MLRL: a simple \FFNN{} of depth $L$ ($1\leq L\leq 4$).\\
% % $\bullet$ \BMLRL: a bagging of 10 \FFNN{} of depth $L$ ($L=1$ or $L=2$).\\
% % $\bullet$ \BMLR{}: an ensemble of 20 \FFNN{} (the aggregation of \BMLRa{} and \BMLRb{} of depth $1$ and $2$ respectively).\\
% % $\bullet$ \BestMLR{}: the best prediction among 20 \NN{} in terms of the validation score.\\
% % $\bullet$ \TopfiveMLR{}: the aggregation of the top 5 among 20 \NN{} in terms of the validation score.\\
% % For the methods based on bagging \cite{breiman1996}, the final prediction is the mean of each \NN{} prediction.
% % }
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% We provide both the code to download raw files and apply each steps, and the resulting data matrices. All results are fully reproducible as both random seeds and random states were manually set and saved at every step of our experiments. 
% %See the supplementary material for the github repository.

% See the supplementary material for the the github repository, the detailed description of our experimental setting and the exhaustive list of compared methods with their performances. 




% To train \eqref{eq:ridgeMLRNN}, we use Adam \cite{kingma2014adam} with default parameters except for the learning rate $\lr$ which depends on the number of layers $L$. Weights $\bth$ are initialized as in \cite{Gloriotetal} and $\bla_{init}$ is chosen to maximize sensitivity of the $\MLR{}$ metric to variation of $\bla$ \sout{(See \eqref{lambdainiti} below for our heuristic rule)}. Our empirical investigations revealed that the obtained $\widehat{\bla}$ after training is close to the optimal oracle choice of $\bla$ on the test set. The complete training protocol is provided in Appendix \ref{sec:appprotocol}. \textcolor{red}{RAJOUTER UNE EXPERIENCE POUR CONFIRMER}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Setting.}


% \paragraph{Benchmark description.}


% To produce this benchmark we aggregated 32 tabular datasets (16 in regression  and 16 in classification), from the UCI repository and Kaggle. %See the appendix for the exhaustive list. 
% For computational reasons, we have chosen to restrict the number of datasets but we performed more $train$/$test$ splitting in order to reduce the variance of our results. 
% We curated the UCI repository and Kaggle through a set of rules detailed in the appendix ($e.g.$ discard empty or duplicate datasets, times series, missing target, non $i.i.d.$ samples, text format, $etc$.). %See in the Appendix for more details.
% %We added $Value$ datasets by repeating the same process on Kaggle\cite{} using the tags with "task": "regression" and "format" : ".csv",".xls". \textcolor{red}{We repeated the same process for classification \sout{and ended up with $Value$ datasets well suited for tabular classification.}}
% %See Table \ref{} in the Appendix for the list of violated rules for each available dataset. \textcolor{red}{In summary, we have ? regression datasets and ? classification datasets.}
% %\textcolor{red}{B: Mauvais argument, il y a déjà des gens qui sont passés derrière et qui ont corrigés le bench. Plutôt dire que pour des raisons de temps de calcul, on a préféré faire moins de jeux de données, mais remanier en plus propre et surtout avec 10 découpages train test par expérience.}
% %Although \cite{Delgado14a} already built a benchmark based on the UCI repository, their methodology presents some flaws \cite{Wainberg2016}. 
% %Hence, we went back to the exhaustive list of $Value$ available datasets tagged as regression in the UCI repository and curated it through  .
% %Hence, we started anew and curated the UCI repository through a set of rules detailed in the appendix ($e.g.$ discard empty or \textbf{duplicate} datasets, times series, missing target, non $i.i.d.$ samples, text format, $etc$.). After an exhaustive screening of the $Value$ available datasets tagged as regression, we were left with $Value$ datasets. We added $Value$ datasets by repeating the same process on Kaggle\cite{} using the tags with "task": "regression" and "format" : ".csv",".xls". \textcolor{red}{We repeated the same process for classification \sout{and ended up with $Value$ datasets well suited for tabular classification.}}
% %See Table \ref{} in the Appendix for the list of violated rules for each available dataset. \textcolor{red}{In summary, we have ? regression datasets and ? classification datasets.}
% %Contrarily to classification, there are not that many publicly available well-known datasets which are actually well suited for a tabular regression benchmark. 



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Preprocessing.} To avoid biasing the benchmark towards specific methods and to get a result as general as possible, we only applied as little preprocessing as we could, without using any feature augmentation scheme. The goal is not to get the best possible performance on a given dataset but to compare the methods on equal ground. We first removed features with constant values such as sample index. Categorical features with more than 12 modalities were discarded as learning embeddings is out of the scope of this benchmark. We also removed samples with missing target. Next, all missing values are imputed with the mean and the mode for numerical and categorical features respectively. We applied one-hot-encoding for categorical values and standardization for numerical features and target. 
% %\textcolor{red}{We use a 80/20 ratio for each of the 10 $train$/$test$ splits of the dataset,} with a different seed and no stratification scheme. 
% %We repeated $10$ times a $80:20$ train/test split of the data with a different seed and no stratification scheme. 
% We repeated our experiments 10 times using a different $80:20$ $train$/$test$ split of the data and no stratification scheme. 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Compared methods.}
% We ran the benchmark with \textbf{all the methods available in the scikit-learn library} for classification and regression (including \RF{} and \XGB) as well as the \GBDT{} methods. In the rest of the paper, we only display the main classes of methods in Table \ref{tab:methods}.
% %\texttt{Fast.ai} \cite{Howard2020}, \Catboost{} \cite{Prokhorenkova2018}, \XGBoost{} \cite{guestrin2016} and \lightgbm{} \cite{Ke2017}. 
% %For all our proposed \MLR-architectures, we run its standard equivalent in \DL{} (denoted as \RNN2 for \MLRb{} as an example). 
% %In the rest of the paper, we only display the main classes of methods: \MLR{}, \GBDT{} (\XGB, \XGBoost, \Catboost, \lightgbm), \RF{} (\RF{} and \XRF), \SVM{}, \RNN{} (\texttt{Fast.ai} and \MLP), \MARS{}, \GLM{} (Generalized Linear Models: LSE, Elastic Net, Ridge, LASSO, Logistic regression), \TREE{} (CART, XCART) and the \Baseline{} (intercept for regression and class probabilities for classification).
% %The exhaustive list of methods and results is provided in the supplementary material.
% %each architecture we tested for MLR, we also ran a standard NN with the same architecture and parameters.


% % \begin{table}[h]
% % \caption{Main classes of methods.}
% % \label{tab:methods}
% % 	\centering
% % 	\footnotesize
% % 	%	\renewcommand{\arraystretch}{1.5}
% % \begin{tabular}{|c|c|}
% % \hline
% % Class      & \\
% % of Methods & Methods\\
% % \hline
% % \MLR{} (this paper)   & \MLRL, \BMLRL, \BMLR, \BestMLR, \TopfiveMLR  \\
% % \hline
% % \GBDT  & \XGB{} \cite{Breiman1997_arcing,Friedman2001,Friedman2002},  \Catboost{} \cite{Prokhorenkova2018}, \XGBoost{} \cite{guestrin2016}, \lightgbm{} \cite{Ke2017} \\
% % \hline
% % \RF  & \RF{} and \XRF{} \cite{breiman2001,barandiaran1998random}  \\
% % \hline               
% % \SVM &  \texttt{Lin-}\SVM{}, \SVM{}, $\nu$\texttt{-}\SVM{} \cite{Chihchung2011}\\
% % \hline
% % \RNN   & \texttt{Fast.ai} \cite{Howard2020}, \MLP \cite{Hinton89connectionistlearning}\\
% % \hline
% % \GLM   & \texttt{OLS}, \Enet{} \cite{Zou05}, \Ridge{} \cite{Hoerl1970}, \LAS{} \cite{tibshirani1996}, \texttt{Logistic regression} \cite{cox1958}\\
% % \hline
% % \MARS & \MARS{} \cite{Friedman1991}\\
% % \hline
% % \TREE& \texttt{CART}, \texttt{XCART} \cite{Breiman1984,gey2005model,Klusowski2020sparse}\\
% % \hline
% % \Baseline & Reg: \texttt{Intercept}$\,|\,$ Classif: \texttt{Class probabilities}\\
% % \hline
% % \end{tabular}
% % \end{table}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Ablation Analysis.}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \begin{table}[!hp]
% % \caption{Ablation Study in Regression. %\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.}
% % }
% % \label{tab:ablation}
% % 	\centering
% % 	\footnotesize
% % 	%	\renewcommand{\arraystretch}{1.5}
% % \begin{tabular}{|l||c|c|}
% % \hline
% % Step  &  Mean $\Rdeux$  & Bagging $\Rdeux$ \\
% % \hline
% % \hline
% % \FFNN   & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% % \hline
% % + Ridge  & $ 0.32  \pm  0.17 $ & $ 0.39  \pm  0.12 $ \\
% % \hline
% % + Ridge + Struct. Dithering   & $ 0.32  \pm  0.16 $ & $ 0.40  \pm  0.11 $ \\
% % \hline
% % + Ridge + Permut.  & $ 0.36  \pm  0.11 $ & $ 0.43  \pm  0.07 $ \\
% % \hline
% % \MLR{}  & $ 0.37  \pm  0.10 $ & $ 0.43  \pm  0.07 $ \\
% % \hline
% % \end{tabular}
% % \end{table}

% %\textcolor{red}{$\ast$}
% %\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.
% \begin{table}[h]
% \label{tab:ablation}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|}
% \hline
% Step  &  Mean $\Rdeux$  & Bagging $\Rdeux$ \\
% \hline
% \hline
% \FFNN  & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% \hline
% + Ridge  & $ 0.321  \pm  0.081 $ & $ 0.394  \pm  0.052 $ \\
% % \hline
% % + Ridge + Struct. Dithering  & $ 0.323  \pm  0.075 $ & $ 0.400  \pm  0.048 $ \\
% \hline
% + Ridge + Permut. & $ 0.364  \pm  0.050 $ & $ 0.432  \pm  0.035 $\\
% \hline
% % \MLR{}   & $ 0.371  \pm  0.024 $ & $ 0.433  \pm  0.000 $ \\
% %\hline
% \end{tabular}
% \caption{Ablation Study for \MLR{} in Regression. %\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.}
% }
% \end{table}



% % NN2  & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% % RidgeNN2  & $ 0.321  \pm  0.081 $ & $ 0.394  \pm  0.052 $ \\
% % RidgeSpectral2  & $ 0.323  \pm  0.075 $ & $ 0.400  \pm  0.048 $ \\
% % RidgePermut2  & $ 0.364  \pm  0.050 $ & $ 0.432  \pm  0.035 $ \\
% % RidgePermutSpectral2  & $ 0.371  \pm  0.024 $ & $ 0.433  \pm  0.000 $ \\


% % The following is a summary of our findings, we refer the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance.
% % %See the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance. 
% % The generic values ($\tilde{\sigma} = 0.03$ and $T=16$) for the \dither{} and the number of permutations hyperparameters yield consistently good results overall. The \dither{} parameter admits an optimal value (see Figure ? in the Appendix) which seems to correspond to the standard deviation of the target noise. As soon as $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. In addition, when $T=16$, GPU parallelization is still preserved.
% % %For $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. Moreover, this value is not too large as it preserves GPU parallelization. Consequently, $T=16$ has little to no impact on the runtime of our method. 
% % Recall that the Ridge parameter $\bla$ is trained alongside the weights of the \FFNN{} architecture and the initial value $\bla_{init}$ is fixed by the heuristic choice (\ref{lambdainiti}). Our investigations (see Figure \ref{?}) reveals that this choice is close to the optimal oracle choice on the test set. We can also see that the runtime overhead cost of replacing a matrix multiplication with a matrix inversion depends only linearly on the width $J$ and the batch size $\bs$, which are fixed in our method.

% % We perform 10 repetitions of our ablation study on 3 datasets which are representative of all the 

% % The improvement of each ingredient of the \MLR{} method is statistically significant 


% We ran our ablation study (Table \ref{tab:ablation}) in the regression setting on 3 datasets with different sample sizes and feature to sample ratios. We repeated each experiment over 100 random $train$/$test$ splits. All the results presented here correspond to the architecture and hyperparameters of \MLRb{} and \BMLRb{}.
% %the 3 components of \MLR{} are Ridge regularization, structure dithering and random permutations.
% %Ridge regularization is the essential component of the method as both structured dithering and random permutations are follow-up steps which require the last layer to be a close form. rely on the Ridge close-form. 
% % Recall that Ridge regularization is the essential component of the method as it provides a closed form representation of the last hidden layer on which we can conveniently apply the follow-up treatments: structured dithering and/or random permutations. 

% %Permutations and structured dithering nous fait battre l'etat de l'art.

% A standard \FFNN{} of $2$ layers with a wide architecture ($J=1024$) cannot be trained efficiently on such small datasets as the \FFNN{} instantly memorizes the entire dataset. This cannot be alleviated through bagging at all. Note also its lower overall performance on the complete benchmark (Table \ref{tab:perfR2_rank}). %Note also that bagging cannot help it overcome its overwhelming flaws. 
% %Applying Ridge on the last hidden layer allows the \FFNN{} to learn but its generalization performance is still far behind the gold standard \RF. 
% Applying Ridge on the last hidden layer allows an extremely overparametrized \FFNN{} to learn but its generalization performance is still far behind the gold standard \RF{}. However, when using bagging with ten such models, we reach very competitive results, underlying the potential of the \MLR{} approach.


% \textcolor{red}{
% In our experiments, we see that both Ridge regularization and  random permutations yield an improvement of the generalization performance. Even better, their effects stack up so that a single \NN{} trained with the \MLR{} method can reach or even outperform the gold-standard methods on most datasets. Furthermore, the improvement yielded by using bagging on top of the \MLR{} method is still of the same order of magnitude ($0.062$) as the one we got when we applied random permutations on top of Ridge regularization to the \FFNN{} ($0.043$). This means the two ingredients of the \MLR{} method (random permutations and Ridge regularization) are not just simple variance reduction techniques like bagging but actually work in a more sophisticated way to build generalizing models. See again Figure \ref{} which reveals highly structured embeddings on the last hidden layer of the trained \NN.}


 



% %the \MLR{} method attains a significantly higher $R^2$-score.  better higher performance


% %Clearly, using permutations improves the performance much further than Structured Dithering, however, they are both useful. Without bagging, a single \NN{} can reach or even outperform the gold-standard methods on most datasets (see the following section for details). Furthermore, the improvement yielded by using bagging($0.062$ is still of the same magnitude as the one when we started ($0.073$). 
% %This means these two ingredients are not just simple variance reduction techniques but actually generate more sophisticated models.

% %This means these two ingredients are not simply improving the robustness of the model or reduce its variance, but contribute to learning more complex yet generalizable patterns even with such a large network, over so few samples. 




% %Interestingly, the impact of the other hyperparameters in our method is sometimes strikingly different from what is usually observed in the general deep learning framework. With our method, using wider architecture and bigger batch size is always better. See Figures \ref{} and \ref{}. 



% \subsection{Overall Performance comparisons.}


% % \begin{table}[!hp]
% % \caption{\textbf{Performances of the $10$ best methods} for the regression task on our benchmark. \Pa, \Pb, \Pc: the number of datasets a model achieves 90\%, 95\%, 98\% or more of the maximum test $\Rdeux$-score respectively, divided by the total number of datasets. \PMA: average percentage of the maximum test $\Rdeux$-score.}
% % \label{tab:perfR2_rank}
% % 	\centering
% % 	\resizebox{\columnwidth}{!}{
% % \begin{tabular}{|l|c|c|c|c|c|c|}
% % \hline
% %  Method        & \FR  & Mean $\Rdeux$-score          & \Pa              & \Pb              & \PMA                          \\ \hline
% % \hline
% % \hline
% % \BMLR{}  & $\bm{3.50 \pm 2.38}$ & \textbf{$0.67 \pm 0.25$} & \textbf{$0.89 \pm 0.32$} & \textbf{$0.72 \pm 0.46$} & \textbf{$0.92 \pm 0.17 $}\\
% % \BMLRb{}  & $ 3.94 \pm 2.84$ & $0.67 \pm 0.26$ & $0.83 \pm 0.38$ & $0.61 \pm 0.50$ & $0.88 \pm 0.28 $\\
% % \BMLRa{}  & $ 5.50 \pm 4.51$ & $0.66 \pm 0.24$ & $0.83 \pm 0.38$ & $0.67 \pm 0.49$ & $0.92 \pm 0.13 $\\
% % \MLRc  & $ 7.33 \pm 3.80$ & $0.65 \pm 0.27$ & $0.67 \pm 0.49$ & $0.44 \pm 0.51$ & $0.83 \pm 0.37 $\\
% % \MLRb  & $ 7.94 \pm 3.83$ & $0.65 \pm 0.26$ & $0.72 \pm 0.46$ & $0.44 \pm 0.51$ & $0.86 \pm 0.26 $\\
% % \MLRa   & $ 9.06 \pm 4.49$ & $0.64 \pm 0.25$ & $0.78 \pm 0.43$ & $0.44 \pm 0.51$ & $0.81 \pm 0.47 $\\
% % \hline
% % \RF   & $ 7.11 \pm 6.57$ & $0.64 \pm 0.28$ & $0.67 \pm 0.49$ & $0.50 \pm 0.51$ & $0.68 \pm 1.01 $\\
% % \XRF  & $ 7.56 \pm 5.82$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.50 \pm 0.51$ & $0.68 \pm 0.93 $\\
% % \hline
% % \XGB  & $ 7.22 \pm 6.68$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.67 \pm 0.49$ & $0.76 \pm 0.59 $\\
% % \hline
% % \RNN2  & $ 11.72 \pm 5.29$ & $0.60 \pm 0.32$ & $0.56 \pm 0.51$ & $0.39 \pm 0.50$ & $0.62 \pm 0.91 $\\
% % \hline
% % \end{tabular}
% % }
% % %\label{tab:stat_test}
% % \end{table}




% \begin{table}[H]
% \label{tab:perfR2_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% Class      &   &           &               &    &           &                          \\
%  of Methods        & \FR  & Mean $\Rdeux$-score          & \Pa              & \Pb    & \Pc          & \PMA                          \\
%   \hline
% \hline
% \hline
% \MLR & $2.525 \pm 1.355$ & $0.744 \pm 0.022$ & $0.963$ & $0.856$ & $0.719$ & $0.946 \pm 0.089$\\
% \GBDT & $2.719 \pm 1.850$ & $0.726 \pm 0.093$ & $0.863$ & $0.756$ & $0.650$ & $0.898 \pm 0.237$\\
% \RF & $3.538 \pm 1.896$ & $0.724 \pm 0.070$ & $0.825$ & $0.681$ & $0.481$ & $0.914 \pm 0.159$\\
% \SVM & $4.281 \pm 1.534$ & $0.711 \pm 0.068$ & $0.831$ & $0.594$ & $0.362$ & $0.882 \pm 0.172$\\
% \RNN & $4.331 \pm 2.206$ & Aberating value & $0.725$ & $0.606$ & $0.475$ & Aberating value \\
% \MARS & $5.644 \pm 1.623$ & $0.677 \pm 0.066$ & $0.537$ & $0.350$ & $0.163$ & $0.861 \pm 0.167$\\
% \LM & $5.938 \pm 1.804$ & $0.658 \pm 0.094$ & $0.531$ & $0.294$ & $0.156$ & $0.837 \pm 0.179$\\
% \TREE & $7.125 \pm 1.613$ & $0.512 \pm 0.237$ & $0.338$ & $0.188$ & $0.119$ & $0.578 \pm 0.570$\\
% \Baseline & $8.900 \pm 0.375$ & $-0.023 \pm 0.211$ & $0.000$ & $0.000$ & $0.000$ & $-0.031 \pm 0.075$\\
% \hline
% \end{tabular}
% }
% \caption{\textbf{Performances of the best method in each class of methods} for the regression task on our benchmark. \Pa, \Pb, \Pc: the number of datasets a model achieves 90\%, 95\%, 98\% or more of the maximum test $\Rdeux$-score respectively, divided by the total number of datasets. \PMA: average percentage of the maximum test $\Rdeux$-score.}
% %\label{tab:stat_test}
% \end{table}



% \textbf{The \MLR{} method clearly outperforms all the compared methods for the regression task.} \BMLR{} with a \Pc{} of $0.719$ on the whole benchmark and Friedman Rank of $2.525$ is above \GBDT{}, with a \Pc{} of $0.65$ and Friedman Rank $2.719$ in Table \ref{tab:perfR2_rank}. 
% As revealed by its \PMA{} statistics at $0.946$%in Table \ref{tab:perfR2_rank})
% , \BMLR{} is far ahead of the other methods. 
% %Thus it actually almost never "loses" to the best method by a lot. 
% This means that \MLR{} produces reliable results at a rate that is even above methods like \RF{} which are often deemed the safest pick. 
% %The same conclusion is also valid for \BMLRa{} and \BMLRb{}.
% Standard \RNN{} with equivalent architecture and \MSE{} loss performs poorly with a Friedman rank of $4.331$. Noticeably, \BMLR{} was most often the best method among all the \MLR{} methods.% See the appendix for more details.




% \begin{table}[h]
% \caption{\textbf{Performances of the best method in each class of methods} for the classification task with the accuracy score.}
% \label{tab:ACCperf}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% Class      &   &           &               &    &           &                          \\
%  of Methods        & \FR  & Mean \Acc        & \Pa              & \Pb    & \Pc          & \PMA                          \\ \hline
% \hline
% \hline
% \GBDT & $1.769 \pm 0.998$ & $0.889 \pm 0.038$ & $0.963$ & $0.881$ & $0.819$ & $0.971 \pm 0.054$\\
% \MLR & $2.913 \pm 1.403$ & $0.882 \pm 0.031$ & $0.963$ & $0.869$ & $0.800$ & $0.956 \pm 0.070$\\
% \RF & $3.056 \pm 1.415$ & $0.882 \pm 0.038$ & $0.912$ & $0.819$ & $0.656$ & $0.958 \pm 0.063$\\
% \GLM & $3.756 \pm 1.561$ & $0.862 \pm 0.060$ & $0.806$ & $0.631$ & $0.463$ & $0.940 \pm 0.062$\\
% \TREE & $4.763 \pm 1.195$ & $0.836 \pm 0.062$ & $0.731$ & $0.381$ & $0.237$ & $0.908 \pm 0.084$\\
% \QDA & $5.675 \pm 1.688$ & $0.723 \pm 0.160$ & $0.338$ & $0.194$ & $0.169$ & $0.796 \pm 0.159$\\
% \Baseline & $6.856 \pm 1.574$ & $0.593 \pm 0.168$ & $0.069$ & $0.025$ & $0.025$ & $0.661 \pm 0.133$\\
% \RNN & $7.213 \pm 0.980$ & $0.565 \pm 0.152$ & $0.025$ & $0.013$ & $0.013$ & $0.625 \pm 0.136$\\
% \hline
% \end{tabular}
% }
% %\label{tab:stat_test}
% \end{table}




% % For binary classification task with the usual accuracy score, \MLR{} is a close second behind \GBDT{} both in terms of Accuracy and AUC scores. 
% % %better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% % %Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% \begin{table}
% \caption{\textbf{Performances of the best in each class of methods} for the classification task with \AUC{} score.}
% \label{tab:AUCperf}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% Class      &   &           &               &    &           &                          \\
% of Methods        & \FR  & Mean \AUC        & \Pa              & \Pb    & \Pc          & \PMA                          \\ \hline
% \hline
% \hline
% \GBDT & $1.738 \pm 1.190$ & $0.918 \pm 0.048$ & $0.938$ & $0.912$ & $0.875$ & $0.963 \pm 0.108$\\
% \MLR & $2.900 \pm 1.304$ & $0.908 \pm 0.012$ & $0.912$ & $0.844$ & $0.694$ & $0.952 \pm 0.106$\\
% \RF & $2.938 \pm 1.390$ & $0.912 \pm 0.047$ & $0.931$ & $0.887$ & $0.706$ & $0.956 \pm 0.095$\\
% \LM & $3.881 \pm 1.572$ & $0.889 \pm 0.060$ & $0.775$ & $0.662$ & $0.475$ & $0.935 \pm 0.094$\\
% \RNN & $4.856 \pm 1.545$ & $0.843 \pm 0.154$ & $0.706$ & $0.506$ & $0.412$ & $0.896 \pm 0.155$\\
% \TREE & $5.975 \pm 1.160$ & $0.813 \pm 0.091$ & $0.394$ & $0.212$ & $0.212$ & $0.852 \pm 0.119$\\
% \QDA & $6.031 \pm 1.371$ & $0.772 \pm 0.149$ & $0.394$ & $0.256$ & $0.150$ & $0.818 \pm 0.152$\\
% \Baseline & $7.681 \pm 1.084$ & $0.499 \pm 0.151$ & $0.006$ & $0.000$ & $0.000$ & $0.537 \pm 0.072$\\
% \hline
% \end{tabular}
% }
% %\label{tab:stat_test}
% \end{table}

% For binary classification task with the usual accuracy score, \MLR{} is a close second behind \GBDT{} both in terms of Accuracy and \AUC{} scores. 
% %better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% %Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% % \textbf{The \MLR{} method clearly outperforms all the compared methods in the regression task.} \BMLR{} with a \Pb{} of $0.72$ on the whole benchmark and Friedman Rank of $3.5$ is far above \RF{}, with a \Pb{} of $0.5$ and Friedman Rank $7.111$ in Table \ref{tab:perfR2_rank}. 
% % As revealed by its \PMA{} statistics at $0.92$%in Table \ref{tab:perfR2_rank})
% % , \BMLR{} is far ahead of the other methods. 
% % %Thus it actually almost never "loses" to the best method by a lot. 
% % This means that \BMLR{} produces reliable results at a rate that is even above methods like \RF{} which are often deemed the safest pick. The same conclusion is also valid for \BMLRa{} and \BMLRb{}.
% % Standard NN (\texttt{NN2}) with equivalent architecture and MSE loss perform poorly with a Friedman rank of $11.722$.





% % For binary classification task with the usual accuracy score, \XRF{} is better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% % Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% % of the is similar  standard deviation of the Friedman rank of the \MLR{} performances are equivalent for the mean \AUC{}, the Friedman Rank (\FR) and the \PMA. 


% % Regarding the accuracy, although \XRF{} is better in terms of mean accuracy, \Pb{}, \Pc{}, the \MLR{} performance is better than \XRF{} in terms of Friedman Rank ($4.0$ for \MLR{}, $4.31$ for \XRF), and worst for the other metrics.


% % AUC: the \MLR{} method produces better discriminating models. Interesting in unbalanced settings.








% % Pas utile vu qu'il y a le Friedman Rank: \textcolor{red}{\textbf{Another important take-away fact is that \MLR{} ranks in the top three on $18$ out of the $21$ datasets, on top of being the best in average.}}


% % As we observe in Tables \ref{tab:perfR2_rank} and \ref{tab:ACCperf}, the depth $L$ in the \MLRL{} method seems to be the only data-dependent hyperparameter. However a simple aggregation of \NN{} of different depths performs as well as %is able to reliably mimic the best performance of 
% % the \NN{} with the most adequate depth for the dataset at hand. 



% %Indeed with a Friedman rank of $\textcolor{purple}{Value}$ on the benchmark, \BMLR{} outperforms all \MLRL{} architectures with a Friedman rank of $\textcolor{purple}{Value}$ at best.

% %\medskip


% % \subsection{Computing time/scalability??????}
% % \textcolor{red}{Computing time raisonable???????}

% % \textcolor{red}{scalability huge datasets ???????}

% % c'est pas le but du papier vu qu'on se concentre sur les petits datasets mais \MLR{} se calcule aussi sur les gros datasets. Cependant le standard NN 

==> Old/rebuttal/C7.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Aug  9 22:13:40 2021
\begin{table}[ht]
\centering
\begin{tabular}{rlll}
  \hline
 & method & ACC & AUC \\ 
  \hline
\hline
\end{tabular}
\caption{} 
\end{table}


==> Old/rebuttal/Response Referee Important/review_response_aout_2021.tex <==
Official Review of Paper5254 by Reviewer 9uXX 
NeurIPS 2021 Conference Paper5254 Reviewer 9uXX
15 Jul 2021 (modified: 16 Jul 2021)NeurIPS 2021 Conference Paper5254 Official ReviewReaders: Program Chairs, Paper5254 Senior Area Chairs, Paper5254 Area Chairs, Paper5254 



Reviewers Submitted, Paper5254 Authors

Summary: 
In their manuscript, the authors introduce a Deep Learning (DL) method for tabular data. Tabular data is a relevant topic for machine learning (ML) and therefore new DL methods, such as the one from the authors, may be highly relevant for NeurIPS. In detail main points of the suggested method are:
usage of ridge regression on the last hidden layer (together with the target) as a closed formula
based on the fixed ridge regression formulas, define new objective instead of the usually optimized MSE or cross entropy which should lead to better regularization
new objective considers permuations of target values
additional noise on target values (regression) or prediction values (classification) The authors state, that their method outperforms other methods on a self-defined benchmark consisting of datasets from UCI and Kaggle.



Main Review: 
NOVELTY: The new objective based on the closed ridge-regression formula, that was introduced by the authors seemed novel to the reviewers knowledge. We are not aware, that others have used the ridge regression formula in the same way, i.e. used it in a Deep Neural Network together with the permutation of target values. Due to the novelty, an experiment such as that described under Major concern 3 would be interesting to better understand the dynamics of networks trained with this objective.

RELEVANCE: The new objective together with the permutation idea might be interesting to the ML community, in case it consistently performs better compared to previously used DL objectives or if it performs consistently at least as good as traditional ML methods (e.g. Random Forests, Gradient Boosting). The experiments try to show the superiority of the new objective at least for the regression setting. However the experiments are not yet fully convincing to us (see technical correctness).


CLARITY: The method itself is clearly described, however there are missing details and open questions on the experimental setup, especially a list which datasets from UCI and Kaggle have been used for the benchmark (see Major concern 1 for the open questions and Major concern 2 for dataset related aspects).


TECHNICAL CORRECTNESs: There are doubts due to missing details and the evaluation on a self-defined benchmark, whether the comparison to other methods were done in a fair way. The reviewers therefore ask to provide further details and an extended experimental setup to be able to better judge this point (see Major concern 1). Further, the term "memorization" is unclear (see Major concern 3).




Major concerns:
It seems strange, that a plain neural network is that much worse (e.g. FFNN in Table 4) than using ridge regression. It would therefore be interesting to have more details on the network architecture and training of this neural network and also pre- and postprocessing for this neural network architecture (e.g. were the inputs and output standardized to mean zero and variance 1?). In order to judge, whether the new objective function is really the cause of the performance improvement, this needs to be known.
Question: Did the authors use the exact same FFNN code (up to their new ideas for the objective function) for the compared plain FFNN or NN (with MSE or cross-entropy as objectives)? (wrt. to this question: Why did the authors cite fast.ai for NN? Is the code for the simple FFNN based on this and is also the advanced version with the new objective based on this?) What is the reason for stating "Aberating value" in Table 5?
Suggested new experiment during the rebuttal phase, that could substantially change our opinion: We suggest to compare with a self-normalizing neural network (SNN) [1] and with a network with Batch-Normalization after each hidden layer, where the authors should try to compare the objective function from their manuscript with MSE and cross-entropy as objective functions. Thereby the inputs and the outputs to the network should be appropriately standardized for the traditional objective functions (MSE, cross-entropy) and rescaling should be applied in the prediction step. We suggest to carry this experiment out on a classification task (especially the Tox21 dataset) and a regression task (especially the Lipophilicity dataset) from MoleculeNet [2] with ECFP features provided from their software package. Ideally predefined test sets (in case they have been made available in MoleculeNet) should be used for evaluation. It would be appreciated if the code to reproduce results of this suggested experiment will be made available to the reviewers.
Chosen experimental datasets There are missing details which datasets are included in the benchmark. A table with details on the dataset name, the number of instances, features, etc. would be helpful. The authors should specify the exact criterions for choosing a UCI dataset to be part of the benchmark or for keeping a dataset away from the benchmark. To our point of view, there is always the danger that the selection of datasets to the benchmark may be the result of a pre-analysis of results on a much larger set. For a possible camera-ready version, we suggest to extend the experiments after the rebuttal on all MoleculeNet datasets, where the input data is fully-described by SMILES and ECFP features can be constructed from it.
Memorization In the abstract it is stated, that MLR penalizes memorization. The authors should either 
more exactly formalize, what the mean with "memorization" and accordingly show related experiments and/or proofs that show how this is achieved or
consider to change the abstract and text.
Especially it would be interesting how their method would work for completely random targets or randomly permutated targets, that are considered to be the ground truth for the machine learning method (see e.g. [3]), i.e. could random labels be learnt with the author's new objective that includes the random permutations? Thereby it would be of interest to check this for networks with a large number of units and layers.
Minor concerns:
page 4, line 125: This effect is much stronger than adding a constraint...: What effect do you concretely mean? What does this statement mean, if a penalty parameter of e.g. 10^20 is chosen for weights being usually ~ N(0,1)?
Supp. page 2, line 30: "However SNN requires careful tuning of hyperparameters and does not outperform SVM or RF on the UCI database." Even if the method did not show statistical significance on their UCI experiments, in their ranking it was still better than SVM and RF. Further it seemed to be the best FNN baseline and could therefore serve to be a valuable baseline. The SNN authors seemed to apply a careful hyperparameter selection for all methods included in their comparison. When comparing the tables on hyperparameter selection in their appendix for the different methods, we don't have the impression that hyperparameter tuning for SNNs is overwhelming.
Question: In the case of a single sample, is 1-R^2 for all your experiments directly proportional to the MSE or did you use some other formula for the computation of R^2? The authors did not explicitly discuss limitations of their approach in the conclusion. These would be especially interesting with respect to numerical instabilities, runtime and their hyperparameter selection in general.
[1] Klambauer et al. Self-Normalizing Neural Networks [2] Wu et al. MoleculeNet: A Benchmark for Molecular Machine Learning [3] Zhang et al. Understanding deep learning requires rethinking generalization
Limitations And Societal Impact: 
Missing completely. There was no discussion on negative societal impact or ethical concerns of their work (although the authors marked "Yes" in the checklist), which however would seem quite a stretch for us for such basic type of research. 
Ethical Concerns: 
Needs Ethics Review: No
Time Spent Reviewing: 3
Rating: 4: Ok but not good enough - rejection
Confidence: 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
Code Of Conduct: While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.
AddOfficial Comment
[–]
Official Review of Paper5254 by Reviewer xwHX 
NeurIPS 2021 Conference Paper5254 Reviewer xwHX
12 Jul 2021NeurIPS 2021 Conference Paper5254 Official ReviewReaders: Program Chairs, Paper5254 Senior Area Chairs, Paper5254 Area Chairs, Paper5254 Reviewers Submitted, Paper5254 Authors
Summary: 
This paper proposes several regularization recipes to improve multi-layer neural networks on tabular data. Specifically, the authors propose to use a closed form ridge regression on the last layer, and panelize the loss function with randomly permuted labels.
Main Review: 
On the positive side, this paper studies a relevant problem of improving the generalization of multilayer neural networks on tabular data. The authors included a comprehensive dataset in the empirical evaluations. The author presented all the recipes(ridge regression, random permutation, structure dithering) clearly. 
It seems that the entire dataset needs to be used due to the explicit form of ridge fitting. This makes the proposed approach diverge from the SGD approach that most NN training takes. It may also prevent existing techniques, such as dropout, to be used in the learning process. It would be interesting to see the impact in terms of the training cost.
While the paper discusses the previous works, the existing MLP-based tabular data methods are not included in baseline studies. It would be useful to include some of them in the empirical evaluations. Additionally, bagging and ensemble are used in the presented results, which could be unfair to some of the baselines -- since it is commonly known that bagging and ensemble will improve over baseline results. 
Besides the aggregated statistics of all the experiments, it may also be helpful to present results of a few selected datasets to show additional insights.
In summary, this paper can be further improved by adding additional discussion about the cost of training(compared to SGD based methods), including additional baselines, and disentangling the benefit bought by ensemble.
Limitations And Societal Impact: 
NA
Needs Ethics Review: No
Time Spent Reviewing: 1
Rating: 5: Marginally below the acceptance threshold
Confidence: 5: You are absolutely certain about your assessment. You are very familiar with the related work and checked the math/other details carefully.
Code Of Conduct: While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.
AddOfficial Comment
[–]
Official Review of Paper5254 by Reviewer rPMv 
NeurIPS 2021 Conference Paper5254 Reviewer rPMv
12 Jul 2021NeurIPS 2021 Conference Paper5254 Official ReviewReaders: Program Chairs, Paper5254 Senior Area Chairs, Paper5254 Area Chairs, Paper5254 Reviewers Submitted, Paper5254 Authors
Summary: 
The paper introduces Muddling Labels for Regularization (MLR): a new dense neural network architecture for prediction on tabular datasets. This architecture is special because of
(1) a last layer whose weights are computed in closed form from Ridge regression (MLR-NN), and 
a loss objective that includes 
(2) label noise (dithering) and
(3) a label-permutation–based loss to guard against overfitting.
Main Review: 
Summary
While the proposed architecture is interesting, the presentation is lacking in clarity and motivation. Further, the experimental evaluation is inadequate, as hyperparameters for baselines are not tuned. I therefore would not recommend acceptance.
Strengths
Although the MLR-objective has previously been published in an ArXiv paper, the general idea of the architecture is somewhat interesting: computing the last layer weights of the network in closed form is at least quirky, and so is the permutation-based loss. (The authors gloss over this, but the scope of the previous publication of the MLR-objective does seem substantially different.)
Weaknesses
1) Proposed approach

The paper is lacking in clarity and does poor job of conveying the main conceptual ideas.
Specifically, the MLR network and objective and the label-permutation based-loss took multiple iterations of reading and ultimately looking at the code, before understanding what exactly is happening in MLR.
For the interested, here is my summary:
The MLR-NN replaces the last layer of a standard dense neural network with a 'ridge regression layer':
Instead of learning the weights of the last layer, the authors compute the weights from the last layer as the closed-form solution to a ridge regression problem (linear regression with L2 regularisation, taking the output of the second-to-last layer as inputs and the training targets as targets).
The prediction is now an explicit function of the training targets Hy, because the closed-form solution depends explicitly on the training targets y. H combines the NN feature extractor layers and the matrix inversions from the closed-form solution.
This will give problems with overfitting in naive application, as zero training loss through memorisation is trivial to achieve with a diagonal H. This is why the paper introduces a auxiliary label permutation loss (see below).
They perform this in each forward pass and backpropagate through the ridge regression layer to train the weights for earlier layers in the network.
Therefore, the 'label permutation' component in the loss regularises the network against learning a diagonal H through an implicit mechanism. This term 'quantifies the amount of memorization', by checking if the model still predicts correctly for randomised targets. This is a possibility because the prediction at training time explicitly depends on these randomised targets and if the matrix H is diagonal, which gives 0 training loss, the model will just predict permuted labels. Such behaviour therefore needs to be guarded against with the auxiliary label permutation loss.
Motivation:
Unfortunately, it is unclear to me why this architecture is a good idea. The authors do not provide sufficient motivation. It is unclear what explicit benefits this approach should give over a standard MLP with L2 regularisation, and the authors do little to provide motivation or intuition. (Confusingly, the authors claim that the ridge regression provides 'much stronger' regularisation than adding standard L2 weight regularisation to the loss. No further justification is given. This statement seems at odds to me with the fact that they need to introduce the permutation loss to add further regularisation.)
Clarity:
Clarity of the paper is severely lacking, and I struggled hard to extract the above information from the paper.
Quality of Experimental evaluation

There are some very debatable choices in the experimental evaluation that are not really acceptable IMHO.
For one, the authors explicitly do not tune hyperparameters of baselines (l. 134 Appendix) but do not give justification for this.
On the other hand, for their architecture, they evaluate a large variety of models (4 baseline models with different learning rates/layers/etc., bagging versions of multiple MLR models, an ensemble of MLR models, additional aggregations of multiple MLR models based on validation loss) and report the best results. This is clearly an implicit hyperparameter search for MLR. Given that hyperparameters are not tuned for baselines and that baselines do not get to benefit from additional ensembling/bagging this constitutes an unfair advantage of MLR over the baselines. It is also in contrast to the paper's claim that their method works without hyperparameter tuning.
Given how much hyperparameter tuning matters for the chosen baselines, I therefore doubt the result that the proposed approach outperforms standard baselines.
The authors also do a good job of introducing recent work in deep learning for tabular datasets, but then fail to include any of them in the experimental comparison.
Reproducibility
The code is given in a single Jupyter Notebook for experiments on the Boston dataset. Describing this as an 'open source package' (supplement p.1) seems somewhat over the top. I have not run code, but the Notebook looks decent (despite it being left in a somewhat messy state). For other experiments, there is no code.
Additional feedback
If you use mini-batching, which training set Y do you plug in at test time? I could not find information for this in the paper. From the code, it looks like this would be just the set of targets from the last train minibatch. This does not seem very principled.
The authors claim that 'using wider architecture and bigger batch size is always better' (l.172). While this may be true for MLR, as the appendix indeed suggests (alas not cited in l. 172), this is certainly not true for deep learning in general. It might be good for you to clarify what you mean here, to not upset future readers.
You could cite the extensive literature around Ridge Regression.
Instead of using the same data for calculating the ridge regression parameters and the loss, have the authors considered splitting the (minibatches of the) data in two? This would avoid the trivial solution of diagonal H as the targets Y in eq 4 no longer match the input. Or how about you simply permute y after computing the ridge regression solution, such that it looks different for the forward pass? Alternatively: instead of using the (somewhat expensive) permutation based loss, why not regularise against diagonal H more directly?
This paper could use a thorough check of grammar/spelling/equations as some parts seem a bit sloppy / wrong. For example,
(l. 18): medecine --> medicine
(l. 180): GVRAM ?
(l. 164): closing bracket for λ(k^) escaped superscript
(l. 166): an hyperparameter → a hyperparameter
(Also, maybe check out the NeurIPS style guide on how to make tables more pretty with booktabs.)
Limitations And Societal Impact: 
Limitations: Under 'scalability' in the supplement, the authors briefly claim that the 'main limitation is the size of the GPU VRAM with a current maximum of 32G on the best available configuration', but I am not sure why exactly they would need larger RAM? They seem to be aware that the matrix inverses of the ridge layer are an expensive component of MLR-NN, but claim that the cost of matrix inversion is 'linear on a GPU thanks to parallelisation'. (In the main paper on p. 4 they have some citations for that, but I am not sure this actually claim holds in practice.)
Soc. Impact: I cannot find a societal impact section in either the submission or the supplementary pdf, despite the authors answering the checklist question on that with 'yes'.
Ethical Concerns: 
None.
Needs Ethics Review: No
Time Spent Reviewing: 5
Rating: 3: Clear rejection
Confidence: 5: You are absolutely certain about your assessment. You are very familiar with the related work and checked the math/other details carefully.
Code Of Conduct: While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.
AddOfficial Comment
[–]
Official Review of Paper5254 by Reviewer 8J2E 
NeurIPS 2021 Conference Paper5254 Reviewer 8J2E
09 Jul 2021 (modified: 09 Jul 2021)NeurIPS 2021 Conference Paper5254 Official ReviewReaders: Program Chairs, Paper5254 Senior Area Chairs, Paper5254 Area Chairs, Paper5254 Reviewers Submitted, Paper5254 Authors
Summary: 
In this paper, the authors propose an end-to-end deep learning framework to train a standard FFNN for tabular data with a novel regularization techinique, named the Muddling Labels for Regularization. Specifically, the regularization method applies the L_2 ridge regularization on the last hidden layer of the neural network with a subset of labeled data being randomly permuted and the structured dithering schema to prevent memorization. Extensive experiments are conducted on 32 datasets (16 regression and 16 classification) to demonstrate the performance of the proposed model. Overall, the paper is well-written and fairly easy to follow. The experimental details and code are provided to help reproduce the results. 
Main Review: 
In this paper, the authors propose an end-to-end deep learning framework to train a standard FFNN for tabular data with a novel regularization techinique, named the Muddling Labels for Regularization. Specifically, the regularization method applies the L_2 ridge regularization on the last hidden layer of the neural network with a subset of labeled data being randomly permuted and the structured dithering schema to prevent memorization. Extensive experiments are conducted on 32 datasets (16 regression and 16 classification) to demonstrate the performance of the proposed model. Overall, the paper is well-written and fairly easy to follow. The experimental details and code are provided to help reproduce the results. However, the experiment section is incomplete and thus make the evaluation inconclusive. In addition, this paper is primarily empirically motivated (ie. there is no theoretical justification on the chosen regularization technique).
The incompleteness of the experiment section:
A. Missing relevant deep learning methods as the benchmarks: No deep learning methods are included as benchmarks even though those methods have claimed their outperformance over GBDT (on a limited number of datasets). In addition, TabNet is claimed to be able to consistently outperform GBDT in table 1. Thus it would be interesting to see its performance over authors' proposed model.
B. No HPO tuning for tree-ensemble models as the benchmarks. In supplemental material table, the authors mentioned "All methods of XGBoost, CatBoost, LightGBM were ran with the default hyperparameters." The number of experimental datasets in this paper is large, 32 totally and thus a single set of hyper-parameters cannot work well with all of them, making the evaluation inconclusive. 
C. The authors proposed a deep learning framework with a particular regularization method. However, there is no comparison between his regularization method and other standard regularization techniques (such as solely L2 regularizations on all of parameters or dropout).
There is no theoretical justification on the chosen regularization technique. The proposed regularization techniques are generally proposed to prevent overfitting. But the authors did not give a good explanation on why overfitting is such a general issue in tabular modeling with deep learning? I saw the cited paper "UNDERSTANDING DEEP LEARNING REQUIRES RETHINKING GENERALIZATION" discusses the overfitting issue in vision domain. But it may not be the same case for tabular data.
Some questions:
A. Why the L2 regularization is only applied to the last hidden layer instead of all of parameters? A good justification should be provided.
B. The number of neurons J in each hidden layer is constant and set as a very large value 2^10. Will the model be over-parameterized when the input dimension is less than 10? (See table 2 in supplemental material there are many datasets having input dimension less than 10 after preprocessing) and thus a regularization method has to be applied to overcome such over-parameterization? Also, the author justified the decision to set the number of neurons J to be as large as possible by only 3 datasets in the supplemental material, which is not very convincing. 
Limitations And Societal Impact: 
NA.
Ethical Concerns: 
NA.
Needs Ethics Review: No
Time Spent Reviewing: 3
Rating: 4: Ok but not good enough - rejection
Confidence: 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
Code Of Conduct: While performing my duties as a reviewer (including writing reviews and participating in discussions), I have and will continue to abide by the NeurIPS code of conduct.

==> Old/rebuttal/overall_HPO_reg_fried.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Sun Aug 15 19:08:41 2021
\begin{table}[ht]
\centering
\caption{Overall performance comparison of models with HPO but without ensemble for the regression task over the 16 regression datasets} 
\label{tab:HPO_R2_Fried}
\begin{tabular}{rllllrrr}
  \hline
 & method & mean.R2.score & F.Rank & PMA & P90 & P95 & P98 \\ 
  \hline
1 & CatBoost & 0.721 & 1.794±0.862 & 0.935±0.267 & 0.86 & 0.84 & 0.73 \\ 
  2 & RF & 0.707 & 2.688±1.047 & 0.944±0.107 & 0.86 & 0.71 & 0.56 \\ 
  3 & MLR & 0.717 & 2.7±1.302 & 0.944±0.15 & 0.86 & 0.76 & 0.58 \\ 
  4 & XgBoost & 0.703 & 2.819±0.903 & 0.913±0.245 & 0.84 & 0.71 & 0.50 \\ 
   \hline
\end{tabular}
\end{table}


==> Old/rebuttal/overall_reg_HPO.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Mon Aug  9 23:06:07 2021
\begin{table}[ht]
\centering
\caption{Overall impact of HPO and Ensemble on R2-test performance for the regression task over the 16 regression datasets} 
\label{tab:overallhpo}
\begin{tabular}{rllll}
  \hline
 & method & R2 & Bagging.R2 & Ensemble.R2 \\ 
  \hline
1 & CAT & 0.721±0.049 & 0.723±0.048 & 0.724±0.047 \\ 
  2 & MLR & 0.717±0.051 & 0.739±0.042 & 0.739±0.042 \\ 
  3 & RF & 0.707±0.044 & 0.709±0.044 & 0.711±0.045 \\ 
  4 & XGB & 0.703±0.051 & 0.712±0.048 & 0.713±0.045 \\ 
   \hline
\end{tabular}
\end{table}


==> Sections/old_experiments.tex <==

\subsection{\TD{} benchmark results}
\textbf{There is no such thing as "SOTA" for \TD.} In our benchmark, the most proficient method, CatBoost, is beaten on 43 out of the 67 datasets we used. The set of existing competitive methods is very large. Out of the 30 candidate methods we included in our study, 20 outperformed all others on at least one dataset. Methods which are neither GBDT, \DNN{} or $\RF$ based are not included in any \textcolor{red}{aforementionned (pas mentionn\'e avant} benchmark. Yet, they outperformed all other methods on $9$ datasets which is more or less the number of datasets considered in these benchmarks. We tried $5$ different implementations of GBDT, Catboost was beaten by at least one of those on $?$ datasets.









\paragraph{Benchmark description.} \TD{} are very diverse. %creating an appropriate benchmark is still an ongoing process for ML research community.
\textcolor{red}{Plus de details sur l'origine des jeux de donnees.}
We included 67 datasets from Kaggle, Uci and openml covering diverse domains with sample size ranging from $57$ to $11M+$ and the number of features from $4$ to $4K+$, with a diverse range of continuous/categorical mixtures. The tasks include $31$ regressions, $24$ binary classification and $13$ multiclass.\\
% $\bullet$ There is no such thing as "SOTA" for \TD. In our benchmark, the most proficient method, CatBoost, is beaten on 43 out of the 67 datasets we used. The set of existing competitive methods is very large. Out of the 30 candidate methods we included in our study, 20 outperformed all others on at least one dataset. Methods which are neither GBDT, \DNN{} or $\RF$ based are not included in any \textcolor{red}{aforementionned (pas mentionn\'e avant} benchmark. Yet, they outperformed all other methods on $9$ datasets which is more or less the number of datasets considered in these benchmarks. We tried $5$ different implementations of GBDT, Catboost was beaten by at least one of those on $?$ datasets.\\
%These includes "old" methods like Lasso and ElasticNet, Support Vector Machines and different implementations of currently popular methods (like the scikit learn implementation of XGB and Neural Networks!). Meanwhile, methods which are neither GBDT, \DNN{} or $RF$ based are not included in any aforementionned benchmark. Yet, they outperformed all others on $9$ datasets which is more or less the number of datasets considered in these benchmarks. %\textcolor{red}{Therefore it is not possible to get an accurate picture when we test only a handful of methods on a dozen tabular datasets.}\\
%$\bullet$ \textcolor{red}{fusionner avec la description du jeux de donnees}. 
Data scarcity is a frequent issue in tabular learning tasks \cite{Chahal2021Small}. 
%\TD{} are frequent in many applications \cite{FENG2019300,JTD4418,Rajkomar2018,Cassotti2015similarity-based}. 
Transfer learning is almost never applicable for TD, so handling the small sample regime is often an important issue. We included $32$ datasets with less than $1000$ observations. For all large datasets, we repeated all experiments for different train sizes.\\
%$\bullet$ limited compute budget \cite{contardo2017} \textcolor{red}{add a sentence d'une de nos intros precedentes}\\
$\bullet$  Although HPO can drastically increase the performance of some methods on some large datasets, it also most often multiply the compute cost by a factor of $500$ ($5$ Fold CV $*$ $100$ iterations).  We did experiment on HPO on a subset of datasets nonetheless.\\
$\bullet$ and META learning schemes\textcolor{red}{a completer}\\
$\bullet$  Handling categorical features is another difficult challenge in \TD{}, but beyond the scope of this paper. We only applied \trainmet{} to simple architectures combined with one-hot-encoding. We implemented MLP with either dense layers, resblocks, gated linear units, or SELU activations.  We always used $Adam$ and $OneCycleLearningRate$ with early stopping. We used $batch norm$ and $dropout = 0.1$ for regular \DNN{} and no explicit regularization scheme for \trainmet{}. Table ... details the characteristics of each architecture evaluated.\\
 
 \paragraph{main takeaways} 
\textbf{There is no such thing as "SOTA" for \TD.} In our benchmark, the most proficient method, CatBoost, is beaten on 43 out of the 67 datasets we used. The set of existing competitive methods is very large. Out of the 30 candidate methods we included in our study, 20 outperformed all others on at least one dataset. Methods which are neither GBDT, \DNN{} or $\RF$ based are not included in any \textcolor{red}{aforementionned (pas mentionn\'e avant} benchmark. Yet, they outperformed all other methods on $9$ datasets which is more or less the number of datasets considered in these benchmarks. We tried $5$ different implementations of GBDT, Catboost was beaten by at least one of those on $?$ datasets.




% \begin{table}[h]
% \label{tab:architectureinfos}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||l|c|c|l|c|c|c|c|}
% \hline
% Name  &  Block Type & \# Blocks &  Block Depth & Activation & Width & Iter/epochs & Batch-Size & max lr\\
% \hline
% \hline
% fast & Linear & $2$ & $1$ & ReLU & $256$ & $200$ & $min(n,2048)$ &  $1e-2$ \\
% standard & Linear & $2$ & $1$ & ReLU & $512$ & $500$ & $min(n,2048)$ & $1e-2$ \\
% wide & Linear & $2$ & $1$ & ReLU & $2048$ & $1000$ & $min(n,2048)$ &  $1e-3$ \\
% batchstandard & Linear & $2$ & 1 & ReLU & $512$ & $20$ & $256$ &  $1e-2$ \\
% fastselu & Linear & $2$ & $1$ & ReLU & $256$ & $200$ & $min(n,2048)$ &  $1e-2$ \\
% selu & Linear & $2$ & $1$ & SeLU & $512$ & $500$ & $min(n,2048)$ & $1e-2$ \\
% resblock & Residual & $2$ & $2$ & ReLU & $512$ & $500$ & $min(n,2048)$ & $1e-2$ \\
% resblockwide & Residual & $2$ & $2$ & ReLU & $2048$ & $1000$ & $min(n,2048)$ &  $1e-3$ \\
% batchresblock & Residual & $2$ & $2$ & ReLU & $512$ & $50$ & $256$ &  $1e-2$ \\
% glu & Gated Linear & $3$ & $1$ & ReLU/Sigmoid & $512$ & $500$ & $min(n,2048)$ &  $1e-2$ \\
% reglu & Gated Linear & $3$ & $2$ & ReLU/ReLU & $512$ & $500$ & $min(n,2048)$ & $1e-2$ \\
% resglu & Gated Residual & $2$ & $2$ & ReLU/Sigmoid & $512$ & $500$ & $min(n,2048)$ & $1e-2$ \\
% resreglu & Gated Residual & $2$ & $2$ & ReLU/ReLU & $512$ & $500$ & $min(n,2048)$ & $1e-2$ \\
% \hline
% \end{tabular}
% \caption{\FFNN{} architectures included in our benchmark. Legend for Block type: L=Linear; Res=Residual,GL=Gated Linear; GR=Gated Residual}
% \end{table}










\paragraph{Performance evaluation metrics.}
$\bullet$ For each dataset, we used the following train-test split strategies: we did $10$ random $80/20$ train-test split without stratification. We also did $10$ train-test splits with train sizes in $\left\lbrace 50 * 2^d,\; 0\leq d\leq 8 \right\rbrace$ with stratification (for both regression an classification tasks).\\
$\bullet$ For each non-deterministic method, we used $1$ random seed for each train-test split, and evaluated on both train and test set the $R2-score$ and $RMSE$ or $Accuracy$ and {\it Area Under Curve} for regression and classification respectively (in a {\it one-versus-rest} fashion for multiclass).\\


\paragraph{Compared methods.} \textbf{There is no such thing as "SOTA" for \TD.} In our benchmark, the most proficient method, CatBoost, is beaten on 43 out of the 67 datasets we used. The set of existing competitive methods is very large. Out of the 30 candidate methods we included in our study, 20 outperformed all others on at least one dataset. Methods which are neither GBDT, \DNN{} or $\RF$ based are not included in any \textcolor{red}{aforementionned (pas mentionn\'e avant} benchmark. Yet, they outperformed all other methods on $9$ datasets which is more or less the number of datasets considered in these benchmarks. We tried $5$ different implementations of GBDT, Catboost was beaten by at least one of those on $?$ datasets.

We included in our study \Catboost{} \cite{Prokhorenkova2018}, \XGBoost{} \cite{guestrin2016}, \lightgbm{} \cite{Ke2017} ), \MARS{} \cite{Friedman1991} (using the py-earth implementation) and the scikit learn implementation of \RF{} and \XRF{} \cite{breiman2001,barandiaran1998random}, Ridge Kernel and Nu-\SVM{} \cite{Chihchung2011}, \MLP{} \cite{Hinton89connectionistlearning}, \Enet{} \cite{Zou05}, \Ridge{} \cite{Hoerl1970}, \LAS{} \cite{tibshirani1996}, \texttt{Logistic regression} \cite{cox1958}, \texttt{CART}, \texttt{XCART} \cite{Breiman1984,gey2005model,Klusowski2020sparse}, \Adaboost, and \XGB{} \cite{Breiman1997_arcing,Friedman2001,Friedman2002}.


See Appendix \ref{app:datamodellist} for the exhaustive lists of methods and the description of datasets included in our benchmark as well as our preprocessing.


\paragraph{\DNN{} training protocol.}

\paragraph{Overall performance comparison.} For concision, we precise for each method the number of times it outperformed all others as $METHOD$, $R:x$, $CLF:y$ where $x$ is the number of datasets for regression and $y$ is the number for classification.\\
$\bullet$ For GBDT algorithms we included Catboost with default hyperparameter values. In agreement with its reputation, it outperformed the other models on more datasets than any other method, but still in a minority of cases. Please note this came at the cost of compute time, since it is also the slowest one with an average training time of $?$ which is not really in tune with our benchmark philosophy. We also evaluated CATboost with  another set of hyper-parameters designed to improve the time/performance tradeoff. It divided average training time by $?$ and still outperformed all other methods on $ $ datasets. We also included XGBoost $ ?$, LightGBM $ ?$, and the scikit learn implementation of $xgb$ $ ?$, and adaboost $? $. This means that even less popular implementations of GBDT are still relevant.\\
$\bullet$ For other tree based methods, we included the scikit learn implementations of $\RF$ $ ?$, $\XRF$ $ ?$, $\CART$ $ ?$ and $\XCART$ $ ?$. Noticeably, $\XRF$ outperforms $\RF$ on $?$ out of $?$ datasets.\\
$\bullet$ Linear models (\LAS{} $?$, \Enet{} $?$, \Ridge{}  $?$, Logistic Regression $? $) are the only ones where we allowed moderate HPO, picking the regularization level with cross validation. Noticeably, \LAS{} and \Enet{} outperformed all other models in $?$ out of the $?$ datasets with more than $?$ features.\\
$\bullet$ We also included Kernel $? $ and NuSVM $? $, and the pyearth implementation of Multivariate Adaptive Regression Splines (MARS) $? $.

These results are in accordance with the aforementionned philosophy, only $?$ methods never came first. 




%CatBoost is usually lauded as the best method for tabular data. In our benchmark, CatBoost was the best model as it outperforms all others models on 30 \% of the datasets, far ahead the second best method. \textbf{But this also means that on 70\% of the datasets, the best method was not CatBoost.}



% $\bullet$  Handling categorical features in \T is another difficult challenge,and beyond the scope of this paper. We included simple architectures (MLP, ResNet, SNN) combined with one-hot-encoding but not (eg. NODES, TABNET,...), each time with and without using \trainmet{}.



Il manque un point sur
\textcolor{red}{COMMENTAIRE IMPORTANCE SMALL DATASETS: few shot learning??? \cite{Ng2016Nuts,Chahal2021Small}}



% See Appendix \ref{app:datamodellist} for the exhaustive lists of methods and the description of datasets included in our benchmark as well as our preprocessing.

%Given a large computation budget, and a large number of samples, which is not the case for most practionners in most cases

\paragraph{Behavior and Properties of \trainmet{} w.r.t \FFNN{} architecture}

- trainmet marche mieux avec des réseaux larges\\
- trainmet marche mieux avec des batch larges\\
- trainmet se combine très bien avec resblock, très mal avec dropout et batchnorm\\
- trainmet requires earlystopping\\
- Il faut pas mettre de coefficient devant les termes de MLR ça marche moins bien.\\
- Commentaire sur l'impact de la profondeur sur trainmet\\





\paragraph{Comparison training \FFNN{} without and without \trainmet{}.}

- sur les petits modèles trainmet est bcp plus long que la méthode classique, sur les gros modèle c'est pas le cas\\
- trainmet loss match beaucoup plus la perf de généralization que la loss normale (et on devait s'y attendre!)\\
- trainmet loss est beaucoup plus stable que standard loss, beaucoup/pas d'estimation \\
- trainmet est-il plus fiable que regularnet? plus souvent dans le top? Moins de fois très mauvais?\\


- Trainmet marche bien aussi avec des convnets, la plus value est très importante sur un trainset plus petit\\
\paragraph{What \trainmet{} is good at.}
- Adacap is much more appropriate for regression tasks: it never came first for classification (NN only came first 3/ 21 times actually anyway) but it came first 6 / 27 times in regression.
We will know focus on regression:
- IF we compare only NN with GBDT: Without including Adacap in the picture, Deep NN come first 9 times out of 31, By adding Adacap to the mix of available NN tricks, we get the NN family to win 12/31 times (Adacap is best 8 times) Meaning the DNN family wins 50\% more often with the addition of Adacap against Catboost.
- If we include all families: without adacap : GBDT wins 16, NN 7 RF 4 SVM 2 GLM 2, meanwhile, with adacap : GBDT wins 16, NN+Adacap 8 Adacap 6 , RF 4 SVM 2 NN 2 GLM 1
- If setting a time budget, the number of times Adacap + NN comes first vary a lot:
for 1sec :0/1, for 10sec 5/4, for 60sec 6/2, 
- In terms of average RMSE, the pictures is more favorable to Adacap, which has a decisive impact on average performance. Being good all around leads to low average RMSE. There, the best Adacap architecture (selu) comes at 0.413024, Catboost at 0.417636, while without adacap, the best regular NN (glu) at 0.422760, RF at 0.438172, NuSVM at 0.472135, MARS at 0.493821, Enet at 0.499256	
 - On datasets with high signal to noise ratio (the 9/31 datasets for which the best possible RMSE is under 0.3, Adacap+resnet+glu comes at 0.161896 (Adacap+selu at 0.164808) regular NN (glu) at 0.165464, Catboost at	0.200510. Noticeably these 9 datasets have a diverse number of samples : 82, 167, 245, 512, 7008, 8000, 36584 but always a somewhat low number of features: 7,  9, 13, 15, 22, 26.
 - In terms of time comparison, Best Adacap (selu with 2 hidden layers) takes 20.709967 in average on the 27 seven regression datasets, Catboost 96.610780 seconds and NN glu (3layers deep) 10.382365 seconds. RF takes 4.010701 nuSVM 13.213286 MARS 1.741683 Enet 0.290724 and CART 0.066393. What is very interesting is that Adacap is faster than regular net for some big architectures: for resblock, 17.830224 vs 18.747128
 - In terms of time comparison on the 15 datasets with less then 1000 samples, Best Adacap (selu with 2 hidden layers) takes 4.528561 seconds in average on the 15 seven regression datasets, Catboost 38.132730 seconds and NN glu (3layers deep) 4.854471 seconds. RF takes 0.302734 nuSVM 0.065009 MARS 0.287235 Enet 0.246365 and CART 0.005134. What is very interesting is that for these small datasets, Adacap is faster than regular net for some big architectures: for resblock, 3.567358 vs 4.252559
-REFAIRE TIME COMPARISON AND AVERAGE RMSE AVEC: mise GEN à 0 si erreur
 
 
 
 

- Adacap is much more appropriate for regression tasks: it never came first for classification (NN only came first 3/ 21 times actually anyway) but it came first 6 / 27 times in regression

- Avec budget temps limité



\paragraph{What \trainmet{} is good at.}
- trainmet est le plus utile pour aller chercher les derniers points de généralisation sur des jeux de donnée midsize\\

\paragraph{Few shot learning.} 

-\cite{Ng2016Nuts,Chahal2021Small}\\
- trainmet marche bien aussi avec des convnets, la plus value est très importante sur un trainset plus petit\\

- Pour le même dataset, selon la taille du train size le classement des méthodes peut changer du tout au tout, besoin de tester plusieurs trainsize pour comprendre\\


\paragraph{HPO vs bagging}

- En faisant du bagging on peut améliorer significativement ça peut être bcp plus efficace et bcp moins cher \\

\paragraph{Meta Learning}
- En faisant du métalearning on peut dépasser la meilleure méthode avec d'autre, donc la meilleure méthode suffit pas\\


\paragraph{Where are we at on Tabular datasets?}

- C'est important d'avoir une diversité de dataset et méthodes\\
- Commentaire sur la taille des données qui cela favorise\\
- Les méthodes les plus réputées le sont quand même pour de bonnes raisons\\
- Catboost reste l'algo qui marche le mieux le plus souvent\\
- trainmet est parfois meilleur\\
- Plein de méthodes différentes sont parfois les meilleurs il faut continuer à tester plein de méthodes sur les benchmarks\\
-Il y a pas vraiment un trade off temps performance, les temps de calcul varient énormément entre méthodes, et entre implémentations\\
- c'est quoi les méthodes qui sont jamais les meilleurs, c'est lesquels qu'on peut commencer à exclure, qui sont toujours moins bonne qu'une autre?\\
- les métriques utilisées impactes beaucoup les résultats du benchmark, R2 vs RMSE\\
- Le nombre de seed est important pour le découpage train test, d'une seed à l'autre les résultats peuvent bcp changer.\\
- Les tabular dataset c'est encore un champ très ouvert, on peut pas pour l'instant choisir une solution unique ou même restreindre à quelques candidats.\\




\paragraph{A classer.}

Voir : % http://proceedings.mlr.press/v139/acar21a/acar21a.pdf
- à feature équivalente, si on change la target on a le classement qui change, l traitement des features fait pas tout\\


- La gestion des features catégorielles est pas le seul axe d'amélioration, sur des jeux de données sans feature cat il y a encore bcp de chose à dire/à faire.\\
- C'est important de regarder les tailles de données, ça suffit pas de regarder juste la classification. \\
- shrinkage peut déjà améliorer beaucoup, ensuite MLR est une upgrade\\
- La seed influence surtout le train valid cut pour l'early stopping, pas le choix des permuts\\
- trainmet est-il parfois vraiment bien meilleur que les autres? \\







\paragraph{Deja inclus dans la discussion benchmark description.}

- beaucoup de dataset + beaucoup de seed + beaucoup de méthodes = coûte cher et compliqué, tâche trop générale, il faudrait peut être restreindre ou segmenter le problème pour pouvoir mieux progresser.\\



\subsection{BENCHMARK AND TABULAR DATASETS}
 We illustrate the potential of \trainmet{} on a benchmark containing \textcolor{red}{67} tabular datasets in regression (\textcolor{red}{31}), binary (\textcolor{red}{24}) and multiclass (\textcolor{red}{13}) classification, against a large set of popular methods(\XGB{} \cite{Breiman1997_arcing,Friedman2001,Friedman2002}, \XGBoost{}, \Catboost{} \cite{Prokhorenkova2018}, \cite{guestrin2016},\lightgbm{} \cite{Ke2017}, \RF{} and \XRF{} \cite{breiman2001,barandiaran1998random}, \SVM and kernel-based \cite{Chihchung2011}, \MLP \cite{Hinton89connectionistlearning}, \Enet{} \cite{Zou05}, \Ridge{} \cite{Hoerl1970}, \LAS{} \cite{tibshirani1996}, \texttt{Logistic regression} \cite{cox1958}, \MARS{} \cite{Friedman1991}, \texttt{CART}, \texttt{XCART} \cite{Breiman1984,gey2005model,Klusowski2020sparse} ). 
 
 For Deep Learning architectures, we combined and compared \trainmet{} with . We left out deep learning methods designed to tackle categorical features as it is not the aim focus of this benchmark and of our proposed method (mainly TabNet\cite{}, Nodes\cite{}, RT transformers\cite{}). We timed on a subset of datasets and random seeds the use of Hyper-parameter optimization, \cite{zimmer-tpami21a, feurer-arxiv20a} which is both outside of the considered usecase and irrelevant to \trainmet{} since this method \textbf{does not introduce new tunable hyper-parameters}. Also note that some technique which require HPO are not
 
 Until recently, there was very little interest for \DL{} on tabular datasets, which fall behind other type of algorithms.
 Very recently, there has been a renewed interest in the subject, with several new methods \cite{kadra2021welltuned,fiedler2021simple,zimmer-tpami21a,gorishniy2021revisiting,kadra2021welltuned} and benchmarks \cite{SHWARTZZIV202284,fiedler2021simple,gorishniy2021revisiting}. See \cite{borisov2021deep} for an extensive review of the state of the art on tabular datasets. Current benchmarks heavily focus on the AutoML (\cite{zoller2021benchmark,yao2018taking,he2021automl}) usecase \cite{zimmer-tpami21a, feurer-arxiv20a}, using costly hyper-parameter tuning over a small collection of very popular big datasets which raised some concerns \cite{koch2021reduced,denton2021genealogy}. We tried to design a benchmark with a larger diversity of sizes and sources while focusing on usecases where models are trained in no more than a few minutes on a personal computer, as is common in most data-science projects \cite{paleyes2020challenges}. 
 COMMENTAIRE IMPORTANCE SMALL DATASETS:
 \cite{Ng2016Nuts,Chahal2021Small}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The goal of this benchmark.}

Phrase objectif de l'etude.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{\trainmet{} Methods.}
We evaluate \trainmet{} variants, namely,...\\
We compare our methods to



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Compared models.}

See Appendix \ref{} for the exhaustive list of compared methods and details about their implementations.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Datasets.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Performance metrics.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Results.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Considered models.}
\textcolor{red}{A REPRENDRE et METTRE DANS LA PARTIE SUIVANTE.}
% \sout{We propose several models with varying depth based on \FFNN{} trained with the \MLR{} loss. We also create ensemble models combining architectures of different depth.
% %We propose several models based on \FFNN{} trained with the \MLR{} loss:\\
% Our models are:\\
% $\bullet$  \MLRL: a simple \FFNN{} of depth $L$ ($1\leq L\leq 4$).\\
% $\bullet$ \BMLRL: a bagging of 10 \FFNN{} of depth $L$ ($L=1$ or $L=2$).\\
% $\bullet$ \BMLR{}: an ensemble of 20 \FFNN{} (the aggregation of \BMLRa{} and \BMLRb{} of depth $1$ and $2$ respectively).\\
% $\bullet$ \BestMLR{}: the best prediction among 20 \NN{} in terms of the validation score.\\
% $\bullet$ \TopfiveMLR{}: the aggregation of the top 5 among 20 \NN{} in terms of the validation score.\\
% For the methods based on bagging \cite{breiman1996}, the final prediction is the mean of each \NN{} prediction.
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



We provide both the code to download raw files and apply each steps, and the resulting data matrices. All results are fully reproducible as both random seeds and random states were manually set and saved at every step of our experiments. 
%See the supplementary material for the github repository.

See the supplementary material for the the github repository, the detailed description of our experimental setting and the exhaustive list of compared methods with their performances. 




To train \eqref{eq:ridgeMLRNN}, we use Adam \cite{kingma2014adam} with default parameters except for the learning rate $\lr$ which depends on the number of layers $L$. Weights $\bth$ are initialized as in \cite{Gloriotetal} and $\bla_{init}$ is chosen to maximize sensitivity of the $\MLR{}$ metric to variation of $\bla$ \sout{(See \eqref{lambdainiti} below for our heuristic rule)}. Our empirical investigations revealed that the obtained $\widehat{\bla}$ after training is close to the optimal oracle choice of $\bla$ on the test set. The complete training protocol is provided in Appendix \ref{sec:appprotocol}. \textcolor{red}{RAJOUTER UNE EXPERIENCE POUR CONFIRMER}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setting.}


\paragraph{Benchmark description.}


To produce this benchmark we aggregated 32 tabular datasets (16 in regression  and 16 in classification), from the UCI repository and Kaggle. %See the appendix for the exhaustive list. 
For computational reasons, we have chosen to restrict the number of datasets but we performed more $train$/$test$ splitting in order to reduce the variance of our results. 
We curated the UCI repository and Kaggle through a set of rules detailed in the appendix ($e.g.$ discard empty or duplicate datasets, times series, missing target, non $i.i.d.$ samples, text format, $etc$.). %See in the Appendix for more details.
%We added $Value$ datasets by repeating the same process on Kaggle\cite{} using the tags with "task": "regression" and "format" : ".csv",".xls". \textcolor{red}{We repeated the same process for classification \sout{and ended up with $Value$ datasets well suited for tabular classification.}}
%See Table \ref{} in the Appendix for the list of violated rules for each available dataset. \textcolor{red}{In summary, we have ? regression datasets and ? classification datasets.}
%\textcolor{red}{B: Mauvais argument, il y a déjà des gens qui sont passés derrière et qui ont corrigés le bench. Plutôt dire que pour des raisons de temps de calcul, on a préféré faire moins de jeux de données, mais remanier en plus propre et surtout avec 10 découpages train test par expérience.}
%Although \cite{Delgado14a} already built a benchmark based on the UCI repository, their methodology presents some flaws \cite{Wainberg2016}. 
%Hence, we went back to the exhaustive list of $Value$ available datasets tagged as regression in the UCI repository and curated it through  .
%Hence, we started anew and curated the UCI repository through a set of rules detailed in the appendix ($e.g.$ discard empty or \textbf{duplicate} datasets, times series, missing target, non $i.i.d.$ samples, text format, $etc$.). After an exhaustive screening of the $Value$ available datasets tagged as regression, we were left with $Value$ datasets. We added $Value$ datasets by repeating the same process on Kaggle\cite{} using the tags with "task": "regression" and "format" : ".csv",".xls". \textcolor{red}{We repeated the same process for classification \sout{and ended up with $Value$ datasets well suited for tabular classification.}}
%See Table \ref{} in the Appendix for the list of violated rules for each available dataset. \textcolor{red}{In summary, we have ? regression datasets and ? classification datasets.}
%Contrarily to classification, there are not that many publicly available well-known datasets which are actually well suited for a tabular regression benchmark. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Preprocessing.} To avoid biasing the benchmark towards specific methods and to get a result as general as possible, we only applied as little preprocessing as we could, without using any feature augmentation scheme. The goal is not to get the best possible performance on a given dataset but to compare the methods on equal ground. We first removed features with constant values such as sample index. Categorical features with more than 12 modalities were discarded as learning embeddings is out of the scope of this benchmark. We also removed samples with missing target. Next, all missing values are imputed with the mean and the mode for numerical and categorical features respectively. We applied one-hot-encoding for categorical values and standardization for numerical features and target. 
%\textcolor{red}{We use a 80/20 ratio for each of the 10 $train$/$test$ splits of the dataset,} with a different seed and no stratification scheme. 
%We repeated $10$ times a $80:20$ train/test split of the data with a different seed and no stratification scheme. 
We repeated our experiments 10 times using a different $80:20$ $train$/$test$ split of the data and no stratification scheme. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Compared methods.}
We ran the benchmark with \textbf{all the methods available in the scikit-learn library} for classification and regression (including \RF{} and \XGB) as well as the \GBDT{} methods. In the rest of the paper, we only display the main classes of methods in Table \ref{tab:methods}.
%\texttt{Fast.ai} \cite{Howard2020}, \Catboost{} \cite{Prokhorenkova2018}, \XGBoost{} \cite{guestrin2016} and \lightgbm{} \cite{Ke2017}. 
%For all our proposed \MLR-architectures, we run its standard equivalent in \DL{} (denoted as \RNN2 for \MLRb{} as an example). 
%In the rest of the paper, we only display the main classes of methods: \MLR{}, \GBDT{} (\XGB, \XGBoost, \Catboost, \lightgbm), \RF{} (\RF{} and \XRF), \SVM{}, \RNN{} (\texttt{Fast.ai} and \MLP), \MARS{}, \GLM{} (Generalized Linear Models: LSE, Elastic Net, Ridge, LASSO, Logistic regression), \TREE{} (CART, XCART) and the \Baseline{} (intercept for regression and class probabilities for classification).
%The exhaustive list of methods and results is provided in the supplementary material.
%each architecture we tested for MLR, we also ran a standard NN with the same architecture and parameters.


% \begin{table}[h]
% \caption{Main classes of methods.}
% \label{tab:methods}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|}
% \hline
% Class      & \\
% of Methods & Methods\\
% \hline
% \MLR{} (this paper)   & \MLRL, \BMLRL, \BMLR, \BestMLR, \TopfiveMLR  \\
% \hline
% \GBDT  & \XGB{} \cite{Breiman1997_arcing,Friedman2001,Friedman2002},  \Catboost{} \cite{Prokhorenkova2018}, \XGBoost{} \cite{guestrin2016}, \lightgbm{} \cite{Ke2017} \\
% \hline
% \RF  & \RF{} and \XRF{} \cite{breiman2001,barandiaran1998random}  \\
% \hline               
% \SVM &  \texttt{Lin-}\SVM{}, \SVM{}, $\nu$\texttt{-}\SVM{} \cite{Chihchung2011}\\
% \hline
% \RNN   & \texttt{Fast.ai} \cite{Howard2020}, \MLP \cite{Hinton89connectionistlearning}\\
% \hline
% \GLM   & \texttt{OLS}, \Enet{} \cite{Zou05}, \Ridge{} \cite{Hoerl1970}, \LAS{} \cite{tibshirani1996}, \texttt{Logistic regression} \cite{cox1958}\\
% \hline
% \MARS & \MARS{} \cite{Friedman1991}\\
% \hline
% \TREE& \texttt{CART}, \texttt{XCART} \cite{Breiman1984,gey2005model,Klusowski2020sparse}\\
% \hline
% \Baseline & Reg: \texttt{Intercept}$\,|\,$ Classif: \texttt{Class probabilities}\\
% \hline
% \end{tabular}
% \end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablation Analysis.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[!hp]
% \caption{Ablation Study in Regression. %\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.}
% }
% \label{tab:ablation}
% 	\centering
% 	\footnotesize
% 	%	\renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|l||c|c|}
% \hline
% Step  &  Mean $\Rdeux$  & Bagging $\Rdeux$ \\
% \hline
% \hline
% \FFNN   & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% \hline
% + Ridge  & $ 0.32  \pm  0.17 $ & $ 0.39  \pm  0.12 $ \\
% \hline
% + Ridge + Struct. Dithering   & $ 0.32  \pm  0.16 $ & $ 0.40  \pm  0.11 $ \\
% \hline
% + Ridge + Permut.  & $ 0.36  \pm  0.11 $ & $ 0.43  \pm  0.07 $ \\
% \hline
% \MLR{}  & $ 0.37  \pm  0.10 $ & $ 0.43  \pm  0.07 $ \\
% \hline
% \end{tabular}
% \end{table}

%\textcolor{red}{$\ast$}
%\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.
\begin{table}[h]
\label{tab:ablation}
	\centering
	\footnotesize
	%	\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l||c|c|}
\hline
Step  &  Mean $\Rdeux$  & Bagging $\Rdeux$ \\
\hline
\hline
\FFNN  & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
\hline
+ Ridge  & $ 0.321  \pm  0.081 $ & $ 0.394  \pm  0.052 $ \\
% \hline
% + Ridge + Struct. Dithering  & $ 0.323  \pm  0.075 $ & $ 0.400  \pm  0.048 $ \\
\hline
+ Ridge + Permut. & $ 0.364  \pm  0.050 $ & $ 0.432  \pm  0.035 $\\
\hline
% \MLR{}   & $ 0.371  \pm  0.024 $ & $ 0.433  \pm  0.000 $ \\
%\hline
\end{tabular}
\caption{Ablation Study for \MLR{} in Regression. %\textcolor{red}{$\ast$ means that the observed $\Rdeux$-score improvement over the previous line is statistically significant according to the Mann-Whitney test on $100$ repetitions of the $train$/$test$ partition.}
}
\end{table}



% NN2  & $ -0.081  \pm  0.173 $ & $ -0.046  \pm  0.169 $ \\
% RidgeNN2  & $ 0.321  \pm  0.081 $ & $ 0.394  \pm  0.052 $ \\
% RidgeSpectral2  & $ 0.323  \pm  0.075 $ & $ 0.400  \pm  0.048 $ \\
% RidgePermut2  & $ 0.364  \pm  0.050 $ & $ 0.432  \pm  0.035 $ \\
% RidgePermutSpectral2  & $ 0.371  \pm  0.024 $ & $ 0.433  \pm  0.000 $ \\


% The following is a summary of our findings, we refer the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance.
% %See the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance. 
% The generic values ($\tilde{\sigma} = 0.03$ and $T=16$) for the \dither{} and the number of permutations hyperparameters yield consistently good results overall. The \dither{} parameter admits an optimal value (see Figure ? in the Appendix) which seems to correspond to the standard deviation of the target noise. As soon as $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. In addition, when $T=16$, GPU parallelization is still preserved.
% %For $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. Moreover, this value is not too large as it preserves GPU parallelization. Consequently, $T=16$ has little to no impact on the runtime of our method. 
% Recall that the Ridge parameter $\bla$ is trained alongside the weights of the \FFNN{} architecture and the initial value $\bla_{init}$ is fixed by the heuristic choice (\ref{lambdainiti}). Our investigations (see Figure \ref{?}) reveals that this choice is close to the optimal oracle choice on the test set. We can also see that the runtime overhead cost of replacing a matrix multiplication with a matrix inversion depends only linearly on the width $J$ and the batch size $\bs$, which are fixed in our method.

% We perform 10 repetitions of our ablation study on 3 datasets which are representative of all the 

% The improvement of each ingredient of the \MLR{} method is statistically significant 


We ran our ablation study (Table \ref{tab:ablation}) in the regression setting on 3 datasets with different sample sizes and feature to sample ratios. We repeated each experiment over 100 random $train$/$test$ splits. All the results presented here correspond to the architecture and hyperparameters of \MLRb{} and \BMLRb{}.
%the 3 components of \MLR{} are Ridge regularization, structure dithering and random permutations.
%Ridge regularization is the essential component of the method as both structured dithering and random permutations are follow-up steps which require the last layer to be a close form. rely on the Ridge close-form. 
% Recall that Ridge regularization is the essential component of the method as it provides a closed form representation of the last hidden layer on which we can conveniently apply the follow-up treatments: structured dithering and/or random permutations. 

%Permutations and structured dithering nous fait battre l'etat de l'art.

A standard \FFNN{} of $2$ layers with a wide architecture ($J=1024$) cannot be trained efficiently on such small datasets as the \FFNN{} instantly memorizes the entire dataset. This cannot be alleviated through bagging at all. Note also its lower overall performance on the complete benchmark (Table \ref{tab:perfR2_rank}). %Note also that bagging cannot help it overcome its overwhelming flaws. 
%Applying Ridge on the last hidden layer allows the \FFNN{} to learn but its generalization performance is still far behind the gold standard \RF. 
Applying Ridge on the last hidden layer allows an extremely overparametrized \FFNN{} to learn but its generalization performance is still far behind the gold standard \RF{}. However, when using bagging with ten such models, we reach very competitive results, underlying the potential of the \MLR{} approach.


\textcolor{red}{
In our experiments, we see that both Ridge regularization and random permutations yield an improvement of the generalization performance. Even better, their effects stack up so that a single \NN{} trained with the \MLR{} method can reach or even outperform the gold-standard methods on most datasets. Furthermore, the improvement yielded by using bagging on top of the \MLR{} method is still of the same order of magnitude ($0.062$) as the one we got when we applied random permutations on top of Ridge regularization to the \FFNN{} ($0.043$). This means the two ingredients of the \MLR{} method (random permutations and Ridge regularization) are not just simple variance reduction techniques like bagging but actually work in a more sophisticated way to build generalizing models. See again Figure \ref{} which reveals highly structured embeddings on the last hidden layer of the trained \NN.}


 



%the \MLR{} method attains a significantly higher $R^2$-score.  better higher performance


%Clearly, using permutations improves the performance much further than Structured Dithering, however, they are both useful. Without bagging, a single \NN{} can reach or even outperform the gold-standard methods on most datasets (see the following section for details). Furthermore, the improvement yielded by using bagging($0.062$ is still of the same magnitude as the one when we started ($0.073$). 
%This means these two ingredients are not just simple variance reduction techniques but actually generate more sophisticated models.

%This means these two ingredients are not simply improving the robustness of the model or reduce its variance, but contribute to learning more complex yet generalizable patterns even with such a large network, over so few samples. 




%Interestingly, the impact of the other hyperparameters in our method is sometimes strikingly different from what is usually observed in the general deep learning framework. With our method, using wider architecture and bigger batch size is always better. See Figures \ref{} and \ref{}. 



\subsection{Overall Performance comparisons.}


% \begin{table}[!hp]
% \caption{\textbf{Performances of the $10$ best methods} for the regression task on our benchmark. \Pa, \Pb, \Pc: the number of datasets a model achieves 90\%, 95\%, 98\% or more of the maximum test $\Rdeux$-score respectively, divided by the total number of datasets. \PMA: average percentage of the maximum test $\Rdeux$-score.}
% \label{tab:perfR2_rank}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
%  Method        & \FR  & Mean $\Rdeux$-score          & \Pa              & \Pb              & \PMA                          \\ \hline
% \hline
% \hline
% \BMLR{}  & $\bm{3.50 \pm 2.38}$ & \textbf{$0.67 \pm 0.25$} & \textbf{$0.89 \pm 0.32$} & \textbf{$0.72 \pm 0.46$} & \textbf{$0.92 \pm 0.17 $}\\
% \BMLRb{}  & $ 3.94 \pm 2.84$ & $0.67 \pm 0.26$ & $0.83 \pm 0.38$ & $0.61 \pm 0.50$ & $0.88 \pm 0.28 $\\
% \BMLRa{}  & $ 5.50 \pm 4.51$ & $0.66 \pm 0.24$ & $0.83 \pm 0.38$ & $0.67 \pm 0.49$ & $0.92 \pm 0.13 $\\
% \MLRc  & $ 7.33 \pm 3.80$ & $0.65 \pm 0.27$ & $0.67 \pm 0.49$ & $0.44 \pm 0.51$ & $0.83 \pm 0.37 $\\
% \MLRb  & $ 7.94 \pm 3.83$ & $0.65 \pm 0.26$ & $0.72 \pm 0.46$ & $0.44 \pm 0.51$ & $0.86 \pm 0.26 $\\
% \MLRa   & $ 9.06 \pm 4.49$ & $0.64 \pm 0.25$ & $0.78 \pm 0.43$ & $0.44 \pm 0.51$ & $0.81 \pm 0.47 $\\
% \hline
% \RF   & $ 7.11 \pm 6.57$ & $0.64 \pm 0.28$ & $0.67 \pm 0.49$ & $0.50 \pm 0.51$ & $0.68 \pm 1.01 $\\
% \XRF  & $ 7.56 \pm 5.82$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.50 \pm 0.51$ & $0.68 \pm 0.93 $\\
% \hline
% \XGB  & $ 7.22 \pm 6.68$ & $0.63 \pm 0.29$ & $0.72 \pm 0.46$ & $0.67 \pm 0.49$ & $0.76 \pm 0.59 $\\
% \hline
% \RNN2  & $ 11.72 \pm 5.29$ & $0.60 \pm 0.32$ & $0.56 \pm 0.51$ & $0.39 \pm 0.50$ & $0.62 \pm 0.91 $\\
% \hline
% \end{tabular}
% }
% %\label{tab:stat_test}
% \end{table}




\begin{table}[H]
\label{tab:perfR2_rank}
	\centering
	\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Class      &   &           &               &    &           &                          \\
 of Methods        & \FR  & Mean $\Rdeux$-score          & \Pa              & \Pb    & \Pc          & \PMA                          \\
  \hline
\hline
\hline
\MLR & $2.525 \pm 1.355$ & $0.744 \pm 0.022$ & $0.963$ & $0.856$ & $0.719$ & $0.946 \pm 0.089$\\
\GBDT & $2.719 \pm 1.850$ & $0.726 \pm 0.093$ & $0.863$ & $0.756$ & $0.650$ & $0.898 \pm 0.237$\\
\RF & $3.538 \pm 1.896$ & $0.724 \pm 0.070$ & $0.825$ & $0.681$ & $0.481$ & $0.914 \pm 0.159$\\
\SVM & $4.281 \pm 1.534$ & $0.711 \pm 0.068$ & $0.831$ & $0.594$ & $0.362$ & $0.882 \pm 0.172$\\
\RNN & $4.331 \pm 2.206$ & Aberating value & $0.725$ & $0.606$ & $0.475$ & Aberating value \\
\MARS & $5.644 \pm 1.623$ & $0.677 \pm 0.066$ & $0.537$ & $0.350$ & $0.163$ & $0.861 \pm 0.167$\\
\LM & $5.938 \pm 1.804$ & $0.658 \pm 0.094$ & $0.531$ & $0.294$ & $0.156$ & $0.837 \pm 0.179$\\
\TREE & $7.125 \pm 1.613$ & $0.512 \pm 0.237$ & $0.338$ & $0.188$ & $0.119$ & $0.578 \pm 0.570$\\
\Baseline & $8.900 \pm 0.375$ & $-0.023 \pm 0.211$ & $0.000$ & $0.000$ & $0.000$ & $-0.031 \pm 0.075$\\
\hline
\end{tabular}
}
\caption{\textbf{Performances of the best method in each class of methods} for the regression task on our benchmark. \Pa, \Pb, \Pc: the number of datasets a model achieves 90\%, 95\%, 98\% or more of the maximum test $\Rdeux$-score respectively, divided by the total number of datasets. \PMA: average percentage of the maximum test $\Rdeux$-score.}
%\label{tab:stat_test}
\end{table}



\textbf{The \MLR{} method clearly outperforms all the compared methods for the regression task.} \BMLR{} with a \Pc{} of $0.719$ on the whole benchmark and Friedman Rank of $2.525$ is above \GBDT{}, with a \Pc{} of $0.65$ and Friedman Rank $2.719$ in Table \ref{tab:perfR2_rank}. 
As revealed by its \PMA{} statistics at $0.946$%in Table \ref{tab:perfR2_rank})
, \BMLR{} is far ahead of the other methods. 
%Thus it actually almost never "loses" to the best method by a lot. 
This means that \MLR{} produces reliable results at a rate that is even above methods like \RF{} which are often deemed the safest pick. 
%The same conclusion is also valid for \BMLRa{} and \BMLRb{}.
Standard \RNN{} with equivalent architecture and \MSE{} loss performs poorly with a Friedman rank of $4.331$. Noticeably, \BMLR{} was most often the best method among all the \MLR{} methods.% See the appendix for more details.




\begin{table}[h]
\caption{\textbf{Performances of the best method in each class of methods} for the classification task with the accuracy score.}
\label{tab:ACCperf}
	\centering
	\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Class      &   &           &               &    &           &                          \\
 of Methods        & \FR  & Mean \Acc        & \Pa              & \Pb    & \Pc          & \PMA                          \\ \hline
\hline
\hline
\GBDT & $1.769 \pm 0.998$ & $0.889 \pm 0.038$ & $0.963$ & $0.881$ & $0.819$ & $0.971 \pm 0.054$\\
\MLR & $2.913 \pm 1.403$ & $0.882 \pm 0.031$ & $0.963$ & $0.869$ & $0.800$ & $0.956 \pm 0.070$\\
\RF & $3.056 \pm 1.415$ & $0.882 \pm 0.038$ & $0.912$ & $0.819$ & $0.656$ & $0.958 \pm 0.063$\\
\GLM & $3.756 \pm 1.561$ & $0.862 \pm 0.060$ & $0.806$ & $0.631$ & $0.463$ & $0.940 \pm 0.062$\\
\TREE & $4.763 \pm 1.195$ & $0.836 \pm 0.062$ & $0.731$ & $0.381$ & $0.237$ & $0.908 \pm 0.084$\\
\QDA & $5.675 \pm 1.688$ & $0.723 \pm 0.160$ & $0.338$ & $0.194$ & $0.169$ & $0.796 \pm 0.159$\\
\Baseline & $6.856 \pm 1.574$ & $0.593 \pm 0.168$ & $0.069$ & $0.025$ & $0.025$ & $0.661 \pm 0.133$\\
\RNN & $7.213 \pm 0.980$ & $0.565 \pm 0.152$ & $0.025$ & $0.013$ & $0.013$ & $0.625 \pm 0.136$\\
\hline
\end{tabular}
}
%\label{tab:stat_test}
\end{table}




% For binary classification task with the usual accuracy score, \MLR{} is a close second behind \GBDT{} both in terms of Accuracy and AUC scores. 
% %better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% %Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

\begin{table}
\caption{\textbf{Performances of the best in each class of methods} for the classification task with \AUC{} score.}
\label{tab:AUCperf}
	\centering
	\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Class      &   &           &               &    &           &                          \\
of Methods        & \FR  & Mean \AUC        & \Pa              & \Pb    & \Pc          & \PMA                          \\ \hline
\hline
\hline
\GBDT & $1.738 \pm 1.190$ & $0.918 \pm 0.048$ & $0.938$ & $0.912$ & $0.875$ & $0.963 \pm 0.108$\\
\MLR & $2.900 \pm 1.304$ & $0.908 \pm 0.012$ & $0.912$ & $0.844$ & $0.694$ & $0.952 \pm 0.106$\\
\RF & $2.938 \pm 1.390$ & $0.912 \pm 0.047$ & $0.931$ & $0.887$ & $0.706$ & $0.956 \pm 0.095$\\
\LM & $3.881 \pm 1.572$ & $0.889 \pm 0.060$ & $0.775$ & $0.662$ & $0.475$ & $0.935 \pm 0.094$\\
\RNN & $4.856 \pm 1.545$ & $0.843 \pm 0.154$ & $0.706$ & $0.506$ & $0.412$ & $0.896 \pm 0.155$\\
\TREE & $5.975 \pm 1.160$ & $0.813 \pm 0.091$ & $0.394$ & $0.212$ & $0.212$ & $0.852 \pm 0.119$\\
\QDA & $6.031 \pm 1.371$ & $0.772 \pm 0.149$ & $0.394$ & $0.256$ & $0.150$ & $0.818 \pm 0.152$\\
\Baseline & $7.681 \pm 1.084$ & $0.499 \pm 0.151$ & $0.006$ & $0.000$ & $0.000$ & $0.537 \pm 0.072$\\
\hline
\end{tabular}
}
%\label{tab:stat_test}
\end{table}

For binary classification task with the usual accuracy score, \MLR{} is a close second behind \GBDT{} both in terms of Accuracy and \AUC{} scores. 
%better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
%Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% \textbf{The \MLR{} method clearly outperforms all the compared methods in the regression task.} \BMLR{} with a \Pb{} of $0.72$ on the whole benchmark and Friedman Rank of $3.5$ is far above \RF{}, with a \Pb{} of $0.5$ and Friedman Rank $7.111$ in Table \ref{tab:perfR2_rank}. 
% As revealed by its \PMA{} statistics at $0.92$%in Table \ref{tab:perfR2_rank})
% , \BMLR{} is far ahead of the other methods. 
% %Thus it actually almost never "loses" to the best method by a lot. 
% This means that \BMLR{} produces reliable results at a rate that is even above methods like \RF{} which are often deemed the safest pick. The same conclusion is also valid for \BMLRa{} and \BMLRb{}.
% Standard NN (\texttt{NN2}) with equivalent architecture and MSE loss perform poorly with a Friedman rank of $11.722$.





% For binary classification task with the usual accuracy score, \XRF{} is better than \MLR{} in terms of \Pc{}. However, the Friedman rank of \BMLR{} is higher than that of \XRF{} (ranks $4.0$ and $4.31$ respectively). The \BMLR{} method performance in terms of \AUC{} compares favorably with \RF{} for \Pc{} ($0.77$ against  $0.69$). The Friedman rank of \MLR{} and \RF{} are equivalent but the standard deviation of the Friedman rank  of \MLR{} is smaller than that of \RF. 
% Finally, the \PMA{} of \MLR{} is also above $0.98$ for both \AUC{} and accuracy scores.

% of the is similar  standard deviation of the Friedman rank of the \MLR{} performances are equivalent for the mean \AUC{}, the Friedman Rank (\FR) and the \PMA. 


% Regarding the accuracy, although \XRF{} is better in terms of mean accuracy, \Pb{}, \Pc{}, the \MLR{} performance is better than \XRF{} in terms of Friedman Rank ($4.0$ for \MLR{}, $4.31$ for \XRF), and worst for the other metrics.


% AUC: the \MLR{} method produces better discriminating models. Interesting in unbalanced settings.








% Pas utile vu qu'il y a le Friedman Rank: \textcolor{red}{\textbf{Another important take-away fact is that \MLR{} ranks in the top three on $18$ out of the $21$ datasets, on top of being the best in average.}}


% As we observe in Tables \ref{tab:perfR2_rank} and \ref{tab:ACCperf}, the depth $L$ in the \MLRL{} method seems to be the only data-dependent hyperparameter. However a simple aggregation of \NN{} of different depths performs as well as %is able to reliably mimic the best performance of 
% the \NN{} with the most adequate depth for the dataset at hand. 



%Indeed with a Friedman rank of $\textcolor{purple}{Value}$ on the benchmark, \BMLR{} outperforms all \MLRL{} architectures with a Friedman rank of $\textcolor{purple}{Value}$ at best.

%\medskip


% \subsection{Computing time/scalability??????}
% \textcolor{red}{Computing time raisonable???????}

% \textcolor{red}{scalability huge datasets ???????}

% c'est pas le but du papier vu qu'on se concentre sur les petits datasets mais \MLR{} se calcule aussi sur les gros datasets. Cependant le standard NN 



==> oldprotocole.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The \MLR{}-\FFNN{}}
\label{sec:MLRmethod}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The (\MLR{}) method for Regression}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\mathcal{D}_{train}=(\bx,\bY)=\{(\bx_i,Y_i)\}_{i=1}^n$ be the $train$-set with $\bx_i\in\R^d$ where $d$ denotes the number of features and $Y_i \in \R$.
We consider a simple \FFNN{} with $L$ layers, $J$ nodes on each hidden layer.



and the \ReLu{} activation function between each hidden layer. For $n$ observations $\bx$, we set $\bA^0=\bx\in\R^{n\times d}$ and
$\bA^1=\ReLu(\bA^{0}W^{1} +B^{1}),\,\,W^1\in\R^{d\times J}$
\begin{eqnarray}
\label{FFNN}
\bA^{\el+1}&=&\ReLu(\bA^{\el}W^{\el+1} +B^{\el+1}),\quad W^{\el+1}\in\R^{J\times J},\,\,\forall\el\in\llbracket1,L-2 \rrbracket,\nonumber\\
\bA^L&=&\bA^{L-1}W^L,\quad W^L\in\R^{J\times 1},
\end{eqnarray}
where $\forall\el\in\llbracket1,L-1 \rrbracket$, $B^{\el} = \mathbbm{1}_n \otimes b^{\el}$, $b^{\el}\in\R^{J}$ are the bias terms.

The 3 essential ingredients of the \MLR{} method are Ridge regularization, structured dithering and random permutations as they promote generalization when we train this \FFNN{}. 

We introduce first the Ridge regularization. For $\bla>0$, we set
\begin{eqnarray}
\label{W}
\bW&=&\bW(\bla,\bth,\bx)=\left[(\bA^{L-1})^\top\bA^{L-1}+\bla \I_J\right]^{-1}(\bA^{L-1})^\top\in\R^{J\times n}\\
\label{H}
\bH&=&\bH(\bla,\bth,\bx)=\bA^{L-1}\bW\in\R^{n\times n}
\end{eqnarray}
where the last hidden layer is $\bA^{L-1}:=\bA^{L-1}(\bth,\bx)$ and $\I_J$ denotes the identity matrix% 
. Note that $\bH$ is differentiable w.r.t. $\bth =\{(W^{\el},b^{\el})\}_{\el=0}^L$ and $\bla$. We apply Ridge regularization\footnote{Ridge model :  $f(\bla,\bth,\bx)=\bx\,\beta_{\bla}(\bx,\bY):=\bx\,(\bx^\top\bx+\bla\I)^{-1}\bx^\top\bY$}
to the last hidden layer $\bA^{L-1}$ instead of input $\bx$: 
\begin{eqnarray}
\label{ridge}
f(\bla,\bth,\bx):=\bA^{L-1}W^L=\bA^{L-1}\bW(\bla,\bth,\bx)\bY=\bH(\bla,\bth,\bx)\bY.
\end{eqnarray}

Next we introduce the \textbf{permutations}. For a permutation $\perm$ of $n$ elements, we define the corresponding label permutation operator $\perm$ of $\bY = (Y_1,\cdots,Y_n)$ as
$
\perm(\bY)=(Y_{\perm(1)},\cdots,Y_{\perm(n)}).
$
Fix $T\geq 1$ and draw $T$ label permutation operators \textbf{uniformly at random} in the set of all possible label permutations : $(\perm^t(\bY))_{t=1}^T$. This operation can be seen as a form of data-augmentation on the labels.



\begin{mydef}[\MLR{} regression loss]
\label{MLRlossBigsetting}
Set $\bH=\bH(\bla,\bth,\bx)$. We draw $i.i.d.$ random vectors $\xi$ and $\left(\xi_t\right)_{t=1}^T$ distributed as $\cN(0_n,\I_n)$. Let $\left(\perm^t(\bY)\right)^T_{t=1}$ be $T$ independently drawn permutations of $\bY$. We set $\overline{\bY} = mean(\bY)$ and define the \MLR{} loss as

\begin{align*}
\MLR(\bla,\bth) &= \RMSE\,\left(\bY+\tbH \xi\,;\,\bH\bY\right)\\
&\hspace{1cm}+\frac{1}{T}\sum_{t=1}^T\left|\RMSE\,( \bY\,;\, \overline{\bY}\mathbbm{1}_n) -  \RMSE\,\left(\perm^t(\bY)+\tbH \,\xi_t\,;\,\bH\,\perm^t(\bY)\right)\right|.
\end{align*}
\end{mydef}





The \MLR{} loss contains two antagonistic terms and was first introduced in the linear regression setting \cite{MLR}. The first term is the usual \RMSE{} while the second term quantifies the amount of memorization of a model by comparing its \RMSE{} on uninformative labels to the baseline $\RMSE\,( \bY\,;\, \overline{\bY}\mathbbm{1}_n)$, $i.e.$ the performance achieved without fitting the data. Using the \RMSE{} instead of the \MSE{} in the comparison slightly improves the generalization performances. We explain below the role of $\tbH \xi$ and $\tbH \xi_t$.




\paragraph{The benefit of close-form regularization.} 

The replacement of the output layer with Ridge regularizes the network in two ways:
$(i)$ the weights on the output layer are a direct function of the last hidden layer $\bA^{L-1}$. This effect is much stronger than adding a constraint or a penalty directly on $W^L$ the weights of the $L$-th layer in (\ref{FFNN}); $(ii)$ the close-form we choose is the Ridge instead of the \OLS, which implicitly subjects the weights to a steerable $L_2$ regularization.











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The generalization effect of random permutations.}
Our work is loosely related to \cite{zhang2016understanding} where label permutations are used after the model has been trained as a \textit{qualitative} observational method to exhibit the overfitting $capacity$ of Neural networks. In our approach, we go further as we use random permutations during the training phase to define a \textit{quantitative} measure of the amount of overfitting of a model. More precisely, label permutation is used to produce a control set $(\bx,\perm(\bY))$ that can only be fitted through memorization. \MLR{} focuses on patterns that appear only in $(\bx,\bY)$ and not in uncorrelated pairs $(\bx,\perm(\bY))$. %See the appendix for more details.



\paragraph{Structured Dithering.} 



We describe an additional scheme to prevent memorization. We apply a dithering scheme which adapts to the spectral structure of $\bH$, the "regularized projector" based on $\bA^{L-1}$ (the output of the last hidden layer). More specifically, we muddle the target using $\tbH \xi\,$ which introduces noise of higher variance along the weakly informative eigendirections of $\bH$.










\paragraph{Computational point of view.} The permutations are drawn once before the training and are not updated or changed thereafter. Once the \FFNN{} is trained, these permutations have no further use and are thus discarded. In practice we take $T=16$ for all the datasets in our benchmark. Therefore, $T$ \textbf{does not require hyperparameter tuning}. Moreover, note that the choice of the seed used to generate the permutations has no impact on the values of the \MLR{} loss. The additional computational cost of using \MLR{} is marginal. We only need to compute a matrix inverse on the output of the last hidden layer $\bA^{L-1}$. This operation is differentiable and inexpensive as parallelization schemes provide linear complexity on GPU when some memory constraints are met \cite{Murugesan2018Embarrassingly,rajibr2010accelerating,chrzeszczyk2013matrix,SHARMA201331}. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model: \NN{} and training protocol}
\label{sec:Protocol}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The \NN{} Architecture.} 
We consider the \FFNN{} described in \eqref{FFNN} with $L$ layers and all the hidden layers of constant width $J$. In our experiments, we always take $J$ as large as possible (our machine with 11GVRAM allowed for $J=2^{10}$) and $L\in\cG_L:=\{1,2,3,4\}$. 
%All these choices are motivated in the ablation study in Section \ref{sec:exp} below. 

The \MLR{} neural net (\NN) is 
\begin{align*}
    \label{NN}
 \NN(\hbth,\hatla,\bigcdot)=\bA^{L-1}(\hbth,\bigcdot) \,\bW(\hbth,\hatla,\bx) \bY \quad\text{with}\quad (\hbth,\hatla) = \underset{\bth,  \bla}{\arg\min} \;\MLR(\bla,\bth)
\end{align*}
with $\bW(\cdot,\cdot,\bx)$ as defined in \eqref{W}. The initialization of $\bth$ is as in \cite{Gloriotetal}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Initialization of the Ridge parameter.} 

The initialization of $\bla$ is both crucial and non trivial. Choosing $\bla$ close to $0$ will hinder regularization. Furthermore, a very small value of $\bla$ will cause numerical instability during the matrix inversion. Conversely, choosing $\bla$ too big will prevent any learning. Indeed, the gradient with respect to $\bla$ will vanish in both cases. From our initial calibration, we discovered that there exists no universal value to initialize $\bla$. The appropriate initial value depends on many factors such as data size, network architecture, difficulty of the task, $etc$. However, we found a very efficient heuristic to pick an appropriate initial value. We want to start training from the point where fitting the data will lead to generalization as much as possible instead of memorization. In this region, the variation of \MLR{} with respect to $\bla$ is maximum. In practice, we pick $\bla_{init}$ by running a grid-search on the finite difference approximation for the derivative of \MLR{} in (\ref{lambdainiti}) on the grid 
$\cG_{\bla}=\left\lbrace \bla^{(k)} = 10^{-1}\times10^{5 \times k / 11}\;: \;   k = 0, \cdots, 11 \right\rbrace$:
%
\begin{eqnarray}
\label{lambdainiti}
\bla_{init}=\sqrt{\bla^{(\hat {k}})\,\bla^{(\hat {k}+1)}}\;\text{where}\;\hat {k}=\arg\max\left\{ \left(\MLR(\bla,\bth^{(k+1)}) - \MLR(\bla,\bth^{{(k)}})\right),\, \bla^{(k)}\in\cG_{\bla}\right\}.
\end{eqnarray}
From a computational point of view, the overcost of this step is marginal because we only compute $\bA^{L-1}$ once, and we do not compute the derivation graph of the $11$ matrix inversions or of the unique forward pass. The Ridge parameter $\bla$ is \textbf{not an hyperparameter} of our method; it is trained alongside the weights of the Neural Net architecture. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{\Dither{} \cite{dither}.} 
We do not apply the \MLR{} loss on $\bY$ and the permuted labels $\left(\perm^t(\bY)\right)_{t=1}^T$ but rather on noisy versions of them. We draw $T+1$ $i.i.d.$ $\cN(\bO_n,\widetilde\sigma^2\I_n)$ noise vectors that are added to $\bY$ and $\perm^t(\bY)$, $1\leq t \leq T$. Here again, $\widetilde\sigma$ is \textbf{not an hyperparameter} as we use the same value $\widetilde\sigma=0.03$ for all the data sets in our benchmark.


  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Training protocol.} 


Using wider architecture ($J=2^{10}$) and bigger batch size ($\bs = \min(J,n)$) is always better. To train our \FFNN{}, we use Adam \cite{kingma2014adam} with default parameters except for the learning rate $\lr$ (which depends on the number of layers $L$. See Table~\ref{tab:architectures1}) and we select a $validation$-set of size $n_{val}=20\%\, n$.

{\it Choice of $\max_{\iter}$ and early stopping.} We fix the budget (\fixB = 5 min) and denote by 
$n_{\iter}$ the possible number of iterations during the alloted time \fixB. We fix the maximum number of iterations $\max_{\iter}$ (depending on the value of $L$).
Then, $\iter = \min(\max_{\iter},n_{\iter})$ is the number of iterations that will actually be performed.
%, i.e. the minimum between between $\max_{\iter}$ and $n_{iter}$ which is the number of iterations during the allotted time \fixB. 
We read the $\Rdeux$-score for each iteration on the $validation$-set and take the iteration with the best $\Rdeux$-score: 
%\textcolor{red}{$\iter^*:=\arg\max\{\texttt{R}^2_k, \ k =1,\cdots,\max_{iter}\}$} \sout{
$\iter^*:=\arg\max\{\texttt{R}^2_k, \ k =1,\cdots,\iter\}$
%}
. Finally, $(\hbth,\hatla)$ will take its value at iteration $\iter^*$.




\begin{table}[!hp]
	\caption{Benchmarked architectures. }
	\label{tab:architectures1}
\footnotesize
 	\centering
 \begin{tabular}{|c||c|c |c|c|c |c|c|c|c|}
 \hline
Architecture & $L$ & $\lr$ & $\max_{\iter}$ & \fixB & $J$ & $\bs$ & $T$ & \multicolumn{2}{|c|} {$\widetilde\sigma$ }   \\ 
\hline
 $\MLRa $& $1$ & $10^{-2}$ & $200$ & $10'$ & $2^{10}$ & $min(n, J)$ & $16$ & Reg.: $0.03$ & Classif.: $0$ \\
  \cline{9-10} 
 $\MLRb $& $2$ & $10^{-3}$ & $200$ & $id.$ & $id.$ & $id.$& $id.$ &\multicolumn{2}{|c|} {$id.$}\\
 $\MLRc $& $3$ & $10^{-3.5}$ & $400$ &  $id.$ & $id.$ & $id.$& $id.$ & \multicolumn{2}{|c|} {$id.$}\\
 $\MLRd $& $4$ & $10^{-4}$ & $400$ &  $id.$ & $id.$ & $id.$& $id.$ & \multicolumn{2}{|c|} {$id.$} \\
 \hline
 \end{tabular}
%	}

 \end{table}

%The following is a summary of our findings, we refer the Appendix for the complete description of the impact of each component of our method on the generalization performance.
%See the Appendix for the complete ablation study on the impact of each component of our method on the generalization performance. 
The generic values ($\tilde{\sigma} = 0.03$ and $T=16$) for the \dither{} and the number of permutations hyperparameters yield consistently good results overall. The \dither{} parameter admits an optimal value which seems to correspond to the standard deviation of the target noise. As soon as $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. In addition, when $T=16$, GPU parallelization is still preserved.
%For $T=16$, the choice of permutations has little impact on the value and the \MLR{} loss. Moreover, this value is not too large as it preserves GPU parallelization. Consequently, $T=16$ has little to no impact on the runtime of our method. 
Recall that the Ridge parameter $\bla$ is trained alongside the weights of the \FFNN{} architecture and the initial value $\bla_{init}$ is fixed by the heuristic choice (\ref{lambdainiti}). Our investigations reveals that this choice is close to the optimal oracle choice on the test set. We can also see that the runtime overhead cost of replacing a matrix multiplication with a matrix inversion depends only linearly on the width $J$ and the batch size $\bs$, which are fixed in our method. As a pure DL method, \MLR{} method is scalable. Its complexity is the same as training a standard \RNN{} \cite{Murugesan2018Embarrassingly}. We refer to the Appendix for a detailed description of the training protocol.


==> oldsota.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Extended state of the art} 
\label{sec:SOTA}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Over the last decade, we have witnessed the spectacular performance of Deep Learning (\DL) in the fields of computer vision \cite{Krizhevsky2012_cnn}, audio \cite{Hinton2012} and natural language processing \cite{bert2019}. Until recently, it was also widely believed that \DL{} is irrelevant for tabular data \cite{videolecture}. While the need to handle tabular data arises in many fields ($e.g.$ material science \cite{FENG2019300}, medecine \cite{Rajkomar2018}, online advertising \cite{Zhou2018click,Guo2016}, finance \cite{buehler_deep_2019}), \DL{} for tabular data remains understudied and underused. It may seem strange considering that tabular data appears at first more straightforward to handle than image or textual data.


Most experiments seem to indicate that tree based ensemble methods \cite{Denil2014narrow,Delgado14a,Mentch2020Rand,Wainberg2016}
are the most reliable option on tabular data and often work well even without any parameter tuning \cite{Delgado14a,Wainberg2016}. By contrast, training \DL{} models usually requires extensive trial and error, expertise and time to properly tune the hyperparameters \cite{smith2018disciplined}. This comparison is even worse in the small data regime ($n < 10^3$ or even $n<300$). In many fields including material sciences \cite{FENG2019300}, medicine \cite{JTD4418,Rajkomar2018}, environmental studies \cite{Cassotti2015similarity-based}, small datasets are not rare occurrences since collecting samples and assembling large datasets may be costly, or even impossible by the nature of the task at hand\footnote{$e.g.$ decision making on a limited amount of cases during a pandemic.}.%\textcolor{red}{Papier new yorker}.



Deep learning mostly relies on transfer learning schemes to tackle small datasets \cite{Oquab_2014_CVPR}, which are almost never an option for tabular datasets \cite{shavitt2018}. This is due to the lack of transferable domain knowledge between tabular features. Another important line of work focuses on the preprocessing of categorical features which was an historical limitation of \DL{} \cite{qu_product-based_2016, guo_deepfm:_2017, wang_collaborative_2015,cheng_wide_2016,covington_deep_2016,zhang_deep_2019}. In that regard, entity embeddings \cite{Guo2016}, which try to capture relationships between categories, have become standard in \DL{} libraries (tensorflow, PyTorch, \textit{etc.}). Meanwhile, tree based ensemble methods and Gradient Boosting Decision Trees (\GBDT{}) are still considered the best option to handle categorical data \cite{Prokhorenkova2018,Anghel2018Bench,Harasymiv2015_gbdt}.

Developing a \DL{} solution for tabular data is desirable at it can leverage the particular strengths of \DL{}, in particular its ability to perform automatic feature engineering and end-to-end training via gradient descent. The recent \texttt{PyTorch Tabular} project \cite{pytorchtab} and the growing number of articles on tabular data in recent years show the increasing interest of the \DL{} community in this topic \cite{YangMorillo2018,arik2020tabnet,ZhouFeng2017,MillerHHJK17,FengYuZhou2018,ke2019tabnn,Olson2018moderna,Arora2020meuf,katzir2021netdnf,Klambauer2017,shavitt2018,Haldar2019,Popov2020Neural,pmlr-v97-du19a}.
%Beat \GBDT significantly

\begin{table}[!hp]
\caption{State-of-the-art: Deep Learning for supervised tasks on tabular data. $\bm{*}$ uses the UCI database which has some well-known flaws \cite{Arora2020meuf,Klambauer2017,Wainberg2016}.}
\label{tab:SotA}
%\footnotesize
\centering
	\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|cc|c|}
\hline
Method        &  End-to-end & Works without & Task & \multicolumn{2}{|c|}{ Benchmark }    & Consistently outperforms  \\
       &   differentiable & HP tuning &  & \# datasets& Range $n$   & \GBDT \\
       \hline
\TabNN{} \cite{ke2019tabnn}             & \no & \no & \BOTH &5&14.8K-7.3M & no\\%14.8K-7.29M 
\hline
\NODE{} \cite{Popov2020Neural}             & \checkmark & \no & \BOTH &6&500K-11M & no\\%Sometimes\\ 
\hline
\TabNet{} \cite{arik2020tabnet}              & self-supervised  & \no  & \BOTH & 4&10K-11M & \checkmark\\%Significantly \\
\hline
\DNDT{} \cite{YangMorillo2018}             & \checkmark & \checkmark &\Clf &14& 150-1.1M & no\\
\hline
\NTK{} \cite{Arora2020meuf}            & \checkmark & \no & \Clf &90\bm{*}& 10-130K & no  \\ 
\hline
\SNN {}\cite{Klambauer2017}          & \checkmark & \no & \BOTH &122\bm{*}&  10-130K & no\\
\hline
\NetDNF{} \cite{katzir2021netdnf}         &  no & \checkmark & \Clf & 6&9.8K-200K &no\\% rarely \\ 
\hline

\RLN{} \cite{shavitt2018}             & \checkmark & \checkmark& Reg & 9&2.5K& no \\ \hline

\MLR{} (this work)          & \checkmark & \checkmark & \BOTH & 32 & 72-65K & Reg:\checkmark\\%Significantly\\ 
\hline
\end{tabular}
}
\end{table}



\paragraph{Regularization.} Two classical \DL{} regularization strategies, dropout \cite{srivastava14a} and weight decay \cite{Hanson1988Comparing}, have been compared by \cite{ZhangDW16} on tabular data. They found dropout to be better, however dropout may still fail in some tabular data tasks \cite{Haldar2019}. Moreover \cite{SongS0DX0T19,ZhangDW16,Qu2018,guo_deepfm:_2017} seem to indicate that dropout parameters are data and model dependent. 




\paragraph{Interpretability.} 
The "black-box" aspect of \DL{} remains a major obstacle to its wider use as interpretability in AI is an important concern \cite{chen2018learning}. Recently, a line of research focuses on the development of novel network architectures with interpretable features. \DNDT{} \cite{YangMorillo2018} is a specific neural network architecture which can be trained via end-to-end gradient descent. In addition, it can also be rendered as a decision tree for the sake of interpretation. However \DNDT{} is not scalable $w.r.t.$ the number of features and does not outperform Random Forests (\RF) or standard \RNN{} on the UCI database. Attention-Mechanism (\AM) has boosted \DL{} performance on a range of \NLP{} tasks \cite{Bahdanau2014-Attention,bert2019}). It turns out that \AM{} can also be used for interpretability purpose. Recently \cite{arik2020tabnet} exploited \AM{} to develop \TabNet{}, an interpretable \DL{} method for tabular data, and claimed it outperforms the gold standard on a limited number of data sets of size $\gtrsim 10K$. A limitation of this approach is the complicated data dependent fine-tuning of the hyperparameters.



\paragraph{Hybrid architecture.}  Several recent works propose to combine decision trees with \DL{}. In that regard, \cite{ZhouFeng2017,MillerHHJK17,FengYuZhou2018} proposed to stack layers of \RF{} or \GBDT{}. However these architectures cannot be trained end-to-end, which may result in potentially inferior performance. \TabNN{} \cite{ke2019tabnn} is a hybrid machine learning algorithm using \GBDT{} and Deep Neural Networks (\DNN). \TabNN{} outperforms standard Feed-Forward Neural Networks (\FFNN{}) but the improvement over \GBDT{} seems marginal in their experiments on 6 data sets ranging in size from $15$K up to $7.9$M training samples. More recently, \NODE{} \cite{Popov2020Neural}, a new \DNN{} architecture consisting of differentiable oblivious decision trees, can be trained end-to-end via backpropagation. \NODE{} marginally outperforms ensemble methods (\Catboost \cite{Prokhorenkova2018}, \XGBoost \cite{guestrin2016}) on 4 out of 6 large size tabular data sets
and requires careful hyperparameter optimization.

\paragraph{New loss functions.} Our contribution falls in this line of research. It consists in replacing the usual loss used to train \DNN{} by specific losses with interesting properties. In that regard, Regularization Learning Networks (\RLN) \cite{shavitt2018} is a new family of neural networks trained with a new loss, named counterfactual loss, together with stochastic gradient descent. \RLN{} performs significantly better than standard \RNN{} but could not beat \GBDT{}.

\paragraph{Other approaches.} We can also cite Neural Tangent Kernel (\NTK){}\cite{Arora2020meuf}, \NetDNF{} \cite{katzir2021netdnf} and Self-Normalized Neural Networks (\SNN) \cite{Klambauer2017}. Table \ref{tab:SotA} summarizes their properties. We provide more details about these methods in the Appendix.



















{\color{red}
\paragraph{Contributions.} 

We propose a pure deep learning solution to train a standard \FFNN{} for tabular data. Our method, \textbf{Muddling labels for Regularization} (\MLR), penalizes memorization over permuted labels and structured noise through the application of a differentiable close-form regularization scheme on the last hidden layer during training. More specifically:


- Our method outperforms usual methods (Ensemble, \SVM, Boosting, Linear Regression, $etc.$ ) including the gold standards \RF{} and \GBDT{} for the usual statistics (Mean $\Rdeux$, Friedman rank, P90, P95, P98, PMA) on a diverse collection of regression datasets. Our method also comes in a close second for classification tasks.
%Our method outperforms the gold standard in terms of Friedman rank for regression and classification whatever the number of samples, of features, the type of features or the domain of the datasets.. 

%Our method proved more reliable than usual methods (Ensemble, \SVM, Boosting, Linear Regression, $etc.$ ) including the gold standards \RF{} and \GBDT{}, on our aggregated benchmark (UCI+ Kaggle).
% \textcolor{red}{It consistently ranked in the top \textcolor{red}{3 or 5} on all datasets in terms of $\Rdeux${} for regression or Accuracy and \AUC{} for binary classification,} whatever the number of samples, of features, the type of features or the domain of the datasets. 



- The \MLR{} method only requires the most basic standardization, one-hot-encoding and standard imputation of missing data. \MLR{} is fully compatible with all feature engineering schemes ($e.g.$ embeddings, Nystr\"om \cite{Williams2001using} and \RBF{} \cite{RasmussenW06} kernels, tree leaves). All the popular \DL{} schemes can also be leveraged including learning rate schedulers \cite{smith2015cyclical}, optimizers, weight decay, batch-normalization, drop-out, residual layers and leaky activations \cite{smith2018disciplined}. 

- The performances of \NN{} are not tied with any of the well-known class of methods. Thus they should be a great addition to the stack of models aggregated by meta-learners. Researchers and practitioners can use \MLR{} on its own as an off-the-shelf \DL{} solution or integrate it into the most advanced ML pipelines. 



- The implementation of our method in torch is available as a stand-alone which follows the scikit-learn API (\textit{i.e.} it can be directly encapsulated into parameter search routines, bagging meta models, \textit{etc.}). For the sake of replicability,  the code to run the benchmarks, the ablation study and the preprocessing applied to each dataset is also provided.



%\paragraph{Paper organisation.}
The rest of the paper is organized as follows. 
We describe our approach in Section \ref{sec:MLRmethod}. In Section \ref{sec:exp}, we carry out a detailed ablation study of our method and evaluate its performances on real data.
}


==> proof-Karim.tex <==
We now have all the necessary ingredients to prove (i). Indeed we first note that for any $\lambda>0$
\begin{align*}
    \MLR(\lambda) + \|P_{\bx}(\bY)\|_2^2 &=  \left(\frac{\lambda/n}{1 +\lambda/n} \right)^{2} \|  \bx\bm{\beta}^* \|_2^2 \left(1 + O\left( \sqrt{\frac{r \sigma^2}{\|\bx\bm{\beta}^*\|_2^2}} \right) \right)+\frac{2 \lambda/n + 1}{(1 + \lambda/n)^2} \left( \frac{r \sigma^2}{(1+\lambda/n)^2} \right)
\end{align*}




\begin{align}
\label{eq:truerisk2}
    R(\lambda)&= \frac{(\lambda/n)^2}{(1 + \lambda/n)^2}  \sum_{j=1}^r \langle \bx\bm{\beta}^* , \bu_j\rangle^2 + \sigma^2 \sum_{j=1}^r\frac{1}{(1 + \lambda/n)^2}= \frac{(\lambda/n)^2 \| \bx\bm{\beta}^*\|^2 + \sigma^2 r }{(1 + \lambda/n)^2}.
\end{align}
% The population risk \eqref{eq:truerisk2} is minimized at 
% \begin{align}
% \label{eq:lambdaopt}
% \lambda^* = \sqrt{\frac{\sigma^2 r}{\|\bx\bm{\beta}^*\|_2^2}},
% \end{align}
% while the minimizer of \MLR{} or equivalently \eqref{eq:MLRloss2} is
% \begin{align}
%     \label{eq:lambdahat}
%     \widehat{\lambda} = \frac{\|P_{\bx}(\bY_{\texttt{perm}})\|_2^2}{\|P_{\bx}(\bY)\|_2^2} + \sqrt{\frac{\|P_{\bx}(\bY_{\texttt{perm}})\|_2^2}{\|P_{\bx}(\bY)\|_2^2} + \left(\frac{\|P_{\bx}(\bY_{\texttt{perm}})\|_2^2}{\|P_{\bx}(\bY)\|_2^2}\right)}.
% \end{align}



Next, if $\lambda_1 = \cdots = \lambda_r = 1$, then \eqref{eq:MLRloss} becomes 
\begin{align}
\label{eq:MLRloss2}
   \MLR(\lambda) &= - \|P_{\bx}(\bY)\|_2^2 + \left(\frac{\lambda/n}{1 +\lambda/n} \right)^{2} \|  P_{\bx}(\bY)\|_2^2+\frac{2 \lambda/n + 1}{(1 + \lambda/n)^2} \| P_{\bx}(\bY_{\texttt{perm}})\|_2^2.
\end{align}
Since $\|P_{\bx}(\bY)\|_2^2$ does not depend on $\lambda$, minimizing $\MLR(\lambda)$ is equivalent to minimizing
\begin{align}
\label{eq:MLRequiv}
    \left(\frac{\lambda/n}{1 +\lambda/n} \right)^{2} \|  P_{\bx}(\bY)\|_2^2+\frac{2 \lambda/n + 1}{(1 + \lambda/n)^2} \| P_{\bx}(\bY_{\texttt{perm}})\|_2^2.
\end{align}

==> r__ponse_ref.tex <==

\newpage


\newpage
\textbf{Question: }\textbf{\textit{"Why the L2 regularization is only applied to the last hidden layer instead of all of parameters? A good justification should be provided."}}

The impact of applying a ridge closed-form on the behavior of MLR goes far beyond a regularization of the weights on the last layer. It allows us to avoid solving a bi-level optimisation problem (argmin of argmax). In addition, it is differentiable and thus fully compatible with gradient descent. See also our previous answer for more details.




The summary provided by the referee is not completely accurate. Using Ridge closed-form on the last hidden layer of the FFNN
already gives some significant improvement of the generalization performance (See the ablation study in Table 4). Using a closed- form compels the network to learn embeddings on the last hidden layer, it does not just regularize the weights."

We also refer to Table 6 in the supplementary on the dependence on $\lambda_{init}$ parameter. We see that the generalization performance can improve significantly by taking some intermediate value of lambda between 0 and $+\infty$. Thus we do not need to use permutation to prevent overfitting of the Ridge closed-form. Permutation is actually used to improve generalization even further on top of what the ridge closed-form already brings.


\textbf{Question: }\textbf{\textit{"It Is Unclear What Explicit Benefits This Approach Should Give Over A Standard Mlp With L2 Regularisation, And The Authors Do Little To Provide Motivation Or Intuition. (Confusingly, The Authors Claim That The Ridge Regression Provides 'Much Stronger' Regularisation Than Adding Standard L2 Weight Regularisation To The Loss. No Further Justification Is Given. This Statement Seems At Odds To Me With The Fact That They Need To Introduce The Permutation Loss To Add Further Regularisation.)"}}


Our benchmark already contained the MLP with L2 regularisation (sklearn.neural_network: MLPRegressor and MLPClassifier). According to the exhaustive result Table in the github repository, standard MLP performs poorly.



\textbf{Question: }\textbf{\textit{"Instead of using the same data for calculating the ridge regression parameters and the loss, have the authors considered splitting the (minibatches of the) data in two? This would avoid the trivial solution of diagonal H as the targets Y in eq 4 no longer match the input. Or how about you simply permute y after computing the ridge regression solution, such that it looks different for the forward pass? Alternatively: instead of using the (somewhat expensive) permutation based loss, why not regularise against diagonal H more directly?"}}

These are interesting suggestions for potential future research. But they fall outside the scope of the MLR methodology.

+++ it has be shown  that MLP+L2 reg works raisonnably on some dataset, but could never bet the state of the art (ref...)

